Evaluating and Improving the Coreference Capabilities of Machine Translation Models

Machine translation (MT) requires a wide range of linguistic capabilities, which current end-to-end models are expected to learn implicitly by observing aligned sentences in bilingual corpora. In this work, we ask: \emph{How well do MT models learn coreference resolution from implicit signal?} To answer this question, we develop an evaluation methodology that derives coreference clusters from MT output and evaluates them without requiring annotations in the target language. We further evaluate several prominent open-source and commercial MT systems, translating from English to six target languages, and compare them to state-of-the-art coreference resolvers on three challenging benchmarks. Our results show that the monolingual resolvers greatly outperform MT models. Motivated by this result, we experiment with different methods for incorporating the output of coreference resolution models in MT, showing improvement over strong baselines.

==> gabi_restructure/00_abstract.tex <==
\begin{abstract}
% - MT models requires addressing \emph{implicitly} a lot of linguistic tasks but our understanding of what is learned is limited.
% - In this work, we measure the coreference capabilities of MT models. we develop an evaluation methodology which consists of deducing \emph{explicit} coreference clusters from the MT model in the target language and evaluate them without any label in the target language. 
%In our evaluation, we compare several commercial and large open source MT models, translating from English to six target languages against SOTA coreference resolvers on three challenging benchmarks.
%Our results show that SOTA coreference models vastly outperform MT models. Consequently,
% - We show ... 
% - to improve coreference capabilities of MT models, we propose both implicit and explicit approaches for injecting coreference signals into MT models. 
% - our method outperforms (many languages, various datasets, ...

% In this work, we investigate the coreference capabilities of end2end neural machine translation against monolingual coreference models. To that end, we develop a new evaluation paradigm that reduces MT models into source-side coreference clusters allowing us to compare their performances on equal ground. We ran experiments on three challenging benchmarks with commercial and large open source models. Our results show that monolingual coreference models are far more capable than MT models. Consequently, we suggest a novel approach of fine-tuning coreference data enriched with coreference signal. Our approach, show vast improvements and achieve comparable or even better results than commercial and large open source MT models. 

Machine translation (MT) requires a wide range of linguistic capabilities, which current end-to-end models are expected to learn implicitly by observing aligned sentences in bilingual corpora.
In this work, we ask: \emph{How well MT models learn coreference resolution via implicit signal?} To answer this question, we develop an evaluation methodology that derives coreference clusters from MT output and evaluates them without requiring annotations in the target language.
Following, we evaluate several prominent open-source and commercial MT systems, translating from English to six target languages, and compare them to state-of-the-art coreference resolvers on three challenging benchmarks.
Our results show that the monolingual coreference resolvers greatly outperform MT models. Motivated by this result, we experiment with different methods for incorporating the output of coreference resolution models in MT, showing improvement over strong baselines.\footnote{Codebase and datasets will be released upon publication.}
%***
%Our method outperforms commercial and large open source MT models on many languages and various datasets.
\end{abstract}

==> gabi_restructure/01_introduction_gabi.tex <==
Machine translation (MT) may require coreference resolution to translate cases where the source and target language differ in their grammatical properties. For example, consider translating \example{The trophy didn't fit in the suitcase because it was too small} from English to French: \example{Le trophée ne rentrait pas dans la valise car elle était trop petite} \citep{Sakaguchi2020WINOGRANDEAA}. In French, suitcase~(\example{valise}) is grammatically feminine and trophy~(\example{trophée}) is masculine, while the source-side English does not encode grammatical noun gender. This requires an MT model to infer that \example{it} refers to the suitcase (and not the trophy) to correctly produce the feminine inflection for the phrase \example{it was too small} (\example{elle était trop petite}), whereas an incorrect coreference resolution may produce the masculine inflection (\example{il était trop petit}) corresponding to the trophy.

% figure 1
\begin{figure}[t]
\centering
\includegraphics[scale=0.33]{images/fig_1_new.png}
\caption{MT models can be compared to source-side coreference resolvers. An example translation from English (blue) to French (yellow). Our method first identifies the grammatical gender of the mentions in the target language marked in purple (female) and blue (male), followed by inferring the source side clusters (orange), through gender agreement.
%In blue, there are English sentences from Wino-X and Wino-MT. In orange, there are translations into French by an MT model. The English sentences have one pronoun and two antecedents/entities (marked in bold) that they can refer. Only one option of the two agrees with world knowledge and solves the coreference resolution correctly. In the translation, the antecedents/entities and entity have grammatical gender marked in purple (female) and blue (male). Using our method, we check if the referring antecedent/entity has the same gender as the pronoun, validating whether the translation matches the source coreference resolution or not. 
}
\label{fig:method_new}
\end{figure}

% Such cases evade lexical one-to-one translation, and instead demand source-side coreference resolution as a prerequisite for producing a correct translation.
% The prominent end-to-end approach to machine translation (citation) assumes that models implicitly learn to resolve such source-side semantic phenomena by observing aligned source-target pairs, without intermediate for the task.

Such texts evade lexical one-to-one translation, and instead demand source-side coreference resolution as a prerequisite for a correct translation. %Other cases can preserve the source-side lexical ambiguity by side-stepping coreference resolution\ariec{this is not clear what is ``preserving lexical ambiguity''. Also it doesn't side-step coref}, for example in the sentence \example{The battery didn't fit the suitcase because it was too small}, where both \emph{battery} and \emph{suitcase} are feminine in French.\ariec{I'd move this part later when we say that we use the pronouns because here the purpose of this statement is too vague.}
The prominent end-to-end approach to MT assumes that translation models implicitly learn source-side coreference resolution by observing aligned source-target pairs that exhibit such phenomena, without intermediate coreference supervision. While the importance of addressing such semantic phenomena been stated in various works~\citep{le-nagard-koehn-2010-aiding,stojanovski-fraser-2018-coreference}, it was also observed that the ubiquitous BLEU metric~\citep{bleu} does not adequately quantify it~\citep{hardmeier-federico-2010-modelling}.


% In this work, we ask the following research question: How does this implicit supervision for coreference resolution fare against direct source-side monolingual training? 

% To answer this question, we develop an evaluation metric to compare the ability of MT and monolingual coreference model on source-side coreference resolution.

% Our approach aims to automatically infer source-side coreference resolution based on the produced translations. Thus, we effectively reduce an MT model to a monolingual coreference resolution


This work addresses the following research question: \textit{How well does MT learn coreference when compared against explicit coreference supervision?}
%Evaluate coreference from implicit supervision and an off-the-shelf supervised coreference is a natural point of comparison.\ariec{I don't understand this sentence}
Answering this question can improve our understanding of the way MT models operate and 
%provide insight into the effects of explicit supervision.
%This question 
also has practical implications: if implicit supervision lags behind monolingual training, it would motivate integration between end-to-end MT approaches and explicitly-supervised monolingual components.
%\ariec{I reiterate my previous comment, implicit supervision of MT can be bad for coref but maybe better models or training data can improve without symbolic components. } %\ariec{That's not accurate, models can be bad at coref but introducing coref signals might not help. I don't think we really need to justify why we want to evaluate the coref capabilites of MT, it's like a probing.} \asafy{we are not saying that, this is a general note on the integration of monolingual signal to end2end models}\oa{now ok?}


% TODO: probably reword
In Section~\ref{sec:consistency_metric} we devise an evaluation paradigm that reduces MT output to source-side coreference resolution predictions by inferring coreference clusters from source inputs and predicted target translations. E.g., in the previous example, 
a feminine inflection for the pronoun ``it'' in French can infer linking ``it'' with ``suitcase'', while a masculine French inflection links ``it'' with ``trophy'', as shown in Figure~\ref{fig:method_new}.
%\oa{Another possibility is to formulate the translation w/o a pronoun, thereby eschewing the coreference problem.}
This approach, built upon recent works focusing on examining gender bias in MT~\citep{stanovsky-etal-2019-evaluating}, allows us to distill the coreference resolution abilities of MT models and compare them against state-of-the-art coreference resolution models, trained explicitly on the task.

We use this approach in Section~\ref{sec:experiments} to evaluate the coreference capabilities of several commercial and open source MT systems, translating from English to six target languages. We conduct our experiments in both synthetic \citep[\winomt{} and \winox{};][]{stanovsky-etal-2019-evaluating,emelin-sennrich-2021-wino}
and naturalistic settings  \citep[\bug{};][]{levy2021collecting}.
Our results show that state-of-the-art coreference resolvers vastly outperform MT models on several benchmarks, indicating that explicit supervision may lead to better coreference performance.
%achieving higher pronoun-antecedent consistency than MT models.
%\ariec{the second half of the sentence doesn't make sense, we don't evaluate consistency but accuracy in english coref models.}\asafy{is it better?}
%On three different datasets, WinoMT 
%.\ariec{the two last sentences are not grammatical/coherent.}

% To improve coreference capabilities of MT models, we propose both implicit and explicit approaches for injecting coreference signals into MT models. 
% Following, we suggest a method for incorporating the signal of a monolingual coref model into MT by ...
Following this finding, in Section~\ref{sec:improving}, we develop methods for improving coreference in MT, both implicitly and explicitly.
Our implicit approach consists of fine-tuning MT models on 
% data that contains coreference clusters on the source side
texts that specifically require many coreference decisions, thus exposing the model to more implicit coreference signal.
Our explicit approach further enriches source sentences with predicted coreference markers. 
We show that these approaches improve coreference over the end-to-end MT approach, achieving comparable or better results than commercial systems, and much bigger open-source MT models. 
% The developed methods do not only improve coreference performance but also lead to more accurate pronoun translation.
%\ariec{What do you mean by ``more accurate translation''? in terms of BLEU?}\asafy{not necessarily, as we can't get BLEU results on our evaluation datasets, but still more consistent translations are more accurate, alternatively by pronoun match results}\ariec{but this falls under coreference consistency, right?}
%Similarly, we show improvements for other metrics, such as pronoun translation and accuracy.\ariec{Readers won't understand this sentence, consider removing this point from the Intro.}

More broadly, our approach can be applied to improve the translation of other semantic phenomena that diverge in realization between source and target languages, such as plurality in second-person pronouns~\citep{Stanovsky2019YallSR} or tense marking~\citep{wolfram1985variability}. %\gabis{add citations} \asafy{like what? your "you" paper? what more?}


==> gabi_restructure/02_background.tex <==
\label{sec:background}
% Coreference resolution is a prerequisite for translating between certain languages, as exemplified in Figure~\ref{fig:method_new}, where producing correct target-side gender agreement relies on source-side coreference resolution. Crucially, a reader of the French translation would infer from the gender inflection of ``it'', whether it refers to ``suitcase'' or the ``trophy''. I.e., a feminine pronoun (``elle'') would agree with the feminine noun suitcase (``valise''), while a masculine pronoun (``il'') would agree with the masculine noun trophy (``trophée').

We start our work by extending the methodology developed in ~\citep{stanovsky-etal-2019-evaluating}, which relies on target-side morphology to infer the translated gender of certain professions.
% \winomt{}~\citep{stanovsky-etal-2019-evaluating} operationalize this observation to evalaute gender bias in MT. 
%In the context of gender bias in machine translation, and get an approximation of the coreference capabilities of MT models by inferring constraints on the target-side clusters from gender agreement.
In particular, assuming a dataset of English sentences $D$, where each instance includes gold coreference annotation between a human entity and its pronoun (e.g., \example{The \textbf{doctor} asked the nurse to help \textbf{her} with the procedure.}), they evaluate gender bias from English to language $T$ with morphological gender in the following manner:


% which describes a scenario with human entities,
% who are identified by their role (e.g., “the doctor” and “the nurse” in Figure 1), and a pronoun
% (“her” in the example), which needs to be correctly
% resolved to one of the entities (“the doctor” in
% this case)

\begin{enumerate}
    \item Predict word alignment between $D$ and $M(D)$, i.e., the output translations of an MT model $M$. This finds the translations for pronouns (e.g., \example{her}) and possible entities (e.g \example{doctor}, \example{nurse}) in the target language $T$.
    \item Automatically extract the gender of the possible entities and the pronouns in the target language based on morphological features.
    \item Check whether the gender of the co-referred entity (e.g., \example{doctor}) in $T$ corresponds to the gender of the English pronoun (e.g., \example{her}).
    % , to form constraints on the coreference clusters.
    % \item
    % \oa{add here how you define the consistency score}
\end{enumerate}

The gender bias of $M$ is then defined as the difference in performance between stereotypical and anti-stereotypical gender role assignments. 

We use a similar setup to address a different question: rather than evaluating the gender bias of the model, we evaluate its coreference abilities, which may be hindered by bias, but also by the inherent difficulty to infer coreference in the absence of an explicit training signal.


% \gabis{$\uparrow$ This seems important enough for small figure, maybe incorporate into Figure~\ref{fig:method_new}}



% As a result, our methodWe note that gender agreement cannot fully identify  cluster assignments, and instead indicates coreference violations.
% % \ariec{because we cannot infer that the model considers them as coreferring}\gabis{for example, ...} 
% Therefore, we treat our measure as an upper bound for the coreference performance of MT models. \ariec{In addition, }Some sentences do not require coreference resolution in order to be translated correctly. Here, we cannot infer the coreference capabilities of the MT model given a feminine inflection of the translation of \emph{it}.
%More generally, we note that gender agreement cannot identify complete cluster assignment and can only indicate coreference violations.\ariec{I'd start the paragraph with something like this sentence, then moving to the example.}  We therefore treat our measure as an upper bound for the coreference performance of MT models.

% We emphasize that our method is completely automatic and does not require any parallel data or target-side annotation.\ariec{but we still require coreference annotation in the source-side. So maybe we can write something like ``Overall, our method allows to measure the coreference capabilities of any MT model translating from English to many languages, while requiring coreference annotation only in the source sentences. } 



%Other cases can preserve the source-side lexical ambiguity by side-stepping coreference resolution\ariec{this is not clear what is ``preserving lexical ambiguity''. Also it doesn't side-step coref}, for example in the sentence \example{The battery didn't fit the suitcase because it was too small}, where both \emph{battery} and \emph{suitcase} are feminine in French.\ariec{I'd move this part later when we say that we use the pronouns because here the purpose of this statement is too vague.}

%We emphasize that our consistency measure provides an upper bound to the coreference abilities of the MT model, as our measure only checks for implicate agreement. Moreover, as noted earlier, for some sentences\ariec{which kind of sentences? } gender agreement can not identify clear clusters assignment and can only indicate coreference violations. Therefore, we treat our measure as the upper bound for coreference performances of MT models.\ariec{this repeats the first sentence of this paragraph}
%1. translate all sentences in D to target language T using model M. 2. align all the sentences in D with their counterpart translations in the target language T using awesome-align \citep{Dou2021WordAB}. Then extract all the translations of mentions annotated in the data set D (e.g ..). 3. Then extract the morphological gender of the target side mentions using language-specific morphological analysis, which we perform using a combination of the off-the-shelf tools together with handcrafted rules design for each target language upon its unique characteristics, as discussed in the following section. 4. For each target pronoun we check if the target side antecedent or entity is in agreement on their attributes, obtaining the necessary constraints. 

%This methodology uses the gender agreement as a tool for inferring the source side clusters by the MT translation. Allowing us to compare MT models against SOTA coreference models on equal ground. \ariec{we already wrote something similar earlier} 

%In addition, we check for each entity if it agrees with the source side gold gender. While the first measure the consistency of model M, the second quantified its accuracy.\oa{I didn't understand the last sent}

%To make the distinction between consistency and accuracy let's examine different translations of our running example from earlier, when both the pronoun and the relevant antecedent share the same gender then the translation is consistent but it is accurate only if the target gender is the source gender. Otherwise, if the entity and pronoun are not in agreement on their gender, the translation is not consistent and only partially accurate. Ideally, we would like a translation to be both consistent and accurate.

% We want to note that both the alignment (2) and the gender extraction (3) might add some noise to the measurement and affect it. In Section~\S\ref{sec:results}, we will present human evaluation showing that these errors are uncommon and have a small effect on the overall results.
%Either directly by returning wrong gender or either by predicting UNKNOWN for empty strings and words without morphological gender.%~\ariec{this sentence is too much detailed from this section IMO}


%We note that target side entity, antecedent or pronoun can be detected as UNKNOWN. This can happen either when word alignment don't find a corresponding word\oa{corresponding to what?} in target language or either when the morphological gender extraction found the gender of the word to be UNKNOWN\oa{when does this happen?}. We observe that for some pro drop languages (e.g Spanish) the target sentence can be consistent without containing an aligned target pronoun.\oa{how so?} Alternatively, when the aligned target pronoun is found but is ambiguous without any morphological gender or is a possessive pronoun in languages that the gender associated with the object and not the entity.\oa{didn't understand the last sent}


==> gabi_restructure/02_evaluation_setup.tex <==
In this work, we note that the approach taken in \winomt{} can be applied beyond the context of gender bias to estimate general coreference abilities of MT.
As exemplified in Figure~\ref{fig:method_new}, producing correct target-side gender agreement relies on source-side coreference resolution. Crucially, a reader of the French translation would infer from the gender inflection of ``it'', whether it refers to ``suitcase'' or the ``trophy''. I.e., a feminine pronoun (``elle'') would agree with the femininenoun suitcase (``valise''), while a masculine pronoun (``il'') would agree with the masculine noun trophy (``trophée').



\paragraph{Required components.} Our evaluation methodology relies on bilingual and monolingual resources, namely an aligner between English and the target language $T$, and a morphological analyzer for $T$. Both inherently add some noise to the measurement and may thus skew our results. In section~\S\ref{sec:results} we present a manual evaluation showing that these errors are uncommon and have a small effect on the overall results.

\paragraph{Our method is an upper bound estimation of MT coreference abilities.} 
Some texts may keep the English ambiguity in the translation, and hence absolve the translation model from resolving coreference. For example, in the sentence \example{The battery didn't fit the suitcase because it was too small}, both \emph{battery} and \emph{suitcase} are feminine in French. Our proposed evaluation method will indicate that the MT model was trivially successful in such cases, and hence serves as an upper bound on its true coreference abilities.

%% \paragraph{Our approach is a generalization of \winomt{}.}
%% Unlike WinoMT,  we do not evaluate societal gender bias in MT systems, but rather use gender as a gauge for the coreference abilities of MT systems. We stress that these are different motivations, as both biased and unbiased systems may fail to perform coreference. 
%% To do so, in the following section we define a \emph{consistency} metric to quantify the frequency in which MT systems generate pronouns that are inconsistent with their coreferent. 





\subsection{Metrics}


\label{subsec:eval}

This section describes our extensive evaluation framework, consisting of 3 evaluation datasets, 6 MT models, the alignment model we use for our consistency evaluation, and the 6 diverse target languages. 
%Then, we will detail the MT models and the training datasets we use for the improving coreference consistency experiments~(§\ref{subsec:improve_exp}).

\textbf{Evaluation Datasets.} %For evaluation, we use three challenging coreference annotated test data in English. Wino-X, WinoMT and BUG aims to measure coreference capabilities in both synthetic and naturalistic settings that require world knowledge.\ariec{consider removing, we explain these datasets in more details just below.}
The first dataset we use is \textbf{Wino-X} \citep{emelin-sennrich-2021-wino}, a filtered subset of WinoGrande \citep{Sakaguchi2020WINOGRANDEAA} built to test commonsense reasoning and coreference resolution of MT models and multilingual encoders. The dataset contains sentences similar to the one in Figure~\ref{fig:method_new}. All sentences have two entities and a pronoun, ``it'', coreferring to one of them. The dataset consists of three parts, each part constructed for a different target language (German, French, and Russian), where each part only contains sentences where the two entities have different morphological gender in the target language. 
This filtration procedure enables more accurate consistency results as the gendered pronoun clearly indicates the coreferring antecedent. Hence this dataset better reflects the MT model source-side coreference resolution capabilities.
% Each part of the dataset contains sentences from WinoGrande only if the two entities in the source sentence are expected to have different morphological gender in the target language.

Second, we use \textbf{WinoMT} \citep{stanovsky-etal-2019-evaluating}, a dataset built following the Winograd schema \citep{Levesque2011TheWS}, designed to test gender bias and coreference resolution of MT models. The sentences in this dataset contain two human entities and one gendered pronoun, e.g., \example{The \textbf{doctor} asked the \textbf{nurse} to help \textbf{her} in the procedure}. The gendered pronoun reveals the gender of the entity and adds gender attributes to the source cluster. In our example, \example{her} refers to the \example{doctor}, revealing the doctor's gender.

Finally, our third dataset is \textbf{BUG} \citep{levy2021collecting}, a semi-automatic collection of natural English sentences that are challenging with respect to societal gender-role assignments. Similar to WinoMT, each sentence contains a human entity, identified by their profession and a gendered pronoun. 
Here we use the \textsc{Gold} portion of this dataset, validated by human annotators, in order to reduce noise in the evaluation. All datasets statistics are presented in App. \S\ref{sec:appendix:06_data_sizes}.

\noindent
\textbf{Machine translation Models.} We apply our evaluation methodology on four Transformers-based machine translation models from EasyNMT\footnote{https://github.com/UKPLab/EasyNMT}: mBART50 \citep{https://doi.org/10.48550/arxiv.2008.00401, liu-etal-2020-multilingual-denoising}, M2M\_418M, M2M\_1.2B \citep{Fan2021BeyondEM}, and the monolingual
Opus-MT~\citep{tiedemann-thottingal-2020-opus}, representing the state-of-the-art for publicly available neural machine translations models.
In addition, we measure coreference consistency on the output of two commercial systems: Google Translate\footnote{https://cloud.google.com/translate} and Microsoft Translator\footnote{https://www.bing.com/translator}. 

\noindent
\textbf{Target Languages.} We conduct our evaluation study on MT models translating from English to a set of six diverse target languages with grammatical gender: Arabic, German, Spanish, Hebrew, Russian and French.
These languages have a variety of linguistic traits (e.g., alphabet, word order, number of grammatical genders, or grammar), while still allowing for highly accurate automatic morphological analysis.
These languages belong to four different families: (1) Romance languages: Spanish and French, which have gendered noun-determiner agreement; Spanish is also a \emph{pro-drop} language, i.e., pronouns can be omitted in certain cases, which in our setting may keep the coreference ambiguity of the source-side English sentence \citep{Webster2020ScalableCL} %, Wang2018TranslatingPL}. 
(2) Slavic languages (Cyrillic alphabet): Russian; that have three grammatical genders (3) Semitic languages: Hebrew and Arabic, each with a unique alphabet; both are partial pro-drop languages. (4) Germanic languages: German, also has three grammatical genders.

% \ariec{more or remove}
% After translating the English sentences to these six languages, we obtain word-alignment between the source and target sentences using awesome-align \citep{dou-neubig-2021-word}, a neural word aligner based on multilingual BERT. To extract the morphological gender of the aligned entity and the pronoun, we use spaCy\footnote{https://spacy.io/} for Spanish, French, Russian, and German, and Stanza~\citep{qi-etal-2020-stanza} for Hebrew and Arabic. 


==> gabi_restructure/03_0_method.tex <==
\label{sec:background}
Coreference resolution is a prerequisite for translating between certain languages, as exemplified in Figure~\ref{fig:method_new}, where producing correct target-side gender agreement relies on source-side coreference resolution. Crucially, a reader of the French translation would infer from the gender inflection of ``it'', whether it refers to ``suitcase'' or the ``trophy''. I.e., a feminine pronoun (``elle'') would agree with the feminine noun suitcase (``valise''), while a masculine pronoun (``il'') would agree with the masculine noun trophy (``trophée').

Following \citet{stanovsky-etal-2019-evaluating}, we operationalize this observation and get an approximation of the coreference capabilities of MT models by inferring constraints on the target-side clusters from gender agreement.
In particular, assuming we have an English dataset $D$ with gold coreference annotation, we evaluate the coreference performance of an MT model $M$ (from English to language $T$ with morphological gender) in the following manner:

\begin{enumerate}
    \item Predict word alignment between $D$ and $M(D)$, i.e., the output translations of $M$. This allows us to find the translations for pronouns and possible entities in the target language $T$.
    \item Automatically extract the gender of the possible entities and the pronouns in the target language based on morphological features.
    \item Check gender agreement between the pronoun and the coreferring entity.
    % , to form constraints on the coreference clusters.
    % \item
    % \oa{add here how you define the consistency score}
\end{enumerate}

% \gabis{$\uparrow$ This seems important enough for small figure, maybe incorporate into Figure~\ref{fig:method_new}}

\paragraph{Required components.} Our evaluation methodology relies on bilingual and monolingual resources, namely an aligner between English and the target language $T$, and a morphological analyzer for $T$. Both inherently add some noise to the measurement and may thus skew our results. In section~\S\ref{sec:results} we present a manual evaluation showing that these errors are uncommon and have a small effect on the overall results.

\paragraph{Our method is an upper bound estimation of MT coreference abilities.} 
Some texts may keep the English ambiguity in the translation, and hence absolve the translation model from resolving coreference. For example, in the sentence \example{The battery didn't fit the suitcase because it was too small}, both \emph{battery} and \emph{suitcase} are feminine in French. Our proposed evaluation method will indicate that the MT model was trivially successful in such cases, and hence serves as an upper bound on its true coreference abilities.

\paragraph{Our approach is a generalization of \winomt{}.}
Unlike WinoMT,  we do not evaluate societal gender bias in MT systems, but rather use gender as a gauge for the coreference abilities of MT systems. We stress that these are different motivations, as both biased and unbiased systems may fail to perform coreference. 
To do so, in the following section we define a \emph{consistency} metric to quantify the frequency in which MT systems generate pronouns that are inconsistent with their coreferent. 
Consequently, our metric can be applied to any sentence, even when candidate entities have no gender in English, as shown in Figure \ref{fig:method_new}.



% As a result, our methodWe note that gender agreement cannot fully identify  cluster assignments, and instead indicates coreference violations.
% % \ariec{because we cannot infer that the model considers them as coreferring}\gabis{for example, ...} 
% Therefore, we treat our measure as an upper bound for the coreference performance of MT models. \ariec{In addition, }Some sentences do not require coreference resolution in order to be translated correctly. Here, we cannot infer the coreference capabilities of the MT model given a feminine inflection of the translation of \emph{it}.
%More generally, we note that gender agreement cannot identify complete cluster assignment and can only indicate coreference violations.\ariec{I'd start the paragraph with something like this sentence, then moving to the example.}  We therefore treat our measure as an upper bound for the coreference performance of MT models.

% We emphasize that our method is completely automatic and does not require any parallel data or target-side annotation.\ariec{but we still require coreference annotation in the source-side. So maybe we can write something like ``Overall, our method allows to measure the coreference capabilities of any MT model translating from English to many languages, while requiring coreference annotation only in the source sentences. } 



%Other cases can preserve the source-side lexical ambiguity by side-stepping coreference resolution\ariec{this is not clear what is ``preserving lexical ambiguity''. Also it doesn't side-step coref}, for example in the sentence \example{The battery didn't fit the suitcase because it was too small}, where both \emph{battery} and \emph{suitcase} are feminine in French.\ariec{I'd move this part later when we say that we use the pronouns because here the purpose of this statement is too vague.}

%We emphasize that our consistency measure provides an upper bound to the coreference abilities of the MT model, as our measure only checks for implicate agreement. Moreover, as noted earlier, for some sentences\ariec{which kind of sentences? } gender agreement can not identify clear clusters assignment and can only indicate coreference violations. Therefore, we treat our measure as the upper bound for coreference performances of MT models.\ariec{this repeats the first sentence of this paragraph}
%1. translate all sentences in D to target language T using model M. 2. align all the sentences in D with their counterpart translations in the target language T using awesome-align \citep{Dou2021WordAB}. Then extract all the translations of mentions annotated in the data set D (e.g ..). 3. Then extract the morphological gender of the target side mentions using language-specific morphological analysis, which we perform using a combination of the off-the-shelf tools together with handcrafted rules design for each target language upon its unique characteristics, as discussed in the following section. 4. For each target pronoun we check if the target side antecedent or entity is in agreement on their attributes, obtaining the necessary constraints. 

%This methodology uses the gender agreement as a tool for inferring the source side clusters by the MT translation. Allowing us to compare MT models against SOTA coreference models on equal ground. \ariec{we already wrote something similar earlier} 

%In addition, we check for each entity if it agrees with the source side gold gender. While the first measure the consistency of model M, the second quantified its accuracy.\oa{I didn't understand the last sent}

%To make the distinction between consistency and accuracy let's examine different translations of our running example from earlier, when both the pronoun and the relevant antecedent share the same gender then the translation is consistent but it is accurate only if the target gender is the source gender. Otherwise, if the entity and pronoun are not in agreement on their gender, the translation is not consistent and only partially accurate. Ideally, we would like a translation to be both consistent and accurate.

% We want to note that both the alignment (2) and the gender extraction (3) might add some noise to the measurement and affect it. In Section~\S\ref{sec:results}, we will present human evaluation showing that these errors are uncommon and have a small effect on the overall results.
%Either directly by returning wrong gender or either by predicting UNKNOWN for empty strings and words without morphological gender.%~\ariec{this sentence is too much detailed from this section IMO}


%We note that target side entity, antecedent or pronoun can be detected as UNKNOWN. This can happen either when word alignment don't find a corresponding word\oa{corresponding to what?} in target language or either when the morphological gender extraction found the gender of the word to be UNKNOWN\oa{when does this happen?}. We observe that for some pro drop languages (e.g Spanish) the target sentence can be consistent without containing an aligned target pronoun.\oa{how so?} Alternatively, when the aligned target pronoun is found but is ambiguous without any morphological gender or is a possessive pronoun in languages that the gender associated with the object and not the entity.\oa{didn't understand the last sent}


==> gabi_restructure/03_coref_evaluation.tex <==
% In this section we describe an evaluation which directly compares between the coreference capabilities of MT models and those of source-side coreference resolvers. 


The approach taken in \winomt{} is limited as it restricts the evaluation to sentences with a known gender in English, indicated by a gendered pronoun of a human entity (e.g., \emph{her}). Consider the sentence in Figure~\ref{fig:method_new}: \example{The trophy didn't fit in the suitcase because it was too small} with the coreference cluster \{suitcase, it\}. Step 3 in \citeauthor{stanovsky-etal-2019-evaluating}'s method will fail to assign a coreference label to the translation, because \example{it} does not have a gender in English. In this section, we extend the \winomt{} approach in order to estimate more general coreference abilities of MT models. 



% \oa{I don't understand this sentence. Where does the problem lie exactly?} \ariec{I mean that Gabi's approach works only on English sentences with a gendered pronoun (e.g. him, her etc) because they compare the gender of aligned profession in the target language to the english pronoun. They can't check coref capabilities on sentences like "the trophy didn't fit in the suitcase because it was too small" because "it", "trophy" and "suitcase" don't have a gender in english}\gabis{I agree the sentence is unclear, and I'm not sure I understand the challenge still. In winomt we take gold coref annotation in the source side English, indeed between gendered pronouns, but why does it matter? maybe add an example where winomt breaks?}  


To achieve this, we note that many languages have gender agreement between pronouns and the noun that they refer to. Therefore, correct target-side gender agreement requires (implicitly) resolving the source-side coreference of the relevant entities. As exemplified in Figure~\ref{fig:method_new}, a reader of the French translation 
%of the English sentence \example{The trophy didn't fit in the suitcase because it was too small} 
would infer from the gender inflection of ``it'' whether it refers to ``suitcase'' or the ``trophy''. I.e., a feminine pronoun (``elle'') would agree with the feminine noun suitcase (``valise''), while a masculine pronoun (``il'') would agree with the masculine noun trophy (``trophée'). 
We therefore formulate a new metric quantifying the ability of the MT model to implicitly resolve source-side coreference (henceforth,  \textit{Target-side Consistency}), defined as the proportion of instances in which the morphological gender of an entity (e.g., ``suitcase'') matches that of its referring pronoun (e.g., ``it'') in the target language $T$.% which has this grammatical property.

This metric examines whether an MT model is consistent in its coreference decisions, regardless of whether it correctly inferred the coreference relations in the input text. Indeed, some texts may keep the English ambiguity in the translation, and hence absolve the MT model from resolving coreference. For example, in the sentence \example{The battery didn't fit in the suitcase because it was too small}, both \emph{battery} and \emph{suitcase} are feminine in French. Our proposed metric will correctly indicate that the MT model was successful in such cases (albeit trivially). The metric thus serves as an upper bound on the MT model's coreference abilities.

We note that while this framing uses the morphological gender inflection of common nouns, it is different in motivation from measures of gender bias. In our example above, gender inflection allows us to determine whether an MT model correctly employs common sense rather than examining whether it tends to prefer stereotypical gender norms. While a model's gender bias may explain some loss in coreference abilities, the model's ability to resolve coreference need not be aligned with the degree of its bias (e.g., a random gender assignment would result in
unbiased performance, but very poor coreference ability).

Most importantly, by considering the gender of the entity and the pronoun, we obtain mention clusters which can be compared against those produced by coreference resolution models. In our example figure, both the first MT model and the coreference model produce the correct clustering: \{\{trophy\}, \{suitcase, it\}\}, while the second MT model errs by producing: \{\{trophy, it\}, \{suitcase\}\}.


% This metric examines whether an MT model is consistent with regards to the coreference decision, regardless of whether it correctly inferred the coreference relations in the input text.

% In this section we describe an evaluation which directly compares between the coreference capabilities of MT models and those of source-side coreference resolvers. 


% To achieve this, we note that the approach taken in \winomt{} can be applied beyond the context of gender bias to estimate general coreference abilities of MT. 
% As exemplified in Figure~\ref{fig:method_new}, producing correct target-side gender agreement relies on source-side coreference resolution. A reader of the French translation would infer from the gender inflection of ``it'', whether it refers to ``suitcase'' or the ``trophy''. I.e., a feminine pronoun (``elle'') would agree with the feminine noun suitcase (``valise''), while a masculine pronoun (``il'') would agree with the masculine noun trophy (``trophée'). 

% Most importantly, by applying considering the gender of the entity and the pronoun, we obtain mention clusters which can be directly compared against those produced by coreference resolution models. E.g., in our example figure, MT model A and the coreference model both produce the correct clustering \{\{trophy\}, \{suitcase, it\}\}, while the second MT model produces the erroneous clustering \{\{trophy, it\}, \{suitcase\}\}.


% We note that while this framing uses the morphological gender inflection of common nouns, it is different in motivation from societal gender bias. In our example above, gender inflection allows us to determine whether an MT model correctly employs common sense rather than examining whether it tends to prefer stereotypical gender norms. 


% Following this observation, 
% % in Section~\ref{sec:metrics} we formulate a suite of metrics by which we estimate how well MT models resolve coreference, 
% in Section~\ref{sec:cons_results} we use these automated metrics to show that MT vastly underperforms direct supervision, and in Section~\ref{sec:human_valid} we validate our results through extensive human annotation.

% Motivated by these results, in Section~\ref{sec:improving}, we improve the coreference in MT models by integrating the output of source-side coreference resolvers into the source-side inputs.

% \subsection{Metrics}
% \label{sec:metrics}
% We formulate two evaluation metrics by which we can compare different aspects of the coreference quality of an MT model:

% \begin{enumerate}
%     \item \textit{Target-side Consistency} is defined as the proportion of instances in which the morphological gender of an entity (e.g., ``suitcase'') matches that of its referring pronoun, both in the target language $T$. This metric examines whether an MT model is consistent with regards to the coreference decision, regardless of whether it correctly inferred the coreference relations in the input text. For example,  \gabis{<- Did I get this right? Can we give an example?}
    
%     \item \textit{Pronoun Accuracy} measures the proportions of instances where a target-side translation matched the coreference clusters of the input text. \gabis{<- Did I get this right? Can we give an example? If I did then I think we can find a more descriptive name for this metric}
    
    
% \end{enumerate}


\subsection{Evaluation Setup}
\label{subsec:eval}

% This section describes our extensive evaluation framework, consisting of 3 evaluation datasets, 6 MT models, the alignment model we use for our consistency evaluation, and the 6 diverse target languages.\oa{I don't think we need this self congratulation; consider removing} 
%Then, we will detail the MT models and the training datasets we use for the improving coreference consistency experiments~(§\ref{subsec:improve_exp}).

\paragraph{Evaluation datasets.} %For evaluation, we use three challenging coreference annotated test data in English. Wino-X, WinoMT and BUG aims to measure coreference capabilities in both synthetic and naturalistic settings that require world knowledge.\ariec{consider removing, we explain these datasets in more details just below.}
The first dataset we use is \winox{}~\citep{emelin-sennrich-2021-wino}, a filtered subset of WinoGrande \citep{Sakaguchi2020WINOGRANDEAA} built to test commonsense reasoning and coreference resolution of MT models and multilingual encoders. The dataset contains sentences similar to the one in Figure~\ref{fig:method_new}. All sentences have two entities and a pronoun, ``it'', coreferring to one of them. The dataset consists of three parts, each part constructed for a different target language (German, French, and Russian), where each part only contains sentences where the two entities have different morphological gender in the target language (e.g., in French \example{trophy} is masculine whereas \example{suitcase} is feminine). Hence, applying our target-side consistency metric on these filtered sentences avoids trivial instances where both candidate entities have the same gender in the target language, and provides a clearer picture of the coreference capabilities of the model.

% This filtration procedure enables more accurate consistency results as the gendered pronoun clearly indicates the coreferring antecedent. Hence this dataset better reflects the MT model source-side coreference resolution capabilities.\oa{better than what? what's the comparison here?}
% Each part of the dataset contains sentences from WinoGrande only if the two entities in the source sentence are expected to have different morphological gender in the target language.

Second, we use \winomt{}~\citep{stanovsky-etal-2019-evaluating},\footnote{\winomt{} is a combination of Winogender~\citep{rudinger-etal-2018-gender} and WinoBias~\citep{zhao-etal-2018-gender}.} a dataset built following the Winograd schema \citep{Levesque2011TheWS}, designed to test gender bias and coreference resolution of MT models. The sentences in this dataset contain two human entities and one gendered pronoun, e.g., \example{The doctor asked the nurse to help her in the procedure}. The gendered pronoun reveals the gender of the entity and adds gender attributes to the source cluster. In our example, \example{her} refers to the \example{doctor}, revealing the doctor's gender. 

Our third dataset is \bug{}~\citep{levy-etal-2021-collecting-large}, a semi-automatic collection of naturalistic English sentences that are challenging with respect to societal gender-role assignments. Similar to WinoMT, each sentence contains a human entity, identified by their profession and a gendered pronoun. 
To reduce noise, we use the \textsc{Gold} portion of this dataset which was validated by human annotators. All datasets statistics are presented in Table \ref{table:data_val}.

\input{tables/data/val}

\paragraph{Machine translation models.} We apply our evaluation methodology to four Transformer-based machine translation models from EasyNMT:\footnote{https://github.com/UKPLab/EasyNMT} mBART50 \citep{https://doi.org/10.48550/arxiv.2008.00401, liu-etal-2020-multilingual-denoising}, M2M\_418M, M2M\_1.2B \citep{Fan2021BeyondEM}, and the bilingual
Opus-MT~\citep{tiedemann-thottingal-2020-opus}, representing the state-of-the-art for publicly available neural machine translations models.
In addition, we measure coreference consistency on the output of two commercial systems: Google Translate\footnote{https://cloud.google.com/translate} and Microsoft Translator.\footnote{https://www.bing.com/translator}

\paragraph{Target languages.} For WinoMT and BUG, we translate from English to six different languages: Arabic, German, Spanish, Hebrew, Russian and French. These languages form a diverse set with respect to how they encode grammatical gender (e.g., number of grammatical genders), as well as to their orthography, word order and other linguistic traits, while still allowing for highly accurate automatic morphological analysis.
These languages belong to four families: (1) Romance languages: Spanish and French, which have gendered noun-determiner agreement with two grammatical genders; Spanish is also a \emph{pro-drop} language, i.e., pronouns can be omitted in certain cases, which in our setting may keep the coreference ambiguity of the source-side English sentence~\citep{Webster2020ScalableCL}.  
(2) Slavic languages (with Cyrillic alphabets): Russian with 3 grammatical genders. (3) Semitic languages: Hebrew and Arabic, each with a unique alphabet; both are partial pro-drop languages and have two grammatical genders. (4) Germanic languages: German with 3 grammatical genders.

% \ariec{more or remove}
% After translating the English sentences to these six languages, we obtain word-alignment between the source and target sentences using awesome-align \citep{dou-neubig-2021-word}, a neural word aligner based on multilingual BERT. To extract the morphological gender of the aligned entity and the pronoun, we use spaCy\footnote{https://spacy.io/} for Spanish, French, Russian, and German, and Stanza~\citep{qi-etal-2020-stanza} for Hebrew and Arabic. 

\subsection{Target-side Consistency Results}
\label{subsec:evaluate_cons}

We first evaluate the accuracy of existing coreference resolvers on our three evaluation datasets, where accuracy is defined as the percentage of instances in which the model identifies that the pronoun is coreferring with the correct entity.
We select state-of-the-art models trained on CoNLL-2012~\citep{pradhan-etal-2012-conll}: SpanBERT~\citep{Joshi2020SpanBERTIP},\footnote{Using AllenNLP's implementation~\citep{Gardner2018AllenNLPAD}.} the s2e model~\citep{Kirstain2021CoreferenceRW} and \textsc{LingMess}~\citep{Otmazgin2022LingMessLI}.
Results in Table \ref{table:coref_models} show that coreference models perform quite well on \winomt{} and \bug{} but poorly on \winox{} (60.8 for \emph{s2e}), indicating weak commonsense capabilities. 

\input{tables/01_coref_models}
\input{tables/winox_cons}
\input{tables/winomt_bug}



Table~\ref{tab:winox_cons} shows the target-side coreference consistency scores for all MT models on \winox{}, which, as mentioned above~(§\ref{subsec:eval}), includes only sentences where the entity and pronoun should be translated using different genders in the target language. We observe that all MT models perform poorly on \winox{} with the highest average score of 46.2 for mBART50, which vastly underperforms English coreference resolvers by 14.6 points. Interestingly, many instances are inconsistent because models tend to generate \textit{neutral} pronoun whereas a gendered pronoun is expected, for example,  {\it cela}, {\it c'était} in French ($31\%$ of translations) and \foreignlanguage{russian}{это,они} in Russian ($17\%$ of translations), meaning ``this'' or ``they'' in English. Likewise, $68\%$ of German translations include neutral pronouns (e.g., ``es''), while only $22\%$ of the entities are neutral. The reported percentages were calculated on Opus-MT. Similar trends were observed in all models. 


Table~\ref{table:winomt_bug} shows the target-side consistency results for \winomt{} and \bug{}. Following common practices on those datasets~\citep{stanovsky-etal-2019-evaluating, levy-etal-2021-collecting-large}, we omit sentences where the candidate pronoun does not provide information about the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun. See App. \S\ref{sec:appendix:04_models_exampels} for more examples. 



% \begin{itemize}
%     \item What do we want to show from the results?
%     \begin{enumerate}
%         \item Wino-X with only challenging sentences: MT models vastly underperform english coref resolvers (e.g. avg of Google is 39.3 vs. 60.8 for s2e). \ariec{Asaf - if the genders are masc and neutral, (e.g., cela), do we consider it as consistent or not?}    
%         \item Although sentences in WinoMT and BUG may lead to sentences with the same gender in both entities in the target language, MT still underpeform coref resolvers (e.g. Google in WinoMT is 64.4 vs. 81.7 for s2e), with some exceptions in BUG \ariec{Asaf - can you report the number of sentences with same gender in both entities in WinoMT? BUG doesn't have a second candidate entity but we can manually analyze a sample, say 100 sentences}
%         \item are there languages that are easier? it's hard to say...
%     \end{enumerate}
% \end{itemize}

Similarly to \winox{}, target-side consistency results on \winomt{} are consistently lower than coreference resolvers. Further, we observe that consistency is affected by two factors: the MT model and the target language. Regarding models, Opus-MT achieves lowest performance, with average consistency of $59.3$, while mBART50 achieves high results with average consistency of $70.5$, sometimes surpassing the second-best MT model by about 9 points. This might be due to the extensive pre-training of mBART50, as previously demonstrated for monolingual LMs \citep{Huang2019CosmosQM, Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR}. With respect to target languages, Russian consistency results are systematically lower than the results in other languages, to the extent that the best model in Russian provides lower results than the worst model in most other languages. In contrast, all models in German achieve a consistency score of about $70$ or more, which can be due to its similarity with English and the research focus on improving English-German translations. 

Consistency results on BUG are higher than on WinoMT for most models, while sometimes surpassing English coreference resolvers, notably in Hebrew and Arabic (e.g., 91.8 for Google vs. 74.6 for \textsc{LingMess}). To understand this gap, we analyze the translation of 50 BUG sentences to Hebrew and French and find that most instances (45 in Hebrew and 33 in French) do not include a distracting entity which should be translated to a different gender in the target language. As mentioned above~(§\ref{sec:consistency_metric}), our metric trivially indicates those examples as consistent.

Overall, target-side consistency results across all datasets demonstrate that both open-source and commercial MT systems exhibit rather poor coreference capabilities compared to English coreference models. 


%Table \ref{table:cons_gmf} presents the consistency results on WinoMT. 

%We first observe that coreference resolvers on average are more accurate on WinoMT than on Wino-X by more than $20\%$ .
%\ariec{move that to afterwards, you first need to explain the results on WinoMT, then compare them to other results} 
%We note that our consistency results are an upper bound on the coreference performance of the MT models.\ariec{But this is always the case, right?} We also note that here we exclude sentences where the pronoun does not provide information on the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun.

% Our results suggest that most tested systems across six tested languages perform quite poorly on our metric.\ariec{can you write a range of performance? what do you mean by poorly? mbart obtains 75+ on some languages of WinoMT, it's not so poor...} The best performing model in each language often does not match the performance of SOTA coreference resolvers. An exception to this rule is in German, where mBART50 and Google Translate achieve better scores than SpanBERT.\ariec{Yes but SpanBERT is not so recent, these MT models are much more recent} This may be explained by German’s similarity to English \citep{Hawkins1986ACT} combined with the amounts of resources and research focus directing to improve English-German translation.\oa{so why does that mean it's more likely to work? I would just say that German is the language with the most resources and research focus, so it's likely it will score higher than others.}\asafy{I combined the two} Another interesting observation is that mBART50 achieves consistently high results compared to other models, sometimes surpassing the second MT model by 3 points. This may be attributed to the extensive pre-training of mBART50, that may endow models with commonsense knowledge, as previously indicated for large-scale monolingual LMs\ariec{is that verbatim?} \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}.

% \input{tables/exampels_improvment}
%We emphasize that our consistency measure can correctly identify a vast variety of different valid uses of pronoun in MT models output's.

\subsection{Human Validation}

The use of automatic tools in the proposed methodology inevitably implies the introduction of noise into the process.
To assess the quality of our measurements, we randomly sampled 50 translations of the Opus-MT model from all evaluation datasets and in all target languages (for a total of 750 annotations), annotating each sample in-house by a native speaker of the target language. The human annotators were asked to identify if the candidate pronoun is indeed the target pronoun and to verify that the gender prediction is correct. This way, we can account for both types of possible errors, i.e., alignment and gender extraction. 

We compare the human annotations to the output of our automatic method and find that the average agreement over all languages and datasets is above $90\%$ (see full results in App. \S\ref{sec:appendix:05_human_validation_results}). These results are comparable to the ones reported by \citet{stanovsky-etal-2019-evaluating}, who conducted human validation and reported that their alignment and gender prediction of the entity in question were reliable for $85\%$ of translations across all languages. %\ariec{what's the purpose of this sentence?}
%\oa{this sentence is unclear; in what setting did they show it?}
%Based on the combination of \citep{stanovsky-etal-2019-evaluating} with our evaluation we can safely say that our alignment and gender prediction are reliable. 
% From the combination of these two results we may conclude that the two tools used for defining our consistency score, e.g. entity and pronoun alignment and gender, are largely reliable.

Some errors can be caused by idiosyncrasies that affect the morphological analysis, as \citet{stanovsky-etal-2019-evaluating} noted.
For example, gender for certain words in Hebrew cannot be determined without diacritics, and some pronouns in German are used in both masculine and neutral forms (e.g., sein), or feminine and third-person plural forms (e.g., ihr). In addition, we notice that sentences from \bug{}, specifically in partial pro-drop languages, were found to be more challenging for the alignment model, and account for most mistakes in Hebrew and Arabic.

% This can be explained by the partial pro-drop treat of those languages, making the alignment of the source pronoun and the relevant target word much harder.\asafy{I add this sentence instead of the next, consider removing the corresponding app.}
% This can be explained by the combination of the longer and naturalistic sentences in BUG and \gabis{this last part is a bit vague ->} the way that the pronoun is translated in partial pro-drop languages. 

==> gabi_restructure/04_0_improving_coref.tex <==
In the previous section, we showed that the coreference performance of MT systems, obtained through an implicit signal, seems inferior to that of coreference resolution learned from an explicit signal. This result raises the question of whether we can leverage dedicated conference resolvers to improve the consistency of MT coreference.

To address this question, we propose two simple data augmentation techniques that leverage a source-side English coreference model. In the following section we experiment with both of these approaches.


\paragraph{Augmented fine-tuning with instances which require coreference resolution.} First, we run a coreference resolution model on the source-side sentences and identify those that have non-singleton clusters.
The motivation for this approach is that further fine-tuning on such instances would expose the MT model to examples that may bear a coreference signal.

\paragraph{Adding explicit source-side coreference markers.}
Second, we use non-singleton clusters outputted by the coreference model by adding inline coreference mark up to the source sentences to mark clusters. For our example sentence, this process  produces the following source side sequence: \emph{``The trophy didn't fit in the \textbf{<ENT1>} suitcase \textbf{</ENT1>} \textbf{<ENT1>} it \textbf{</ENT1>} was too small''}, indicating that ``suitcase'' and ``it'' are coreferring (see Figure~\ref{fig:tokens}).


% For each cluster, we added two unique coreference markers, which we inserted around each mention in the sentence. \ariec{Since coreference resolvers usually do not output singleton clusters (ie. cluster with only one mention), }
% %\ariec{you should elaborate here, what are the markers? how exactly we obtain those markers ``based'' on the coref resolvers. I know that the figure explains it but the text should be self contained and clearly describe the process.} 
% These tokens guide the model to associate the pronoun and the coreferring antecedent, aiding the model in generating a more consistent translation that is faithful%\ariec{is it the right term?}\asafy{aligned? can be confusing too.., faithful output with respect to the source sound right} 
% to source coreference clusters.

% %\oa{This section needs to be rewritten. The figure is helpful though. It should first state the approach in high level (that part is pretty much ok), then it should \textbf{formally} define the three procedures (and refer to the figure), then related work (that part is mostly ok)}
% In this section, we present a novel fine-tuning approach for improving coreference consistency \gabist{based on the observation that NMT models can quickly adapt}~\ariec{who observed? adapt to what? what's the relationship between the adapation and fine-tuning?}\gabis{agreed, I suggest to just remove that part, I think we can do without it}\citep{Freitag2016FastDA, saunders-byrne-2020-reducing}.
%  Specifically, we propose two methods\ariec{I still find it confusing to have ``\textbf{a} novel fine-tuning approach'', then ``\textbf{two} methods''. Maybe we can write from the beginning that we develop two novel methods for fine-tuning, explicit and implicit?}\gabis{+1} for fine-tuning MT models, which inject coreference signals either implicitly or explicitly.

% \ariec{Our first/implicit method....}
% Our motivation for this data augmention method stems from our analysis of our parallel dataset~\ariec{which parallel data? and which analysis? where did you show them?}, which showed that approximately one fifth of the sentences in it have coreference phenomena, hence enriching it with more examples of this phenomena can improve training of MT models with regard to coreference.~\ariec{but we don't add more examples with coref, we only remove other sentences that don't involve coref. We can write that since there are only a few instances with coref, when trained on the full data, the model learns more from the other examples and doesn't focus on coref.} Accordingly, we propose to fine-tune on a subset of the data\ariec{which data?}, with sentences that all contain coreference clusters \ariec{in the source-side}. Notice that in this setting, the inference remains standard.\ariec{do we need this sentence? When the readers arrive to this part, they won't think that the inference should be different}\gabis{$\uparrow$ Given all the comments here, I think we can just remove this paragraph, let's skip to saying what we actually do}


% %In the implicit approach,\oa{maybe a name for it?} we consider three steps for this adaptation problem. Filter parallel training data from instances that the source sentence does not contain coreference phenomena (as deemed by a coreference resolver),fine-tune the model on the filtered data, and inference with the enhanced models produced by adaptation.\oa{why is this three steps? inference is not part of it; you can just say we train only on a dataset that contains coreference phenomena.}\asafy{because in inference we insert coreference markers as well, not in the implicit approach but it maybe helpful to notice that those three steps are relevant to our method. }\ariec{I agree with Omri, these 3 steps are confusing because we describe them as new method for \textbf{fine-tuning} so actually even the second point is not relevant here, you should only say that before fine-tuning, we select sentences that contain coreferencec clusters. I also suggest to explain the motivation for this method: if you fine-tune an entire dataset for MT, only less than third of the sentences have coref, and models don't manage to learn well the task. We propose to fine-tune on a subset of the data, with sentences that all contain coref. Notice that in this setting, the inference remains standartd. }

% %Regarding data filtering, we took a parallel dataset and ran a coreference resolver on the source side sentences. Then we filter all the sentences that do not contain coreference clusters.\oa{how is that defined? at least two corefering mentions?} The filtered data we got overrepresents coreference phenomena. Such that fine-tuning MT models on that data will enhance their coreference capabilities.\oa{I would remove this paragraph and instead just write formally how the filtering works.}

% \ariec{isn't it obvious? maybe we can say in the previous paragraph that we use a coref model for that and in footnote the exact criterion of 2 coreferring mentions?}
% Our data filtering schema works as follows. We take parallel dataset, we run the coreference resolver on the source sentences.% For each sentence in $\mathcal{P}$, we get all the coreference clusters $CR$ identified. 
%  In cases where a sentence does not have coreference cluster, that is, if it does not have at least two coreferring mentions, we filter it out from the dataset. the outcome dataset overrepresents coreference phenomena.%\ariec{Too much detailed, no need for mathematical symbols, should be shortened.}
% Hence is more equipped to enhance coreference capabilities.% \ariec{see my comment above, I'd start by the motivation, maybe we can find citations that also support this finding} %for  MT models.


% \ariec{I think here again we should start with some motivation, something like: The implicit method is effective, but we want to go a step further and aid the model by specifying expressly the coreferring mentions. Then we will describe how we add markup given the coreference clusters.}
% In the explicit data augmentation method, we fine-tune the MT model with the same source sentences (i.e., same filtering method) augmented with coreference markup.\ariec{this is not really clear, what is coref markup? in the next sentence, you say markers, what's the difference between them?} We integrate those coreference markers based on the coreference resolver predication's (see Figure~\ref{fig:tokens}). For each cluster, we added two unique coreference markers, which we inserted around each mention in the sentence. \ariec{Since coreference resolvers usually do not output singleton clusters (ie. cluster with only one mention), }We added such markers only for clusters containing more than two mentions.
% %\ariec{you should elaborate here, what are the markers? how exactly we obtain those markers ``based'' on the coref resolvers. I know that the figure explains it but the text should be self contained and clearly describe the process.} 
% These tokens guide the model to associate the pronoun and the coreferring antecedent, aiding the model in generating a more consistent translation that is faithful%\ariec{is it the right term?}\asafy{aligned? can be confusing too.., faithful output with respect to the source sound right} 
% to source coreference clusters.

% %\ariec{it should be written that this is only for the ``explicit'' approach}
% During inference, we can add coreference markers to the evaluation dataset in two ways. The first is by using gold annotation if such coreference annotation is available. The second is by using the predictions of a coreference resolver, as used for creating the training data. These tokens utilize the explicit coreference signal inserted into the training data to direct the model towards translation where mentions within the same cluster have the same morphological gender.~\ariec{what's the purpose of this sentence?}
% %a direct signal to associate between antecedent and pronoun within the same cluster, assisting the model in translating coreferring antecedent and pronoun with the same morphological gender.\ariec{this repeats the last sentence of the previous paragraph, consider removing. }

% %After fine-tuning, when the models already trained to use those coreference markers as indication of antecedents in the same clusters. in inference time, we can add coreference markers based on coreference resolver predication's or gold annotation if such data is available. Giving the model direct signal to associate between antecedent and pronoun within the same cluster, helping it to translate them with the same morphological gender. 

% %we consider three steps that may benefit from such fine-tuning: fine-tuning the model on parallel data where the source sentences contain coreference phenomena (as deemed by a coreference resolver), incorporating explicit coreference signal into the data, and inference with the enhanced models produced by adaptation.
% %Additionally, to add explicit coreference signal we use coreference resolver predication's to integrate the source side sentences with coreference markers as demonstrated in Figure~\ref{fig:tokens}. Those tokens guide the model to associate the pronoun and the co-referring antecedent. Aiding the model in generating a more consistent translation that is faithful to source coreference clusters.


%\oa{general note: I think we're diving too quickly to the technical details here. We should start with the general notion of integrating information about coreference into the MT model's training data. We can say that we explore two ways of do so: (1) explicitly encoding it in the input; (2) filtering the data so as to overrepresent coreference phenomena. We should also briefly refer to prev work (if it's too long, we need to add it to another section and reference it from here.} 
%Previous method used Oracle(2 articals) and gender markers to improve co-reference to minimize gender biases by adding tokens to the source sentences.\oa{I didn't understand this sentence} In a similar fashion we enrich the source side sentences with co-reference markers.
%Guiding the model to associate between the pronoun and the co-referring antecedent (entity).

\begin{figure}[tb!]
\centering
\includegraphics[scale=0.31]{images/tokens.png}
\label{fig:method}
\caption{An example of adding coreference markers, given the prediction of a coreference model. Given an English sentence, we run a coreference resolver on it. The coreference resolver predicts the coreference clusters in the sentence. Then we add a markup to indicate mentions belonging to the same cluster. 
}
\label{fig:tokens}
\end{figure}

%Several previous methods aiming for improving coreference of MT models and reducing undesirable biases such as gender bias modified the training data in ways that shear some similarities with our method. \cite{vanmassenhove-etal-2018-getting} incorporate a ‘speaker gender’ tag into training data, allowing gender to be conveyed at the sentence level. Similarly, \cite{moryossef-etal-2019-filling} added a prefix to disambiguate the coreference in the sentence. \citep{stafanovics-etal-2020-mitigating}, train NMT models from scratch with all source language words annotated with target language grammatical gender. \citep{stojanovski-fraser-2018-coreference} advise oracle based approach to inject pronoun translation and its gender into the source sentence. In later research they combined this method with curriculum learning training \citep{stojanovski-fraser-2019-improving}. Our method is novel in the way it enrich the data with coreference signal using only source side and can be used with monolingual coreference model only without the need of annotated data. 

%Finally, in inference time we can add coreference markers based on model or gold clusters if available. Giving  the model direct signal to associate between antecedent and pronoun within the same cluster, helping it to translate them with the same morphological gender. 

%The method we use is reminiscent of other fine-tuning approaches to enhance model capabilities similarly to \citep{saunders-byrne-2020-reducing} that view fine-tuning as a domain adoption task.%\oa{in what sense are they similar?}
%Other lines of related work uses source-side sentences to reduce gender bias \citep{vanmassenhove-etal-2018-getting, stafanovics-etal-2020-mitigating, saunders-etal-2020-neural} or to improve coreference in MT \citep{ stojanovski-fraser-2018-coreference, stojanovski-fraser-2019-improving}, by appending them with explicit gender tokens and target pronoun tokens. However, to our knowledge, no previous work has used coreference annotation over the input to improve coreference capabilities in MT.


% In figure 2 we exemplified the way we incorporate the co-reference markers.
% Into the sentences. This method allows us to enrich the sentences with gold co-reference signal or a strong monolingual co-reference models signal.
% This way when we fine-tune the MT model it learns to associate mentions within the same cluster, helping it to translate them with the same morphological attributes.


%In our experiments we took parallel data and ran Kirshten model on the source side sentences. We then used the model prediction to incorporate co-reference markers into the source side sentences.When translating sentences in inference time we can enrich the sentences with both model or gold coreference signal, helping the model to produce consistent translation Our method incorporated source side signal allowing us to use it in both training and inference time.Differently, from other methods that incorporate target side signal prevent them to use their methods in inference time.

==> gabi_restructure/04_1_experimental_setup.tex <==
% %\oa{redundant} 
% In this section, we will first describe the evaluation datasets, MT models, target languages, and alignment model we use for our consistency evaluation~(§\ref{subsec:eval}). Then, we will detail the MT models and the training datasets we use for the improving coreference consistency experiments~(§\ref{subsec:improve_exp}).

% %\ariec{We need to better structure this section. I suggest to keep the order of the paper: (1) Evaluation -- datasets (explain that we only need english sentences with coref annotation and give example of each dataset to explain why we chose those), language and morpholigizer -- and (2) Models -- models (baseline, commercial and others) and training data } 

% %\ariec{consider adding an outline of the section in a style like ``We first describe the evaluation then how we improve. (should be rephrased of course)}

% \subsection{Evaluation}
% \label{subsec:eval}

% %\ariec{This section currently looks like a bunch of boring techincal details, I suggest to add an outline of the subsection and refer to the described method for each detail (see what I wrote for the word-alignment and morphological analyzer). BTW, we might consider modifying a bit the current flow and write the paper as a story, (1) eval description + experimental setting + results and (2) improving method + experimental setting + results. Because it's a lot of technical details that are not related one to each other. }


% %In a lot of cases a lexical translation of the source sentence will seem as it preserve the necessary constraints and provide an consistent translation. This is the reason we wanted to choose a challenging data sets aiming to investigate MT models ability in challenging scenario. 
% \textbf{Evaluation Dataset.} For evaluation, we use three challenging coreference annotated test data in English. Wino-X, WinoMT and BUG aims to measure coreference capabilities in both synthetic and naturalistic settings that require world knowledge.\ariec{consider removing, we explain these datasets in more details just below.}

% %\ariec{consider removing this sentence}
% % and gender understanding.\oa{what is gender understanding? find another term or remove}

% %focus on two major obstacle for coreference models, gender and world knowledge, in both syntactic and neutral setting.
% %In our study we mainly focus on gender agreement as a way to check the coreference consistency. Accordingly, we focus on two challenge sets. 



% The first dataset is Wino-X \citep{emelin-sennrich-2021-wino}, a subset of WinoGrande \citep{Sakaguchi2020WINOGRANDEAA} built to test commonsense reasoning and coreference resolution of MT models and multilingual encoders. The dataset contains sentences similar to the one in Figure~\ref{fig:method_new}. The pronoun in all the sentences is ``it'', and it refers to one of the two entities. The dataset consists of three parts, each part constructed for a different target language (German, French, and Russian). Each part of the dataset contains sentences from WinoGrande only if the two entities in the source sentence are expected to have different morphological gender in the target language.

% %contains sentences similar to the one appearing in Figure~\ref{fig:method_new}. The pronoun in all the sentences is ``it'', and it refers to one antecedent determined by the trigger word, in our example \example{small}. The dataset was designed such that each sentence translation has two antecedents of different genders. This design forces the tested model to select, which antecedent of the two the pronoun is referring to.\ariec{need rephrasing. Start by saying that Wino-X exists in 3 languages (ru, fr, de), then for each language, they choose a subset of english sentences with that desired property.}

% %filtered to contain only sentences where the two antecedent in the target language are of different gender. Wino-X is free of gender or positional bias. Solving the CoR is heavily depend on using common-sens reasoning and deploying world knowledge.
% The second dataset is WinoMT \citep{stanovsky-etal-2019-evaluating}, a dataset built following the Winograd schema \citep{Levesque2011TheWS}, designed to test gender bias and coreference resolution of MT models. The examples in this dataset contain two human~\ariec{is this important? I mean is it critical that readers will know that WinoMT is not all entities but human entities?} entities and one gendered pronoun as in this example: \example{The \textbf{doctor} asked the \textbf{nurse} to help \textbf{her} in the procedure}. In this setting, the gender pronoun reveals the gender of the entity and adds gender attributes to the source cluster. In our example, \example{her} refers to the \example{doctor}, revealing the doctor's gender.

% The third dataset is BUG \citep{levy2021collecting}, a semi-automatic collection of natural English sentences which are challenging with respect to societal gender-role assignments.~\ariec{I don't understand this sentence} Similar to WinoMT, each sentence contains a human entity, identified by their profession and a gendered pronoun. %As these sentences are more naturalistic, they can have many more unannotated antecedents and pronouns in each sentence.%
% % Due to the naturalistic nature\ariec{what is the naturalistic nature?} of these sentences and the way the dataset was constructed, the sentences may have a greater number of mentions and pronouns.\ariec{why this is important?}
% %For example, in the sentence \example{The \textbf{doctor} said \textbf{she} did not think the boy had SARS, but would treat it as such} there is a pronoun ,\example{she}, coreferring to one entity ,\example{doctor}, and other entity and pronoun (\example{boy} \example{it}). 
% Here we use the \textsc{Gold} portion of this dataset, which was validated by human annotators, in order to reduce noise in the evaluation.
% %\ariec{be more explicit and say we use the \textsc{Gold} portion of this dataset, which was validated by human annotators, in order to reduce noise in the evaluation.}
% %While both data sets require Cor information in order to translate the sentences accurately and constantly, the later opus\ariec{what do you mean?} other difficulty\ariec{I wouldn't call it other difficulty because performance is higher in BUG than in MT.} by coming from real-world distribution. 
% % the source side

% % We note that there are a few differences between these three datasets. Wino-X is a more challenging evaluation dataset as the model choice to connect the pronoun to its true antecedent is determined by the trigger word alone.\ariec{WinoMT also depends on a trigger word} WinoMT and BUG, on the other hand, contain stereotypical and unstereotypical examples designed to test for social and gender biases. These considerations are relevant to the challenge that each dataset presents, but are orthogonal to our comparison of MT models and coreference resolvers, as all models face the same challenging datasets.\oa{what do you mean ``all models share the same challenges''? can we remove this part?}\asafy{I rephrased it, what part did you meant?}\ariec{How important is this paragraph for the paper? I mean, what the readers loose if we remove this paragraph?}
% % We also note that BUG contains more neutral sentences that tend to be longer with possibly much more mentions.

% \noindent
% \textbf{Machine translation Models.} We apply our evaluation methodology on four transformers-based machine translation models from EasyNMT\footnote{https://github.com/Helsinki-NLP/Opus-MT}: the multilingual mBART50 \citep{https://doi.org/10.48550/arxiv.2008.00401, liu-etal-2020-multilingual-denoising} the multilingual M2M\_418M, M2M\_1.2B \citep{Fan2021BeyondEM}, and the monolingual
% Opus-MT~\citep{tiedemann-thottingal-2020-opus}, representing the state-of-the-art for publicly available neural machine translations models.
% %mBART50 is a one to many, multilingual translation model built on top of a pre-trained mBART. The inclusion of mBART50 follows the assumption that extensive pre-training may endow models with commonsense knowledge, as previously indicated for large-scale monolingual LMs \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}.
% %M2M model The Many-to-many (M2M) multi-language translation model can directly translate between set of 100 languages. After large-scale pre-training, different variants can be obtained. We use 418M and 1.2B models as strong baselines.
% %Opus-MT is based on Marian-NMT2 framework, a NMT with efficient training and decoding capabilities \citep{junczys-dowmunt-etal-2018-marian}. %Those models where trained on OPUS\footnote{\url{opus.nlpl.eu}}\citep{tiedemann-2012-parallel}, a large  parallel corpora.
% In addition, we measure coreference consistency on the output of two commercial systems: Google Translate\footnote{https://cloud.google.com/translate} and Microsoft Translator\footnote{https://www.bing.com/translator}. 

% \noindent
% \textbf{Target Languages.} We conduct our evaluation study on MT models translating from English to a set of six diverse target languages with grammatical gender: Arabic, German, Spanish, Hebrew, Russian and French.
% These languages have a variety of other linguistic characteristics (e.g., alphabet, word order, number of grammatical gender, or grammar), while still allowing for highly accurate automatic morphological analysis.%\ariec{is this sentence important?}
% These languages belong to four different families: (1) Romance languages: Spanish and French, which have gendered noun-determiner agreement; Spanish is also a pro-drop language.
% %\ariec{what is it? and what about other languages?} 
% (2) Slavic languages (Cyrillic alphabet): Russian; that have three grammatical genders (3) Semitic languages: Hebrew and Arabic, each with a unique alphabet; both are partial pro-drop languages. (4) Germanic languages: German, that also have three grammatical genders. %and is non pro-drop language.
% %\ariec{Consider merging this sentence with the previous ones, the names of languages are repetitive.}
% After translating the English sentences to these six languages, we obtain word-alignment between the source and target sentences (step 2) using awesome-align \citep{dou-neubig-2021-word}, a neural word aligner based on multilingual BERT. To extract the morphological gender of the aligned entity and the pronoun (step 3), we use spaCy\footnote{\url{https://spacy.io/}} for Spanish, French, Russian, and German, and Stanza~\citep{qi-etal-2020-stanza} for Hebrew and Arabic. 

% % \noindent
% % \textbf{Alignment.} We use awesome-align \citep{dou-neubig-2021-word}. A neural word aligner that extracts word alignments from multilingual BERT (mBERT).%It obtains robust performance in zero-shot settings.

% %\textbf{Coreference Resolution Models.} For comparison with SOTA coreference models we use the AllenNLP \citep{Gardner2018AllenNLPAD} implementation of SpanBERT \citep{Joshi2020SpanBERTIP} start-to-end (\emph{s2e}) model~\citep{Kirstain2021CoreferenceRW} and \textsc{LingMess}~\citep{Otmazgin2022LingMessLI}. SpanBERT introduces contextual span representation to the the e2e-coreference model to achieve state-of-the-art results on the English portion of the popular CoNLL-2012 shared task coreference benchmark \citep{pradhan-etal-2012-conll}.(\emph{s2e}) model is a more efficient model without span representation. \textsc{LingMess} ... \asafy{arie can you elaborate}.We use those models as the best current models for coreference resolution.

% \subsection{Improving Coreference Experiment}
% \label{subsec:improve_exp}

\noindent
\textbf{Machine translation.} In our fine-tuning experiments, we opted for the Opus-MT model, since its size (68M parameters) and efficiency \citep{junczys-dowmunt-etal-2018-marian}, enabled us to run extensive experiments across many languages. 

% We apply our fine-tuning method on Opus-MT model because it's 
%For fine-tuning we used Opus-MT models. Based on Marian-NMT2 framework, 
%Opus-MT is NMT with 
%efficient training and decoding capabilities \citep{junczys-dowmunt-etal-2018-marian} and .their 
%size (68M parameters) and efficiency \citep{junczys-dowmunt-etal-2018-marian} allow us to run extensive experiments on a large set of languages.
%\ariec{This paragraph is unclear, it should be ``We apply our fine-tuning method on XXX model because...''} 
\noindent
\textbf{Traning Datasets.}
For fine-tuning data of Spanish, French, and German, we use Europarl \citep{Koehn2005EuroparlAP}, and for Russian, Hebrew, and Arabic, we use CCMatrix \citep{Schwenk2021CCMatrixMB}. The CCMatrix dataset is very large (e.g., 140M sentences in English-Russian), due to limited computational resources, we randomly sample 5M sentences and use them for the following step. For each parallel dataset we find instances that require coreference resolution with the \emph{s2e} coreference resolver. We dub this data ``Coref data''. We add coreference mark up to the Coref data by using \emph{s2e} predictions (see Figure~\ref{fig:tokens}). See datasets statistics in App. \S\ref{sec:appendix:06_data_sizes}.
%on Europarl/CCMatrix source side (English) sentences. We then filter the sentences without coreference clusters. We daubed this data coref data. 
%Afterward, we filter the sentences where the coreference cluster didn't contain gender pronouns, we daubed this data gender-data.~\ariec{This filtering makes sense only for some datases (WinoMT and BUG) and it's not part of our method (we didn't write this filtering in the improving section) maybe we can move it to the results? }  %For comparison we randomly sample sentences in the same sizes of coref data and gender data from the original datasets. 
%\ariec{Again, you should refer to our two methods of fine-tuning.}
%To both coref data and gender data we add coreference markers as described in section \S\ref{sec:improving}.
%In addition, for training data of Spanish, French, and German we used Europarl \citep{Koehn2005EuroparlAP}, and for Russian, Hebrew and Arabic we use CCMatrix \citep{Schwenk2021CCMatrixMB}. 




==> gabi_restructure/04_2_results_and_discussion.tex <==
% %%%%%%%%% Compression of Consistency %%%%%%%%%
% \subsection{Consistency evaluation}
% % coref models:

% \ariec{arrange the start/first etc.}

% %\ariec{I rephrase, please see that it's OK}
% We \textbf{first} evaluate the performance of existing coreference resolvers on our three evaluation datasets (Wino-X, WinoMT and BUG). We select state-of-the-art models trained on CoNLL-2012~\citep{pradhan-etal-2012-conll}: SpanBERT \citep{Joshi2020SpanBERTIP}\footnote{We use the AllenNLP implementation~\citep{Gardner2018AllenNLPAD}.}, the \emph{s2e} model~\citep{Kirstain2021CoreferenceRW} and the very recent \textsc{LingMess} model~\citep{Otmazgin2022LingMessLI}.
% % For comparison~\ariec{Which comparison? it's not clear} with SOTA coreference models we use the AllenNLP \citep{Gardner2018AllenNLPAD} implementation of SpanBERT large \citep{Joshi2020SpanBERTIP}, the start-to-end (\emph{s2e}) model~\citep{Kirstain2021CoreferenceRW} and the very recent \textsc{LingMess} model~\citep{Otmazgin2022LingMessLI}. We use those models as they achieve state-of-the-art results on CoNLL-2012 coreference benchmark \citep{pradhan-etal-2012-conll}. 
% Results are shown in Table \ref{table:coref_models}.
% %We will use this table for comparison to consistncy scores of MT models throughout this section. 
% \input{tables/01_coref_models}

% % wino-x results:
% %\ariec{now that we combine the tables on Wino-X with WinoMT, it makes more sense to refer to the table once for both datasets, then you can write separetely the findings of each dataset.}

% Table~\ref{table:cons_gmf} shows the target-side coreference consistency scores for all baseline models, on the sentences from Wino-X and WinoMT. See Appendix \ref{sec:appendix:03_bug_results} for the results on BUG sentences. 

% We \textbf{start} by analyzing Wino-X results.
% \textbf{Firstly}, we notice that Wino-X is more challenging than WinoMT and BUG as all models, both coreference resolvers and MT models, perform poorly on Wino-X. The coreference resolvers average accuracy of Wino-X is $20\%$ less than the average accuracy of WinoMT.

% We \textbf{first} observe that coreference resolvers on average are more accurate on WinoMT than on Wino-X by more than $20\%$ .
% % We start by measuring the consistency results of MT models on Wino-X. We note that this dataset is exceptionally hard,\ariec{maybe use a softer expression?} such that SpanBERT achieves accuracy results that are hardly better than chance ($50\%$).\ariec{I'd write a simpler sentence, something like ``Wino-X seems more challenging that WinoMT and BUG as all models perform poorly on Wino-X.''} %, on associating the right antecedent with the pronoun. 
% %In this regard, we note that several languages, such as German and Russian have three grammatical genders, decreasing the random chance in our setting to $33\%$.\oa{so is the chance level 50\% or 33\%? or does this depend on the language? if it depends on the language, don't write in the prev sent that it's 50}
% %\oa{didn't understand the last sentence; what is the change level then in these cases? we should report chance level in all tables.}
% %Consistency results of commercial and open-source MT models on Wino-X provide an upper bound on the coreference accuracy of those models. It is noticeable that our baseline models lag behind supervised resolvers.
% %Table \ref{table:cons_gmf} shows The consistency results of commercial and open-source MT on Wino-X. 
% %The left side of Table \ref{table:cons_gmf} shows the consistency results of commercial and open-source MT on Wino-X. Results of MT models lag behind supervised resolvers even though consistency is a more forgiving measure.\ariec{consider repeating briefly why it's a more forgiving measure}
% Consistency results provide an upper bound for the source-side coreference accuracy of MT models since consistency only indicates coreference valuation and not accurate coreference assignment.
% The Consistency results of commercial and open-source MT models on Wino-X show those models lag behind supervised coreference resolvers.

% We notice that MT systems tend to produce translations where the pronoun does not carry gender. For example,  {\it cela}, {\it c'était} in French and \foreignlanguage{russian}{это,они} in Russian, meaning ``this'' or ``they'' in English.
% %\ariec{I changed to ``this'' because it can be confusing with the original ``it'' in the source sentence.} in English.
% Such translations avoid resolving the coreference as it is unclear to which entity the pronoun is referring to. Similarly, in German, the MT models tend to select the neutral pronoun ``es'' much more than the 
% male and female pronouns ``er'' and ``sie'' respectfully. \ariec{can you add some statistics of all these phenomena? Because now, it sounds like you pick a few examples and tell your observation...}
% % \input{tables/wino-x/02_Wino-x_gmf_con}
% % % wino-mt results:
% % \input{tables/wino-mt/03_consistency_gmf}
% \input{tables/2_cons_gmf_both}

% %Now, we move to discuss the evaluation of WinoMT. 
% We \textbf{start} by noting that in WinoMT we exclude translations where the candidate pronoun does not provide information on the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun. 
% See Appendix \ref{sec:appendix:04_models_exampels} for examples. 

% %Table \ref{table:cons_gmf} presents the consistency results on WinoMT. 
% Results on WinoMT suggest that consistency is affected by both MT model and target language. Regarding models, in most target languages Opus-MT performances are last, with average consistency of $59.3$. In contrast, mBART50 achieves consistently high results with average consistency of $70.5$, sometimes surpassing the second MT model by about 9 points. The cuase of this can be the extensive pre-training of mBART50, which may endow models with commonsense knowledge, as previously demonstrated for monolingual LMs \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}. similarly, Russian consistency results are systematically lower than the results in other languages. To demonstrate that we can observe that the best model in Russian provide lower results the the worst model in most other languages. In the opposite end, all model in German achieve consistency of about $70$ or more. This may be explained by German’s similarity to English \citep{Hawkins1986ACT} combined with the amounts of resources and research focus directing to improve English-German translation.

% Generally, results suggest that most tested systems across six tested languages perform quite poorly on our metric. The best consistency results( upper bound of source-side accuracy) in each language often does not match the accuracy of SOTA coreference resolvers. Two exceptions to this rule are the performances of mBART50 and consistency results in German. Specifically, mBART50 and Microsoft Translator achieve consistency results that are better than SpanBERT accuracy, although lower than \emph{s2e} and \textsc{LingMess}.

% %We first observe that coreference resolvers on average are more accurate on WinoMT than on Wino-X by more than $20\%$ .
% %\ariec{move that to afterwards, you first need to explain the results on WinoMT, then compare them to other results} 
% %We note that our consistency results are an upper bound on the coreference performance of the MT models.\ariec{But this is always the case, right?} We also note that here we exclude sentences where the pronoun does not provide information on the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun.

% % Our results suggest that most tested systems across six tested languages perform quite poorly on our metric.\ariec{can you write a range of performance? what do you mean by poorly? mbart obtains 75+ on some languages of WinoMT, it's not so poor...} The best performing model in each language often does not match the performance of SOTA coreference resolvers. An exception to this rule is in German, where mBART50 and Google Translate achieve better scores than SpanBERT.\ariec{Yes but SpanBERT is not so recent, these MT models are much more recent} This may be explained by German’s similarity to English \citep{Hawkins1986ACT} combined with the amounts of resources and research focus directing to improve English-German translation.\oa{so why does that mean it's more likely to work? I would just say that German is the language with the most resources and research focus, so it's likely it will score higher than others.}\asafy{I combined the two} Another interesting observation is that mBART50 achieves consistently high results compared to other models, sometimes surpassing the second MT model by 3 points. This may be attributed to the extensive pre-training of mBART50, that may endow models with commonsense knowledge, as previously indicated for large-scale monolingual LMs\ariec{is that verbatim?} \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}.

% \input{tables/lang_exampels}
% %We emphasize that our consistency measure can correctly identify a vast variety of different valid uses of pronoun in MT models output's.
% Previous automated metrics for pronoun translation struggled to identify valid translations that use different pronouns than the reference. Our method is agnostic to this problem as we look at consistency between entity and pronoun rather then exact match. To exemplify this finding in table \ref{table:exampels_improv}\asafy{TO DO}, we present a few translations that exhibit the use of less typical pronouns
% that differ from the gold pronoun ( giving in Wino-X).Moreover, previous methods focused on non-pro drop languages like German and French where the candidate pronoun is mostly pronoun too. In partial pro-drop languages like Hebrew and Arabic, there are cases where the information of the pronoun can encode into a verb or a noun. Our methodology can account for such cases by reeling on the gender agreement between the candidate entity and candidate pronoun even though the candidate pronoun belongs to a different part of speech. Such examples also appear in \ref{table:exampels_improv}. \asafy{TO DO}
% In addition, figure \ref{}\asafy{TO DO} we present the part of speech distribution of the candidate pronoun. We emphasize that this capability is a clear advantage of our methodology compared to previous automatic metrics for pronoun translation.

% % and examples where the candidate pronoun is a noun or a verb that expresses the pronoun gender. We note that identifying valid pronoun translations is a known problem in the field of pronoun translation that mostly focuses on non-pro drop languages like German and French. Here we show that our methodology can handle even partial pro-drop languages like Hebrew and Russian or null-subject languages like Arabic.

% % We emphasize that while the way in which pronouns are used varies between translations, our consistency measure identifies a wide range of valid translations.\oa{didn't understand the last sent}\asafy{I rephrased the sentence}\ariec{it's still not clear. You should explain the phenomenon of multiple valid translations, then say that our method is agnostic to this problem as we look at consistency between entity and pronoun} To exemplify this finding in table \ref{table:exampels_improv}\ariec{I don't see the table.}, we present a few translations that exhibit the use of less typical pronouns or use inflection to nouns or verbs to convey the pronoun gender.\ariec{not clear, you should give an example (either here or in a table) of an english sentence with expected translation and another valid translation that changes the gender of the entity or the pronoun.} We note that identifying valid pronoun translations is a known problem in the field of pronoun translation that mostly focuses on non-pro drop languages like German and French. Here we show that our methodology can handle even partial pro-drop languages like Hebrew and Russian or null-subject languages like Arabic.\ariec{some of these terms weren't define above, assume that people don't know what is a null-subject or a partial pro-drop} In figure \ref{} we present the part of speech distribution per language of the candidate pronoun.\ariec{this sentence is out-of-context, you should explicitly say that this is an advantage of our method compared to pronoun translation.}


% % When translating the English pronoun we observe that  
% % Applying our method on set of six diverse languages give rise to the morphological differences between them. Specifically, the way different 
% % A known challenge of previous works is the shortcoming regarding the ability to identify valid alternative translations.
% % consistency instead of exact matches allowing us to treat a range of valid alternative translations and observe model behavior when encountering coreference resolution phenomena.
% % We want to emphasis that our method is able to identify vast variety of valid translation. In order to exemplified our 
%%%%%%%%% Improvement of Consistency %%%%%%%%%
% wino-x improvement:
% \subsection{Improving Consistency with Fine-tuning}
% \input{tables/wino-x/04_Wino-x_ours_con}
\input{tables/3_cons_ours_both}

Table~\ref{table:cons_ours} shows the target-side coreference consistency scores for our fine-tuning approach, on Wino-X and WinoMT.
%We present experiments in which we apply the approach detailed in Section \ref{sec:improving} to improve the consistency of MT models. 
We present results for our baseline model, Opus-MT, and our two fine-tuning approaches (detailed in Section \S\ref{sec:improving}) applied to two sets of augmented datasets. The first dataset is Coref dataset. The second dataset is the Gender dataset, a subset of the Coref data, contains only sentences with coreference phenomena that involve gender pronouns. This dataset aims to address the characteristics of WinoMT and BUG evaluation datasets, where most sentences use gender pronouns. For each fine tuning data, we apply both our fine-tuning approaches, and use both predicted and gold markers at inference time. See App. \S\ref{sec:appendix:03_bug_results} for the performance on BUG.

Results suggest that performances on Wino-X are generally better when fine tuning on Coref data and WinoMT results are better when fine tuning on Gender data. These results can indicate that the model's improvement depends on the specific coreference phenomena that it is exposed to in training,
%Coref data is unequivocal more beneficial for improvement on Wino-X than Gender data.
notably, the lack of sentences containing coreference with the pronoun ``it'' in Gender data. Coref data is also helpful for increasing performance on WinoMT, although in most cases it provides a more moderate improvement compared with Gender data.  This result is aligned with the observation of \citet{saunders-byrne-2020-reducing}, that smaller, more goal-oriented data is better for fine-tuning.

In most of our experiments, 14 out of 18, the explicit approach of fine tuning was found to be more beneficial than the implicit data augmentation approach when using the same data (Coref or Gender data). These results suggest that an explicit monolingual signal can improve results more than an implicit signal.

Results also show that improvement is more pronounced when incorporating gold coreference markers instead of predicted markers. Although these results hold for both Wino-X and WinoMT, its effect is more noticeable in Wino-X. This is likely because of the low accuracy ,about $ 60\%$, of \emph{s2e} model on Wino-X, effecting the quality of the added mark ups. In comparison, \emph{s2e} achieved more than $ 80\%$ accuracy on WinoMT. Moreover, this model was found to generate fewer translations on Wino-X where the pronoun does not carry gender ($8\%$ on average).

%Our approach\oa{dont call it that; say something like the Opus-MT when fine tuned on ..} attain comparable or better results than top commercial and much bigger open-source MT models. Specifically 
Applying our fine-tuning with gold coreference markers outperforms all other baseline MT models in German and Russian on both Wino-X and WinoMT, and achieves comparable results in all other target languages.

\input{tables/exampels_improvment}

In Table \ref{table:lang_exampels} we show an example where our approach improves translation consistency and quality. We note that these fine tuning procedures only have a minor effect on BLEU results (see results on App. \S\ref{sec:appendix:02_bleu_results}).

%Regarding fine tuning with explicit coreference markers compared with the implicit data augmentation method, we find that on most our experiments, 15 out of 18, the explicit fine tuning was found to be more beneficial. 
% We present experiments in which we apply the methods detailed in Section \ref{sec:improving} to improve the consistency of MT models. We start by analyzing our Wino-X experiments.\ariec{again -- since we unfiy the table, say that the table shows results for both dataset (add also a reference to the appendix for the results on BUG), then you can analyze them separetely or together, here it makes more sense to analyze them together as some findings (e.g predicted vs. gold markers) are similar for both datasets} In Table \ref{table:cons_ours} we present three sets of experiments. We apply our implicit and explicit fine-tuning approaches with both coreference\ariec{you mean predicted?} and gold markers on coref data and gender data.\ariec{this sounds like 2x2x2 experiments.. See also my comment in the improving section about the gender data}

% \ariec{the flow is not good, it looks like a concatenation of independent sentences. Compare the results in that explicit order (1) coref vs. gender data (Wino-X and WinoMT behave differently), (2) implicit vs. explicit approach (same for Wino-X and WinoMT), (3) predicted vs. gold}
%, leading to substantial gains in German and French

%Noticeably, the results are better when we use coref data as the pronoun ``it'' is lacking from gender data. Fine-tuning on coref data improves the models substantially in German and French. Moreover, fine-tuning with coreference markers provides additional improvement. Improvement is more pronounced when using gold coreference markers as the accuracy of \emph{s2e} on Wino-X is quite low (about $ 60\%$). Applying our fine-tuning with gold coreference markers improves over the baseline and outperforms all other commercial and open-source MT models in German and Russian.

% wino-mt improvement:
%Table \ref{table:cons_ours} present our consistency results on WinoMT. Here, we notice that most models fine-tuned on gender data perform better on WinoMT than ones trained on coref data. This result aligned with the observation of \citealt{saunders-byrne-2020-reducing}, that smaller more goal-oriented data is better for fine-tuning. We also observe that gold markers get smaller improvements than the improvements we saw in WinoMT as coreference resolvers achieve higher accuracy on WinoMT.\ariec{This is likely because of the high performance of the \emph{s2e} model on WinoMT} Our approaches achieves comparable or better results than top commercial and much bigger open-source MT models.\ariec{e.g XX vs. XX} In Table \ref{table:lang_exampels} we show examples where our approach improve translation consistency and quality. We note that our fine tuning has only minor effect on BLEU results (see results on App. \S\ref{sec:appendix:02_bleu_results}).\ariec{This is a really important point which is not related to WinoMT, maybe you can add a paragraph for that. }
% \input{tables/wino-mt/05_consistency_ours}

%Another evaluation study we did for estimating the improvement of our method
%\ariec{Move this paragraph after all the consistency results and add a subsection}

% In the first one, we fine-tuned our MT model on data with coreference phenomena, enriching the model with an implicit signal. In the second, we use our explicit approach of fine-tuning our MT model on the same data enrich with \emph{s2e}'s coreference markers. Then we use \emph{s2e} to produce coreference markers for evaluation data too. For the third experiment, we use the same fine-tuned MT model as in the second, but gold coreference markers are used in inference time.\oa{you should not repeat the description of these methods. just mark them with names and say here that we report results with them.}

%Results show that our method greatly improves consistency results across all languages. Outperforms all other MT models in German and Russian.%\oa{what outperforms what?} Fine-tuning on coreference data improves the models substantially in German and French. Moreover, Fine-tuning with coreference markers provides additional improvement. Improvement is more pronounced when using gold coreference markers as the accuracy of \emph{s2e} on Wino-X is quite low (about $ 60\%$).

\subsection{Other Evaluation Analysis}

We now turn to observing the empirical effect of the suggested fine-tuning, using %previously proposed 
additional metrics.
For each sentence in Wino-X, we have the gold target pronoun that should appear in its translation. We use it to compute pronoun translation accuracy by comparing the candidate pronoun with the gold target pronoun. Table \ref{table:ours_pm_winox} presents the results. We can see that our method provides a large improvement over the baseline. Comparing these results against those of prominent open-source and commercial MT (see App. \S\ref{sec:appendix:01_gmf_pm}) will show that our approach outperforms other MT models in German and Russian, and it is only second to mBART50 in French.
%\oa{I would make this a paragraph in the prev section}\asafy{not sure i understand what you meant by that, the opening or discard the new subsection title? or other alternative?}

%This section evaluates the impact of the fine-tuning methods on improving coreference performance according to previously proposed evaluation metrics.%\oa{is this true?}\asafy{it somewhat similar, see the two first sentences of the abstract here: https://aclanthology.org/W17-4802.pdf, still it sufficiently different that we can present it as sanity check or other measurement we add} In Wino-X we have a gold target pronoun annotated in the dataset. We use it to compute pronoun translation accuracy by comparing the candidate pronoun with the gold target pronoun. Table \ref{table:ours_pm_winox} presents the results. We can see that our method provides a large improvement over the baseline. Comparing these results against those of prominent open-source and commercial MT (see Table in App. \S\ref{sec:appendix:01_gmf_pm}) will show that our approach outperforms other MT models in German and Russian, and it is only second to mBART50 in French. % which surpasses all other models by a large margin. 
In WinoMT, \citet{stanovsky-etal-2019-evaluating} computed {\it gender accuracy}, as the percentage of instances in which the translation preserved the gender of the entity from the original English sentence. Table \ref{table:ours_acc_wino-mt} shows that our approach improved gender accuracy results across all languages except Arabic.%\ariec{e.g +XX, +XX}

%\ariec{It's not other measures, but more a drill down to the gender accuracy}
Other metrics that \citet{stanovsky-etal-2019-evaluating} used, are $\Delta S$ and $\Delta G$. $\Delta S$, measure the difference in gender accuracy between stereotypical and non-stereotypical gender role assignments (as defined by \citealp{zhao-etal-2017-men}), and $\Delta G$ measure the difference in performance (F1 score) between source sentences with male and female entities. Our method decrease $\Delta S$ and $\Delta G$ by $5-6$ points on average, indicating that adding explicit signal can also help the model associate the pronoun with the coreferring entity, even in the presence of social and gender biases.

% \subsection{Human Validation}

% We estimate the accuracy of our consistency evaluation method by randomly sampling 50 translations of the Opus-MT model from all evaluation datasets and in all target languages, annotating each sample by a target language native speaker. The human annotators were asked to identify if the candidate pronoun is indeed the target pronoun and to verify is the gender prediction is correct. This way, we can account for both types of possible errors, i.e., alignment and gender extraction. 
% We compare the sentence-level human annotations to the output of our automatic method and find that the average agreement over all languages and datasets is above $90\%$ ( see full human validation results in Appendix \ref{sec:appendix:05_human_validation_results}). In the research of \citealp{stanovsky-etal-2019-evaluating} they used human validation to show that the alignment and gender prediction of the entity are reliable for $85\%$ of translations across all languages.%\ariec{what's the purpose of this sentence?}
% %\oa{this sentence is unclear; in what setting did they show it?}
% %Based on the combination of \citep{stanovsky-etal-2019-evaluating} with our evaluation we can safely say that our alignment and gender prediction are reliable. 
% From the combination of these two results we can conclude that our consistency scores are reliable.

% As \citealp{stanovsky-etal-2019-evaluating} noted, some errors occur when language-specific idiosyncrasies%\ariec{I don't know this word, what does it mean?} 
% introduce ambiguity to the morphological analysis. For example, gender for certain words in Hebrew cannot be distinguished without diacritics, and some pronouns in German are used in both masculine and neutral (e.g., sein) or feminine and third-person plural (e.g., ihr) forms. In addition, we notice that BUG sentences, specifically in partial pro-drop languages, were found to be more challenging for the alignment model~\ariec{can you explain why?}, and found to account for most mistakes in Hebrew and Arabic. This can be explained by the combination of noise in BUG sentences and the way that the pronoun is translated in partial pro-drop languages.
% %\ariec{I don't understand the purpose of this paragraph, if it's an analysis of the errors for each dataset, you should support these statements with numbers. }
% %\oa{I don't understand this sentence. you mean that the agreement on BUG was considerably higher than on the Winos? if so, say that}

%\input{tables/wino-x/Wino-x_gmf_pm}
\input{tables/wino-x/06_Wino-x_ours_pm}


\input{tables/wino-mt/07_acc_ours}

% \input{tables/Wino}
% \input{tables/BugGold}

==> gabi_restructure/05_Related_Work.tex <==
The study of coreference has a long tradition in machine translation.
%However, the way to evaluate Cor is nontrivial and varies from work to work. 
%\ariec{This section should be shortened, the goal is to position our work with the literature, we don't need to know the exact details of each paper. Also, it should end by a sentence like ``our work is the first ...''}
A long line of work uses pronoun translation as a way of measuring coreference, since BLEU-based evaluation was shown to be insufficient for measuring improvement in coreference \citep{hardmeier-federico-2010-modelling}.
% Works that still used BLEU, used sentences with coreference for test data \citep{stojanovski-fraser-2018-coreference, voita-etal-2018-context}.
%\oa{I don't understand this sentence. Please split it into two and explain what you mean  by 'modifying or filtering test sentences}

An alternative evaluation methodology is using automatic reference-based methods that produce a score based on word alignment between the source, reference translation, and translation output, and identification of pronouns in them, such as AutoPRF \citep{hardmeier-federico-2010-modelling} and APT~\citep{miculicich-werlen-popescu-belis-2017-validation}. 
Nevertheless, a later human meta-evaluation showed substantial disagreement between these metrics and human annotators, especially because of the existence of valid alternative translations and pronouns than the ones used in the reference \cite{guillou-hardmeier-2018-automatic}. % from those found in the reference.
%These conclusions led to scoring-based evaluation approach \citep{sennrich-2017-grammatical}, that works by creating contrasting pairs and comparing model scores.
Based on these conclusions, \citet{sennrich-2017-grammatical} developed a scoring-based evaluation approach that compares model scores of a predefined set of correct and incorrect translations and evaluates how often the model selects the correct option. 
%correct translation
%\oa{I don't understand what this means; rephrase}\asafy{any better?}\ariec{no} Accuracy is defined as how often the model selects the
%correct translation from a pool of alternative incorrect translations.

Our method extends \citep{stanovsky-etal-2019-evaluating}, which used a reference-free approach by aligning the source and candidate translation, but focused on entity translation accuracy to evaluate gender bias in MT models.
The availability of references was assumed by most previous work \citep{guillou-hardmeier-2016-protest, bawden-etal-2018-evaluating, muller-etal-2018-large, stojanovski-etal-2020-contracat, emelin-sennrich-2021-wino}, where most of them are limited to a single language pair. 
%\ariec{What the purpose of this sentence?}  % as well as in size (a few hundred examples).
The flexibility afforded by a reference-free approach allows us to evaluate any target language for which an alignment model and morphological analyzer are available. Moreover, our approach is not restricted by a predefined set of translations and can also correctly detect valid translations that are different from the reference.

% On the one hand, reference-based metrics tend to miss valid alternative translations that differ from the reference. On the other hand, approaches that rely on correct and incorrect examples, are confined to a small set of examples. In our reference-free approach, we do not suffer from those shortcomings. We are not restricted by a predefined set of translations and we can correctly detect valid translations.\oa{This sentence is very unclear. You need to explain the difficulty with using reference-based translations in terms of multiple valid translations, and then say that a reference-free approach does not suffer from this shortcoming.}\asafy{I rephrase these few sentences}

Several previous methods aimed to improve the coreference abilities of MT models and reduce undesirable biases, by modifying the training data in ways that share some similarities with our method. \citet{vanmassenhove-etal-2018-getting} incorporate a ``speaker gender'' tag into training data, allowing gender to be conveyed at the sentence level. Similarly, \citet{moryossef-etal-2019-filling} added a prefix to disambiguate the coreference in the sentence. %\citet{stafanovics-etal-2020-mitigating} train NMT models from scratch with all source language words annotated with target language grammatical gender.
\citet{stojanovski-fraser-2018-coreference} used oracle-based approach to inject new tokens indicating the pronoun translation and its gender into the source sentence. %In later research, they combined this method with curriculum learning training \citep{stojanovski-fraser-2019-improving}. 
Our method is novel in the way it enriches the data with coreference signal using only the source-side signal, and thus requires only an English coreference resolution model without the need for coreference annotation in the target language.

%add token representing the gender of the speaker.  

% 1
% A notable different approach focus on scoring-based evaluation (Sennrich, 2017), which works by creating contrasting pairs and comparing model scores. Accuracy is calculated as how often the model chooses the
% correct translation from a pool of alternative incorrect translations.

% Alternatives to bleu include F1, partial credit, and oracle-guided approaches (Hardmeier and Federico, 2010; Guillou and Hardmeier, 2016; Miculicich Werlen and Popescu-Belis, 2017).
% However, Guillou and Hardmeier (2018) show that these metrics can miss important cases and
% propose semi-automatic evaluation. In contrast, our evaluation is completely automatic.

% % In the past, several CoR datasets have been proposed for 
% Many of those works proposed datasets for evaluating and testing Cor in MT \citep{guillou-hardmeier-2016-protest, bawden-etal-2018-evaluating, muller-etal-2018-large, stojanovski-etal-2020-contracat, emelin-sennrich-2021-wino}. Most of them are limited to a single pair of languages (e.g EN-DE, EN-FR) as well as in size (few hundreds examples). Among those, that of \citep{emelin-sennrich-2021-wino} is the most similar to our work as they address multiple target languages and used data that require the model to use world knowledge to resolve the Cor. In contrast, our method allows evaluating each target language without any parallel data, on both synthetic and natural data.  

% One of the clear 
% Our method is similar to the work done by \citep{stanovsky-etal-2019-evaluating}, evaluating aspects of MT models by the morphological attributes of their translations. Our focus is to asses Cor of model and no 


==> gabi_restructure/06_conclusion.tex <==
Our work is the first to present an automatic methodology for assessing the coreference capabilities of MT models that can be applied in any target language and do not require any target side annotations. Furthermore, we are the first to conduct a large-scale multilingual coreference evaluation study on prominent open-source and commercial MT models, and compare them against SOTA coreference resolvers on three challenging benchmarks. Finally, based on the superior results of SOTA coreference resolvers, we propose a novel approach to improve coreference capabilities of MT models, that outperform or achieve comparable results to strong baselines.
%\oa{in what cases is it comparable?}
% We introduced a new evaluation methodology for coreference consistency in translation. Our methodology leverages the grammatical constraint that each mentions in the generated translation need to agree upon their morphological attributes, specifically gender. This measure allows us to provide an upper bound on the ability of MT models to perform coreference and enable a fair comparison of MT models and SOTA coreference resolvers. We evaluate several prominent open-source and commercial MT systems, translating from English to six target languages, and compare them to SOTA coreference resolvers on three challenging benchmarks. Our results showed that SOTA coreference resolvers are considerably better. Based on that result, we advise two novel fine-tuning approaches, for injecting coreference signals into MT models either implicitly or explicitly, using coreference resolvers. Our experiments showed that applying these approaches can provide compelling gains in consistency, as well as in other measures.\ariec{this looks like the abstract, it should be far much shorter}

In future research, we will expand our approach to account for number and person agreement phenomena. We will investigate how to extend our approach to more coreference clusters and more mentions per cluster in intra-sentential as well as inter-sentential settings. Moreover, we intend to investigate how different morphological attributes affect MT models' coreference abilities.%\ariec{I don't understand this sentence.} 


%further research
% broader understating of the unique morphological effect on different languages
% extend to other attributes and more mentions
% extend our method to new domains

==> gabi_restructure/08_limitation.tex <==
% We note that intrinsic limitation of our evaluation methodology is regarding the ability to treat pro-drop languages.
% In pro-drop languages like Spanish, the pronoun can be drooped without any other morphological indication to it's gender. In such cases, for sentences in WinoMT and BUG the only indication regarding the way the MT models understand the coreference relations in the source side is by the gender inflection of the profession.\ariec{in the paper, we didn't say that, we manage to evaluate consistency on these languages, while accuracy is a different measure.}
% - human validation of consistency as a whole.\ariec{??}

Even though our study presents the first large-scale multilingual coreference evaluation study in MT, it still has some limitations that could be addressed in future work. First, our methodology provides an upper bound to the coreference capabilities based on detecting gender valuations. While this could allow for a  controlled evaluation experiment, this upper bound can become not indicative in cases where gender assignment is not a discriminative factor. This can be addressed by accounting for more semantic and syntactic constraints that the translation needs to follow. Second, in our setting, we treat one entity and co-referring pronoun in the naturalistic sentences experiment. Ideally, our methodology could be augmented to deal with more coreference clusters and more mentions per cluster. With such enhancements, we would be able to deal with naturalistic sentences in a similar manner to that of coreference resolvers. Finally, even though in Section \ref{sec:improving} we show big gains in results by our fine-tuning approach, it is clear that there is much more room for improvement for the coreference capabilities of MT models, especially with regard to the performances of SOTA coreference resolvers. We hope that this work will help others to develop MT models with better coreference capabilities.


==> gabi_restructure/99_defs.tex <==
\newcommand{\winox}[0]{Wino-X}
\newcommand{\winomt}[0]{WinoMT}
\newcommand{\bug}[0]{BUG}

==> gabi_restructure/obsolete/03_1_evaluation_experiments.tex <==
%%%%%%%%% Compression of Consistency %%%%%%%%%
% \subsection{Consistency evaluation}

% coref models:
%\gabis{This is a rather long subsection - can you summarize what are its findings? can you maybe higlight them in the text, e.g., using the paragraph command?}


We first evaluate the accuracy of existing coreference resolvers on our three evaluation datasets (Wino-X, WinoMT and BUG), where accuracy is defined as the percentage of instances in which the model identifies that the pronoun is coreferring with the correct entity.
We select state-of-the-art models trained on CoNLL-2012~\citep{pradhan-etal-2012-conll}: SpanBERT \citep{Joshi2020SpanBERTIP}\footnote{We use the AllenNLP implementation~\citep{Gardner2018AllenNLPAD}.}, the start-to-end (\emph{s2e}) model~\citep{Kirstain2021CoreferenceRW} and \textsc{LingMess} model~\citep{Otmazgin2022LingMessLI}.
Accuracy results are shown in Table \ref{table:coref_models}. 

\input{tables/01_coref_models}

We find that \textbf{Wino-X} is more challenging than WinoMT and BUG, as all models perform quite poorly on Wino-X. Specifically, the average accuracy of coreference resolvers on Wino-X is $20\%$ lower than on WinoMT. 

% consistency results:
Table~\ref{table:cons_gmf} shows the target-side coreference consistency scores for all baseline models, on the sentences from Wino-X and WinoMT. %See Appendix \ref{sec:appendix:03_bug_results} for the results on BUG sentences.\gabis{I don't thinkt that this is a valid reference. Can you at least explain what trends we see there?}\asafy{similar ones}
The consistency results of commercial and open-source MT models on Wino-X show that these models score notably lower than accuracy of supervised coreference resolvers, indicating that the coreference capabilities of MT models are inferior. 

We notice that when MT models translate Wino-X sentences they tend to produce translations where the pronoun does not carry gender. For example,  {\it cela}, {\it c'était} in French ($31\%$ of translations) and \foreignlanguage{russian}{это,они} in Russian ($17\%$ of translations), meaning ``this'' or ``they'' in English.
%\ariec{I changed to ``this'' because it can be confusing with the original ``it'' in the source sentence.} in English.
Such translations avoid resolving the coreference as it is unclear which entity the pronoun is referring to. Similarly, in German, the MT models tend to select the neutral pronoun ``es'' much more than the 
male and female pronouns ``er'' and ``sie'' respectfully. Concretely, $68\%$ of translations have neutral pronouns, although only $22\%$ of the candidate entities are neutral. The reported percentages were calculated on Opus-MT. Similar trends were observed in all models.  
% \input{tables/wino-x/02_Wino-x_gmf_con}
% % wino-mt results:
% \input{tables/wino-mt/03_consistency_gmf}
\input{tables/2_cons_gmf_both}

%Now, we move to discuss the evaluation of WinoMT. 
In \textbf{WinoMT} evaluation we exclude translations where the candidate pronoun does not provide information about the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun. 
See App. \S\ref{sec:appendix:04_models_exampels} for examples. 

%Table \ref{table:cons_gmf} presents the consistency results on WinoMT. 
Results on WinoMT suggest that consistency is affected by both the MT model and the target language. Regarding models, in most target languages Opus-MT performances are the lowest, with average consistency of $59.3$. In contrast, mBART50 achieves consistently high results with average consistency of $70.5$, sometimes surpassing the second MT model by about 9 points. The reason for this can be the extensive pre-training of mBART50, which may endow models with commonsense knowledge, as previously demonstrated for monolingual LMs \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}. Similarly, Russian consistency results are systematically lower than the results in other languages, to the extent that the best model in Russian provides lower results than the worst model in most other languages. On the opposite end, all models in German achieve consistency of about $70$ or more. There are likely to be several reasons for this, including German's similarity with English and the research focus on improving English-German translations. 

Generally, results suggest that most tested systems across the six tested languages perform quite poorly on our metric. The best consistency results (which are an upper bound of source-side accuracy) in each language often does not match the accuracy of SOTA coreference resolvers. Two exceptions to this rule are the performances of mBART50 and consistency results in German. Specifically, mBART50 and Microsoft Translator achieve consistency results that are better than SpanBERT accuracy, although lower than \emph{s2e} and \textsc{LingMess}.


We present \textbf{BUG} consistency results in App. \S\ref{sec:appendix:03_bug_results}. Consistency results on BUG tend to be higher than WinoMT results. One explanation can be the absence of distracting entity as the one used in Wino-X and WinoM. This difference can lead to higher consistency results for lexical one-to-one translations.

It may be attributed to the absence of distracting entities such as in the syntactic Wino-X and WinoMT, which can lead to higher consistency for lexical one-to-one translations.
%We first observe that coreference resolvers on average are more accurate on WinoMT than on Wino-X by more than $20\%$ .
%\ariec{move that to afterwards, you first need to explain the results on WinoMT, then compare them to other results} 
%We note that our consistency results are an upper bound on the coreference performance of the MT models.\ariec{But this is always the case, right?} We also note that here we exclude sentences where the pronoun does not provide information on the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun.

% Our results suggest that most tested systems across six tested languages perform quite poorly on our metric.\ariec{can you write a range of performance? what do you mean by poorly? mbart obtains 75+ on some languages of WinoMT, it's not so poor...} The best performing model in each language often does not match the performance of SOTA coreference resolvers. An exception to this rule is in German, where mBART50 and Google Translate achieve better scores than SpanBERT.\ariec{Yes but SpanBERT is not so recent, these MT models are much more recent} This may be explained by German’s similarity to English \citep{Hawkins1986ACT} combined with the amounts of resources and research focus directing to improve English-German translation.\oa{so why does that mean it's more likely to work? I would just say that German is the language with the most resources and research focus, so it's likely it will score higher than others.}\asafy{I combined the two} Another interesting observation is that mBART50 achieves consistently high results compared to other models, sometimes surpassing the second MT model by 3 points. This may be attributed to the extensive pre-training of mBART50, that may endow models with commonsense knowledge, as previously indicated for large-scale monolingual LMs\ariec{is that verbatim?} \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}.

% \input{tables/exampels_improvment}
%We emphasize that our consistency measure can correctly identify a vast variety of different valid uses of pronoun in MT models output's.


\paragraph{Advantages of our Methodology.} 

% Advantages of our methodology: this paragraph looks like a related work section, which shouldn't be here. What do we want to enumerate as advantages? I can think of (1) we can capture a wide range of pronouns, including different POS, (2) our method doesn't require annotated data for coreference in the target languages. Then in related work, we will compare to pronoun translation etc



There are two important advantages in our evaluation methodology. First, while requiring only source-side  coreference annotation, our method can be used for evaluating the coreference capabilities of any MT model when translating from English to a wide range of target languages, for which a morphological analyzer is available. \ariec{I'll complete later}





% \textbf{Advantages of our methodology.} 
% Previous automated metrics for pronoun translation struggled to identify valid translations that use different pronouns than the reference. Our method is agnostic to this problem as we look at consistency between entity and pronoun rather than exact match. To exemplify this finding in Table \ref{table:lang_exampels}, we present a translation that exhibits the use of less typical pronouns
% %or that differ from the gold pronoun (provided by Wino-X)
% (see more examples in App. \S\ref{sec:appendix:04_models_exampels}). Moreover, previous methods focused on non-pro-drop languages like German and French where the candidate pronoun in the target language are pronoun. In partial pro-drop languages like Hebrew and Arabic, there are cases where the information of the pronoun can be encoded into a noun or other part of speech. Our methodology can account for such cases by relying on the gender agreement between the candidate entity and candidate pronoun, even though the candidate pronoun has a different part of speech. Such examples also appear in App. \S\ref{sec:appendix:04_models_exampels}.
% In addition, Figure \ref{fig:pron_dis} shows the parts of speech (POS) distribution of the candidate pronoun for the candidate pronoun of Opus-MT in Hebrew, where we filter rare POS that appear less than once.%  We emphasize that this capability is a clear advantage of our methodology compared to previous automatic metrics for pronoun translation. sec:appendix:03_bug_results

% figure 2
\begin{figure}[tb!]
\centering
\includegraphics[scale=0.35]{images/myplot_new_font.png}
\caption{The distribution of parts of speech for the candidate pronoun of Opus-MT in Hebrew.}
\label{fig:pron_dis}
\end{figure}

==> gabi_restructure/obsolete/03_2_Human_Validation.tex <==
To assess our evaluation methodology, we randomly sampled 50 translations of the Opus-MT model from all evaluation datasets and in all target languages, annotating each sample by a target language native speaker. The human annotators were asked to identify if the candidate pronoun is indeed the target pronoun and to verify that the gender prediction is correct. This way, we can account for both types of possible errors, i.e., alignment and gender extraction. 
We compare the human annotations to the output of our automatic method and find that the average agreement over all languages and datasets is above $90\%$ (see full results in App. \S\ref{sec:appendix:05_human_validation_results}). These results are comparable to the ones reported by \citet{stanovsky-etal-2019-evaluating}, who conduct human validation and report that their alignment and gender prediction of the entity in question are reliable for $85\%$ of translations across all languages. %\ariec{what's the purpose of this sentence?}
%\oa{this sentence is unclear; in what setting did they show it?}
%Based on the combination of \citep{stanovsky-etal-2019-evaluating} with our evaluation we can safely say that our alignment and gender prediction are reliable. 
From the combination of these two results we may conclude that the two tools used for defining our consistency score, e.g. entity and pronoun alignment and gender, are largely reliable.

Some errors can be caused by language-specific idiosyncrasies that affect the morphological analysis, as \citet{stanovsky-etal-2019-evaluating} noted.
For example, gender for certain words in Hebrew cannot be distinguished without diacritics, and some pronouns in German are used in both masculine and neutral (e.g., sein) forms, or feminine and third-person plural (e.g., ihr) forms. In addition, we notice that BUG sentences, specifically in partial pro-drop languages, were found to be more challenging for the alignment model, and found to account for most mistakes in Hebrew and Arabic. This can be explained by the combination of the longer and naturalistic sentences in BUG and the way that the pronoun is translated in partial pro-drop languages.

==> images/fig_1.tex <==
In blue, there are English sentences from Wino-X and Wino-MT. In orange, there are translations into French by an MT model. The English sentences have one pronoun and two antecedents/entities (marked in bold) that they can refer. Only one option of the two agrees with world knowledge and solves the coreference resolution correctly. In the translation, the antecedents/entities and entity have grammatical gender marked in purple (female) and blue (male). Using our method, we check if the referring antecedent/entity has the same gender as the pronoun, validating whether the translation matches the source coreference resolution or not. 

==> sections/00_abstract.tex <==
\begin{abstract}
% - MT models requires addressing \emph{implicitly} a lot of linguistic tasks but our understanding of what is learned is limited.
% - In this work, we measure the coreference capabilities of MT models. we develop an evaluation methodology which consists of deducing \emph{explicit} coreference clusters from the MT model in the target language and evaluate them without any label in the target language. 
%In our evaluation, we compare several commercial and large open source MT models, translating from English to six target languages against SOTA coreference resolvers on three challenging benchmarks.
%Our results show that SOTA coreference models vastly outperform MT models. Consequently,
% - We show ... 
% - to improve coreference capabilities of MT models, we propose both implicit and explicit approaches for injecting coreference signals into MT models. 
% - our method outperforms (many languages, various datasets, ...

% In this work, we investigate the coreference capabilities of end2end neural machine translation against monolingual coreference models. To that end, we develop a new evaluation paradigm that reduces MT models into source-side coreference clusters allowing us to compare their performances on equal ground. We ran experiments on three challenging benchmarks with commercial and large open source models. Our results show that monolingual coreference models are far more capable than MT models. Consequently, we suggest a novel approach of fine-tuning coreference data enriched with coreference signal. Our approach, show vast improvements and achieve comparable or even better results than commercial and large open source MT models. 

Machine translation (MT) requires a wide range of linguistic capabilities, which current end-to-end models are expected to learn implicitly by observing aligned sentences in bilingual corpora.
In this work, we ask: \emph{How well do MT models learn coreference resolution from implicit signal?} To answer this question, we develop an evaluation methodology that derives coreference clusters from MT output and evaluates them without requiring  annotations in the target language.
We further evaluate several prominent open-source and commercial MT systems, translating from English to six target languages, and compare them to state-of-the-art coreference resolvers on three challenging benchmarks.
Our results show that the monolingual resolvers greatly outperform MT models. Motivated by this result, we experiment with different methods for incorporating the output of coreference resolution models in MT, showing improvement over strong baselines.\footnote{Codebase and datasets will be released upon publication.}
%***
%Our method outperforms commercial and large open source MT models on many languages and various datasets.
\end{abstract}

==> sections/01_introduction_gabi.tex <==
Machine translation (MT) may require coreference resolution to translate cases where the source and target language differ in their grammatical properties. For example, consider translating \example{The trophy didn't fit in the suitcase because it was too small} from English to French: \example{Le trophée ne rentrait pas dans la valise car elle était trop petite} \citep{Sakaguchi2020WINOGRANDEAA}. In French, suitcase~(\example{valise}) is grammatically feminine, and trophy~(\example{trophée}) is masculine, while the source-side English does not encode grammatical noun gender. This requires an MT model to infer that \example{it} refers to the suitcase (and not the trophy) to correctly produce the feminine inflection for the phrase \example{it was too small} (\example{elle était trop petite}), whereas an incorrect coreference resolution may produce the masculine inflection (\example{il était trop petit}) corresponding to the trophy.

% figure 1
\begin{figure}[t]
\centering
\includegraphics[scale=0.33]{images/fig_1_new.png}
\caption{MT models can be compared to source-side coreference resolvers. An example translation from English (blue) to French (yellow). Our method first identifies the grammatical gender of the mentions in the target language marked in purple (female) and blue (male), followed by inferring the source side clusters (orange), through gender agreement.
%In blue, there are English sentences from Wino-X and Wino-MT. In orange, there are translations into French by an MT model. The English sentences have one pronoun and two antecedents/entities (marked in bold) that they can refer. Only one option of the two agrees with world knowledge and solves the coreference resolution correctly. In the translation, the antecedents/entities and entity have grammatical gender marked in purple (female) and blue (male). Using our method, we check if the referring antecedent/entity has the same gender as the pronoun, validating whether the translation matches the source coreference resolution or not. 
}
\label{fig:method_new}
\end{figure}

% Such cases evade lexical one-to-one translation, and instead demand source-side coreference resolution as a prerequisite for producing a correct translation.
% The prominent end-to-end approach to machine translation (citation) assumes that models implicitly learn to resolve such source-side semantic phenomena by observing aligned source-target pairs, without intermediate for the task.

Such texts evade lexical one-to-one translation, and instead demand source-side coreference resolution as a prerequisite for a correct translation. %Other cases can preserve the source-side lexical ambiguity by side-stepping coreference resolution\ariec{this is not clear what is ``preserving lexical ambiguity''. Also it doesn't side-step coref}, for example in the sentence \example{The battery didn't fit the suitcase because it was too small}, where both \emph{battery} and \emph{suitcase} are feminine in French.\ariec{I'd move this part later when we say that we use the pronouns because here the purpose of this statement is too vague.}
The prominent end-to-end approach to MT assumes that translation models implicitly learn source-side coreference resolution by observing aligned source-target pairs, without intermediate coreference supervision. While the importance of addressing such semantic phenomenon has been stated in various works~\citep{le-nagard-koehn-2010-aiding,stojanovski-fraser-2018-coreference}, it was also observed that the ubiquitous BLEU metric~\citep{bleu} does not adequately quantify it~\citep{hardmeier-federico-2010-modelling, freitag2022results}.


% In this work, we ask the following research question: How does this implicit supervision for coreference resolution fare against direct source-side monolingual training? 

% To answer this question, we develop an evaluation metric to compare the ability of MT and monolingual coreference model on source-side coreference resolution.

% Our approach aims to automatically infer source-side coreference resolution based on the produced translations. Thus, we effectively reduce an MT model to a monolingual coreference resolution


This work addresses the following research question: \textit{How well does MT learn coreference when compared against explicit coreference supervision?}
%Evaluate coreference from implicit supervision and an off-the-shelf supervised coreference is a natural point of comparison.\ariec{I don't understand this sentence}
Answering this question can improve our understanding of the way MT models operate and 
%provide insight into the effects of explicit supervision.
%This question 
also has practical implications: if implicit supervision lags behind monolingual training, it would motivate integration between end-to-end MT approaches and explicitly-supervised monolingual components.
% \oa{we can also add here that these results can help us understand to what extent an abstract semantic phenomena can be learned from an implicit signal, which is a very active field of research activity these days (we can cite here one or two examples, e.g. BLIMP or Tal Linzen's work, Leshem's work from the last ACL and say there are many others.)}
%\ariec{I reiterate my previous comment, implicit supervision of MT can be bad for coref but maybe better models or training data can improve without symbolic components. } %\ariec{That's not accurate, models can be bad at coref but introducing coref signals might not help. I don't think we really need to justify why we want to evaluate the coref capabilites of MT, it's like a probing.} \asafy{we are not saying that, this is a general note on the integration of monolingual signal to end2end models}\oa{now ok?}

In Section~\ref{sec:consistency_metric} we devise an evaluation paradigm that reduces MT output to source-side coreference resolution predictions by inferring coreference clusters from source inputs and predicted target translations. E.g., in the previous example, 
a feminine inflection for the pronoun ``it'' in French can infer linking ``it'' with ``suitcase'', while a masculine French inflection links ``it'' with ``trophy'', as shown in Figure~\ref{fig:method_new}.
%\oa{Another possibility is to formulate the translation w/o a pronoun, thereby eschewing the coreference problem.}
This approach allows us to distill the coreference resolution abilities of MT models and compare them against state-of-the-art coreference resolution models, trained explicitly on the task.

We use this approach to evaluate the coreference capabilities of several commercial and open source MT systems, translating from English to six target languages. We conduct our experiments in both synthetic \citep[\winomt{} and \winox{};][]{stanovsky-etal-2019-evaluating,emelin-sennrich-2021-wino}
and naturalistic settings  \citep[\bug{};][]{levy-etal-2021-collecting-large}.
Our results show that state-of-the-art coreference resolvers vastly outperform MT models on several benchmarks, indicating that explicit supervision may lead to better coreference performance.
%achieving higher pronoun-antecedent consistency than MT models.
%\ariec{the second half of the sentence doesn't make sense, we don't evaluate consistency but accuracy in english coref models.}\asafy{is it better?}
%On three different datasets, WinoMT 
%.\ariec{the two last sentences are not grammatical/coherent.}

% To improve coreference capabilities of MT models, we propose both implicit and explicit approaches for injecting coreference signals into MT models. 
% Following, we suggest a method for incorporating the signal of a monolingual coref model into MT by ...
Following this finding, in Section~\ref{sec:improving}, we develop methods for improving coreference in MT, both implicitly and explicitly.
Our implicit approach consists of fine-tuning MT models on 
% data that contains coreference clusters on the source side
texts that specifically require many coreference decisions, thus exposing the model to more implicit coreference signal.
Our explicit approach further enriches source sentences with predicted coreference markers. 
We show that these approaches improve coreference over the end-to-end MT approach, achieving comparable or better results than much larger MT models, both commercial systems and open-source.
% The developed methods do not only improve coreference performance but also lead to more accurate pronoun translation.
%\ariec{What do you mean by ``more accurate translation''? in terms of BLEU?}\asafy{not necessarily, as we can't get BLEU results on our evaluation datasets, but still more consistent translations are more accurate, alternatively by pronoun match results}\ariec{but this falls under coreference consistency, right?}
%Similarly, we show improvements for other metrics, such as pronoun translation and accuracy.\ariec{Readers won't understand this sentence, consider removing this point from the Intro.}

More broadly, our approach can be applied to improve the translation of other semantic phenomena that diverge in realization between source and target languages, such as plurality in second-person pronouns~\citep{Stanovsky2019YallSR} or tense marking~\citep{wolfram1985variability}. %\gabis{add citations} \asafy{like what? your "you" paper? what more?}


==> sections/02_evaluation_setup.tex <==
\label{subsec:eval}

This section describes our extensive evaluation framework, consisting of 3 evaluation datasets, 6 MT models, the alignment model we use for our consistency evaluation, and the 6 diverse target languages. 
%Then, we will detail the MT models and the training datasets we use for the improving coreference consistency experiments~(§\ref{subsec:improve_exp}).

\textbf{Evaluation Datasets.} %For evaluation, we use three challenging coreference annotated test data in English. Wino-X, WinoMT and BUG aims to measure coreference capabilities in both synthetic and naturalistic settings that require world knowledge.\ariec{consider removing, we explain these datasets in more details just below.}
The first dataset we use is \textbf{Wino-X} \citep{emelin-sennrich-2021-wino}, a filtered subset of WinoGrande \citep{Sakaguchi2020WINOGRANDEAA} built to test commonsense reasoning and coreference resolution of MT models and multilingual encoders. The dataset contains sentences similar to the one in Figure~\ref{fig:method_new}. All sentences have two entities and a pronoun, ``it'', coreferring to one of them. The dataset consists of three parts, each part constructed for a different target language (German, French, and Russian), where each part only contains sentences where the two entities have different morphological gender in the target language. 
This filtration procedure enables more accurate consistency results as the gendered pronoun clearly indicates the coreferring antecedent. Hence this dataset better reflects the MT model source-side coreference resolution capabilities.
% Each part of the dataset contains sentences from WinoGrande only if the two entities in the source sentence are expected to have different morphological gender in the target language.

Second, we use \textbf{WinoMT} \citep{stanovsky-etal-2019-evaluating}, a dataset built following the Winograd schema \citep{Levesque2011TheWS}, designed to test gender bias and coreference resolution of MT models. The sentences in this dataset contain two human entities and one gendered pronoun, e.g., \example{The \textbf{doctor} asked the \textbf{nurse} to help \textbf{her} in the procedure}. The gendered pronoun reveals the gender of the entity and adds gender attributes to the source cluster. In our example, \example{her} refers to the \example{doctor}, revealing the doctor's gender.

Finally, our third dataset is \textbf{BUG} \citep{levy2021collecting}, a semi-automatic collection of natural English sentences that are challenging with respect to societal gender-role assignments. Similar to WinoMT, each sentence contains a human entity, identified by their profession and a gendered pronoun. 
Here we use the \textsc{Gold} portion of this dataset, validated by human annotators, in order to reduce noise in the evaluation. All datasets statistics are presented in App. \S\ref{sec:appendix:06_data_sizes}.

\noindent
\textbf{Machine translation Models.} We apply our evaluation methodology on four Transformers-based machine translation models from EasyNMT\footnote{https://github.com/UKPLab/EasyNMT}: mBART50 \citep{https://doi.org/10.48550/arxiv.2008.00401, liu-etal-2020-multilingual-denoising}, M2M\_418M, M2M\_1.2B \citep{Fan2021BeyondEM}, and the monolingual
Opus-MT~\citep{tiedemann-thottingal-2020-opus}, representing the state-of-the-art for publicly available neural machine translations models.
In addition, we measure coreference consistency on the output of two commercial systems: Google Translate\footnote{https://cloud.google.com/translate} and Microsoft Translator\footnote{https://www.bing.com/translator}. 

\noindent
\textbf{Target Languages.} We conduct our evaluation study on MT models translating from English to a set of six diverse target languages with grammatical gender: Arabic, German, Spanish, Hebrew, Russian and French.
These languages have a variety of linguistic traits (e.g., alphabet, word order, number of grammatical genders, or grammar), while still allowing for highly accurate automatic morphological analysis.
These languages belong to four different families: (1) Romance languages: Spanish and French, which have gendered noun-determiner agreement; Spanish is also a \emph{pro-drop} language, i.e., pronouns can be omitted in certain cases, which in our setting may keep the coreference ambiguity of the source-side English sentence \citep{Webster2020ScalableCL} %, Wang2018TranslatingPL}. 
(2) Slavic languages (Cyrillic alphabet): Russian; that have three grammatical genders (3) Semitic languages: Hebrew and Arabic, each with a unique alphabet; both are partial pro-drop languages. (4) Germanic languages: German, also has three grammatical genders.

% \ariec{more or remove}
% After translating the English sentences to these six languages, we obtain word-alignment between the source and target sentences using awesome-align \citep{dou-neubig-2021-word}, a neural word aligner based on multilingual BERT. To extract the morphological gender of the aligned entity and the pronoun, we use spaCy\footnote{https://spacy.io/} for Spanish, French, Russian, and German, and Stanza~\citep{qi-etal-2020-stanza} for Hebrew and Arabic. 

==> sections/03_0_method.tex <==
\label{sec:method}
Coreference resolution is a prerequisite for translating between certain languages, as exemplified in Figure~\ref{fig:method_new}, where producing correct target-side gender agreement relies on source-side coreference resolution. Crucially, a reader of the French translation would infer from the gender inflection of ``it'', whether it refers to ``suitcase'' or the ``trophy''. I.e., a feminine pronoun (``elle'') would agree with the feminine noun suitcase (``valise''), while a masculine pronoun (``il'') would agree with the masculine noun trophy (``trophée').

Following \citet{stanovsky-etal-2019-evaluating}, we operationalize this observation and get an approximation of the coreference capabilities of MT models by inferring constraints on the target-side clusters from gender agreement.
In particular, assuming we have an English dataset $D$ with gold coreference annotation, we evaluate the coreference performance of an MT model $M$ (from English to language $T$ with morphological gender) in the following manner:

\begin{enumerate}
    \item Predict word alignment between $D$ and $M(D)$, i.e., the output translations of $M$. This allows us to find the translations for pronouns and possible entities in the target language $T$.
    \item Automatically extract the gender of the possible entities and the pronouns in the target language based on morphological features.
    \item Check gender agreement between the pronoun and the coreferring entity.
    % , to form constraints on the coreference clusters.
    % \item
    % \oa{add here how you define the consistency score}
\end{enumerate}

% \gabis{$\uparrow$ This seems important enough for small figure, maybe incorporate into Figure~\ref{fig:method_new}}

\paragraph{Required components.} Our evaluation methodology relies on bilingual and monolingual resources, namely an aligner between English and the target language $T$, and a morphological analyzer for $T$. Both inherently add some noise to the measurement and may thus skew our results. In section~\S\ref{sec:results} we present a manual evaluation showing that these errors are uncommon and have a small effect on the overall results.

\paragraph{Our method is an upper bound estimation of MT coreference abilities.} 
Some texts may keep the English ambiguity in the translation, and hence absolve the translation model from resolving coreference. For example, in the sentence \example{The battery didn't fit the suitcase because it was too small}, both \emph{battery} and \emph{suitcase} are feminine in French. Our proposed evaluation method will indicate that the MT model was trivially successful in such cases, and hence serves as an upper bound on its true coreference abilities.

\paragraph{Our approach is a generalization of \winomt{}.}
Unlike WinoMT,  we do not evaluate societal gender bias in MT systems, but rather use gender as a gauge for the coreference abilities of MT systems. We stress that these are different motivations, as both biased and unbiased systems may fail to perform coreference. 
To do so, in the following section we define a \emph{consistency} metric to quantify the frequency in which MT systems generate pronouns that are inconsistent with their coreferent. 
Consequently, our metric can be applied to any sentence, even when candidate entities have no gender in English, as shown in Figure \ref{fig:method_new}.



% As a result, our methodWe note that gender agreement cannot fully identify  cluster assignments, and instead indicates coreference violations.
% % \ariec{because we cannot infer that the model considers them as coreferring}\gabis{for example, ...} 
% Therefore, we treat our measure as an upper bound for the coreference performance of MT models. \ariec{In addition, }Some sentences do not require coreference resolution in order to be translated correctly. Here, we cannot infer the coreference capabilities of the MT model given a feminine inflection of the translation of \emph{it}.
%More generally, we note that gender agreement cannot identify complete cluster assignment and can only indicate coreference violations.\ariec{I'd start the paragraph with something like this sentence, then moving to the example.}  We therefore treat our measure as an upper bound for the coreference performance of MT models.

% We emphasize that our method is completely automatic and does not require any parallel data or target-side annotation.\ariec{but we still require coreference annotation in the source-side. So maybe we can write something like ``Overall, our method allows to measure the coreference capabilities of any MT model translating from English to many languages, while requiring coreference annotation only in the source sentences. } 



%Other cases can preserve the source-side lexical ambiguity by side-stepping coreference resolution\ariec{this is not clear what is ``preserving lexical ambiguity''. Also it doesn't side-step coref}, for example in the sentence \example{The battery didn't fit the suitcase because it was too small}, where both \emph{battery} and \emph{suitcase} are feminine in French.\ariec{I'd move this part later when we say that we use the pronouns because here the purpose of this statement is too vague.}

%We emphasize that our consistency measure provides an upper bound to the coreference abilities of the MT model, as our measure only checks for implicate agreement. Moreover, as noted earlier, for some sentences\ariec{which kind of sentences? } gender agreement can not identify clear clusters assignment and can only indicate coreference violations. Therefore, we treat our measure as the upper bound for coreference performances of MT models.\ariec{this repeats the first sentence of this paragraph}
%1. translate all sentences in D to target language T using model M. 2. align all the sentences in D with their counterpart translations in the target language T using awesome-align \citep{Dou2021WordAB}. Then extract all the translations of mentions annotated in the data set D (e.g ..). 3. Then extract the morphological gender of the target side mentions using language-specific morphological analysis, which we perform using a combination of the off-the-shelf tools together with handcrafted rules design for each target language upon its unique characteristics, as discussed in the following section. 4. For each target pronoun we check if the target side antecedent or entity is in agreement on their attributes, obtaining the necessary constraints. 

%This methodology uses the gender agreement as a tool for inferring the source side clusters by the MT translation. Allowing us to compare MT models against SOTA coreference models on equal ground. \ariec{we already wrote something similar earlier} 

%In addition, we check for each entity if it agrees with the source side gold gender. While the first measure the consistency of model M, the second quantified its accuracy.\oa{I didn't understand the last sent}

%To make the distinction between consistency and accuracy let's examine different translations of our running example from earlier, when both the pronoun and the relevant antecedent share the same gender then the translation is consistent but it is accurate only if the target gender is the source gender. Otherwise, if the entity and pronoun are not in agreement on their gender, the translation is not consistent and only partially accurate. Ideally, we would like a translation to be both consistent and accurate.

% We want to note that both the alignment (2) and the gender extraction (3) might add some noise to the measurement and affect it. In Section~\S\ref{sec:results}, we will present human evaluation showing that these errors are uncommon and have a small effect on the overall results.
%Either directly by returning wrong gender or either by predicting UNKNOWN for empty strings and words without morphological gender.%~\ariec{this sentence is too much detailed from this section IMO}


%We note that target side entity, antecedent or pronoun can be detected as UNKNOWN. This can happen either when word alignment don't find a corresponding word\oa{corresponding to what?} in target language or either when the morphological gender extraction found the gender of the word to be UNKNOWN\oa{when does this happen?}. We observe that for some pro drop languages (e.g Spanish) the target sentence can be consistent without containing an aligned target pronoun.\oa{how so?} Alternatively, when the aligned target pronoun is found but is ambiguous without any morphological gender or is a possessive pronoun in languages that the gender associated with the object and not the entity.\oa{didn't understand the last sent}

==> sections/03_1_evaluation_experiments.tex <==
%%%%%%%%% Compression of Consistency %%%%%%%%%
% \subsection{Consistency evaluation}

% coref models:
%\gabis{This is a rather long subsection - can you summarize what are its findings? can you maybe higlight them in the text, e.g., using the paragraph command?}


We first evaluate the accuracy of existing coreference resolvers on our three evaluation datasets (Wino-X, WinoMT and BUG), where accuracy is defined as the percentage of instances in which the model identifies that the pronoun is coreferring with the correct entity.
We select state-of-the-art models trained on CoNLL-2012~\citep{pradhan-etal-2012-conll}: SpanBERT \citep{Joshi2020SpanBERTIP}\footnote{We use the AllenNLP implementation~\citep{Gardner2018AllenNLPAD}.}, the start-to-end (\emph{s2e}) model~\citep{Kirstain2021CoreferenceRW} and \textsc{LingMess} model~\citep{Otmazgin2022LingMessLI}.
Accuracy results are shown in Table \ref{table:coref_models}. 

\input{tables/01_coref_models}

We find that \textbf{Wino-X} is more challenging than WinoMT and BUG, as all models perform quite poorly on Wino-X. Specifically, the average accuracy of coreference resolvers on Wino-X is $20\%$ lower than on WinoMT. 

% consistency results:
Table~\ref{table:cons_gmf} shows the target-side coreference consistency scores for all baseline models, on the sentences from Wino-X and WinoMT. %See Appendix \ref{sec:appendix:03_bug_results} for the results on BUG sentences.\gabis{I don't thinkt that this is a valid reference. Can you at least explain what trends we see there?}\asafy{similar ones}
The consistency results of commercial and open-source MT models on Wino-X show that these models score notably lower than accuracy of supervised coreference resolvers, indicating that the coreference capabilities of MT models are inferior. 

We notice that when MT models translate Wino-X sentences they tend to produce translations where the pronoun does not carry gender. For example,  {\it cela}, {\it c'était} in French ($31\%$ of translations) and \foreignlanguage{russian}{это,они} in Russian ($17\%$ of translations), meaning ``this'' or ``they'' in English.
%\ariec{I changed to ``this'' because it can be confusing with the original ``it'' in the source sentence.} in English.
Such translations avoid resolving the coreference as it is unclear which entity the pronoun is referring to. Similarly, in German, the MT models tend to select the neutral pronoun ``es'' much more than the 
male and female pronouns ``er'' and ``sie'' respectfully. Concretely, $68\%$ of translations have neutral pronouns, although only $22\%$ of the candidate entities are neutral. The reported percentages were calculated on Opus-MT. Similar trends were observed in all models.  
% \input{tables/wino-x/02_Wino-x_gmf_con}
% % wino-mt results:
% \input{tables/wino-mt/03_consistency_gmf}
\input{tables/2_cons_gmf_both}

%Now, we move to discuss the evaluation of WinoMT. 
In \textbf{WinoMT} evaluation we exclude translations where the candidate pronoun does not provide information about the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun. 
See App. \S\ref{sec:appendix:04_models_exampels} for examples. 

%Table \ref{table:cons_gmf} presents the consistency results on WinoMT. 
Results on WinoMT suggest that consistency is affected by both the MT model and the target language. Regarding models, in most target languages Opus-MT performances are the lowest, with average consistency of $59.3$. In contrast, mBART50 achieves consistently high results with average consistency of $70.5$, sometimes surpassing the second MT model by about 9 points. The reason for this can be the extensive pre-training of mBART50, which may endow models with commonsense knowledge, as previously demonstrated for monolingual LMs \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}. Similarly, Russian consistency results are systematically lower than the results in other languages, to the extent that the best model in Russian provides lower results than the worst model in most other languages. On the opposite end, all models in German achieve consistency of about $70$ or more. There are likely to be several reasons for this, including German's similarity with English and the research focus on improving English-German translations. 

Generally, results suggest that most tested systems across the six tested languages perform quite poorly on our metric. The best consistency results (which are an upper bound of source-side accuracy) in each language often does not match the accuracy of SOTA coreference resolvers. Two exceptions to this rule are the performances of mBART50 and consistency results in German. Specifically, mBART50 and Microsoft Translator achieve consistency results that are better than SpanBERT accuracy, although lower than \emph{s2e} and \textsc{LingMess}.


We present \textbf{BUG} consistency results in App. \S\ref{sec:appendix:03_bug_results}. Consistency results on BUG tend to be higher than WinoMT results. One explanation can be the absence of distracting entity as the one used in Wino-X and WinoM. This difference can lead to higher consistency results for lexical one-to-one translations.

It may be attributed to the absence of distracting entities such as in the syntactic Wino-X and WinoMT, which can lead to higher consistency for lexical one-to-one translations.
%We first observe that coreference resolvers on average are more accurate on WinoMT than on Wino-X by more than $20\%$ .
%\ariec{move that to afterwards, you first need to explain the results on WinoMT, then compare them to other results} 
%We note that our consistency results are an upper bound on the coreference performance of the MT models.\ariec{But this is always the case, right?} We also note that here we exclude sentences where the pronoun does not provide information on the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun.

% Our results suggest that most tested systems across six tested languages perform quite poorly on our metric.\ariec{can you write a range of performance? what do you mean by poorly? mbart obtains 75+ on some languages of WinoMT, it's not so poor...} The best performing model in each language often does not match the performance of SOTA coreference resolvers. An exception to this rule is in German, where mBART50 and Google Translate achieve better scores than SpanBERT.\ariec{Yes but SpanBERT is not so recent, these MT models are much more recent} This may be explained by German’s similarity to English \citep{Hawkins1986ACT} combined with the amounts of resources and research focus directing to improve English-German translation.\oa{so why does that mean it's more likely to work? I would just say that German is the language with the most resources and research focus, so it's likely it will score higher than others.}\asafy{I combined the two} Another interesting observation is that mBART50 achieves consistently high results compared to other models, sometimes surpassing the second MT model by 3 points. This may be attributed to the extensive pre-training of mBART50, that may endow models with commonsense knowledge, as previously indicated for large-scale monolingual LMs\ariec{is that verbatim?} \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}.

% \input{tables/exampels_improvment}
%We emphasize that our consistency measure can correctly identify a vast variety of different valid uses of pronoun in MT models output's.


\paragraph{Advantages of our Methodology.} 

% Advantages of our methodology: this paragraph looks like a related work section, which shouldn't be here. What do we want to enumerate as advantages? I can think of (1) we can capture a wide range of pronouns, including different POS, (2) our method doesn't require annotated data for coreference in the target languages. Then in related work, we will compare to pronoun translation etc



There are two important advantages in our evaluation methodology. First, while requiring only source-side  coreference annotation, our method can be used for evaluating the coreference capabilities of any MT model when translating from English to a wide range of target languages, for which a morphological analyzer is available. \ariec{I'll complete later}





% \textbf{Advantages of our methodology.} 
% Previous automated metrics for pronoun translation struggled to identify valid translations that use different pronouns than the reference. Our method is agnostic to this problem as we look at consistency between entity and pronoun rather than exact match. To exemplify this finding in Table \ref{table:lang_exampels}, we present a translation that exhibits the use of less typical pronouns
% %or that differ from the gold pronoun (provided by Wino-X)
% (see more examples in App. \S\ref{sec:appendix:04_models_exampels}). Moreover, previous methods focused on non-pro-drop languages like German and French where the candidate pronoun in the target language are pronoun. In partial pro-drop languages like Hebrew and Arabic, there are cases where the information of the pronoun can be encoded into a noun or other part of speech. Our methodology can account for such cases by relying on the gender agreement between the candidate entity and candidate pronoun, even though the candidate pronoun has a different part of speech. Such examples also appear in App. \S\ref{sec:appendix:04_models_exampels}.
% In addition, Figure \ref{fig:pron_dis} shows the parts of speech (POS) distribution of the candidate pronoun for the candidate pronoun of Opus-MT in Hebrew, where we filter rare POS that appear less than once.%  We emphasize that this capability is a clear advantage of our methodology compared to previous automatic metrics for pronoun translation. sec:appendix:03_bug_results

% figure 2
\begin{figure}[tb!]
\centering
\includegraphics[scale=0.35]{images/myplot_new_font.png}
\caption{The distribution of parts of speech for the candidate pronoun of Opus-MT in Hebrew.}
\label{fig:pron_dis}
\end{figure}

==> sections/03_2_Human_Validation.tex <==
To assess our evaluation methodology, we randomly sampled 50 translations of the Opus-MT model from all evaluation datasets and in all target languages, annotating each sample by a target language native speaker. The human annotators were asked to identify if the candidate pronoun is indeed the target pronoun and to verify that the gender prediction is correct. This way, we can account for both types of possible errors, i.e., alignment and gender extraction. 
We compare the human annotations to the output of our automatic method and find that the average agreement over all languages and datasets is above $90\%$ (see full results in App. \S\ref{sec:appendix:05_human_validation_results}). These results are comparable to the ones reported by \citet{stanovsky-etal-2019-evaluating}, who conduct human validation and report that their alignment and gender prediction of the entity in question are reliable for $85\%$ of translations across all languages. %\ariec{what's the purpose of this sentence?}
%\oa{this sentence is unclear; in what setting did they show it?}
%Based on the combination of \citep{stanovsky-etal-2019-evaluating} with our evaluation we can safely say that our alignment and gender prediction are reliable. 
From the combination of these two results we may conclude that the two tools used for defining our consistency score, e.g. entity and pronoun alignment and gender, are largely reliable.

Some errors can be caused by language-specific idiosyncrasies that affect the morphological analysis, as \citet{stanovsky-etal-2019-evaluating} noted.
For example, gender for certain words in Hebrew cannot be distinguished without diacritics, and some pronouns in German are used in both masculine and neutral (e.g., sein) forms, or feminine and third-person plural (e.g., ihr) forms. In addition, we notice that BUG sentences, specifically in partial pro-drop languages, were found to be more challenging for the alignment model, and found to account for most mistakes in Hebrew and Arabic. This can be explained by the combination of the longer and naturalistic sentences in BUG and the way that the pronoun is translated in partial pro-drop languages.

==> sections/04_0_improving_coref.tex <==
In the previous section we showed that the coreference performance of MT systems, obtained through an implicit signal, seems inferior to that of coreference resolution learned from an explicit signal. This result raises the question of whether we can leverage dedicated conference resolvers to improve the consistency of MT coreference.

To address this question, we propose two data augmentation techniques that leverage a source-side English coreference model, and show that finetuning on them indeed improves coreference resolution in MT.
%In the following section we experiment with both of these approaches.


\paragraph{Augmented fine-tuning with instances which require coreference resolution.} First, we run a coreference resolution model on the source-side sentences. We then consider two approaches for constructing the augmented fine-tuning data: (1) \emph{Coref data} with all sentences that have non-singleton clusters and (2) \emph{Gender data}, a subset of \emph{Coref data} where there is at least one non-singleton cluster with a gendered pronoun (he, she, her, him, hers, his) . The motivation for this augmented fine-tuning strategy is that further fine-tuning on such instances would expose the MT model to examples that may bear a coreference signal. 

\paragraph{Adding explicit source-side coreference markers.}
Second, we use the non-singleton clusters from the coreference model to add inline coreference markers in the source sentences. For our example sentence, this process produces the following source-side sequence: \emph{``The trophy didn't fit in the \textbf{<ENT1>} suitcase \textbf{</ENT1>} because \textbf{<ENT1>} it \textbf{</ENT1>} was too small''}, indicating that ``suitcase'' and ``it'' are coreferring. 
% We apply this explicit coreference markers to both \emph{Coref data} and \emph{Gender data}. 


% gabis{I'm not sure if this figure is actually needed. It's pretty clear from the text.}


% For each cluster, we added two unique coreference markers, which we inserted around each mention in the sentence. \ariec{Since coreference resolvers usually do not output singleton clusters (ie. cluster with only one mention), }
% %\ariec{you should elaborate here, what are the markers? how exactly we obtain those markers ``based'' on the coref resolvers. I know that the figure explains it but the text should be self contained and clearly describe the process.} 
% These tokens guide the model to associate the pronoun and the coreferring antecedent, aiding the model in generating a more consistent translation that is faithful%\ariec{is it the right term?}\asafy{aligned? can be confusing too.., faithful output with respect to the source sound right} 
% to source coreference clusters.

% %\oa{This section needs to be rewritten. The figure is helpful though. It should first state the approach in high level (that part is pretty much ok), then it should \textbf{formally} define the three procedures (and refer to the figure), then related work (that part is mostly ok)}
% In this section, we present a novel fine-tuning approach for improving coreference consistency \gabist{based on the observation that NMT models can quickly adapt}~\ariec{who observed? adapt to what? what's the relationship between the adapation and fine-tuning?}\gabis{agreed, I suggest to just remove that part, I think we can do without it}\citep{Freitag2016FastDA, saunders-byrne-2020-reducing}.
%  Specifically, we propose two methods\ariec{I still find it confusing to have ``\textbf{a} novel fine-tuning approach'', then ``\textbf{two} methods''. Maybe we can write from the beginning that we develop two novel methods for fine-tuning, explicit and implicit?}\gabis{+1} for fine-tuning MT models, which inject coreference signals either implicitly or explicitly.

% \ariec{Our first/implicit method....}
% Our motivation for this data augmention method stems from our analysis of our parallel dataset~\ariec{which parallel data? and which analysis? where did you show them?}, which showed that approximately one fifth of the sentences in it have coreference phenomena, hence enriching it with more examples of this phenomena can improve training of MT models with regard to coreference.~\ariec{but we don't add more examples with coref, we only remove other sentences that don't involve coref. We can write that since there are only a few instances with coref, when trained on the full data, the model learns more from the other examples and doesn't focus on coref.} Accordingly, we propose to fine-tune on a subset of the data\ariec{which data?}, with sentences that all contain coreference clusters \ariec{in the source-side}. Notice that in this setting, the inference remains standard.\ariec{do we need this sentence? When the readers arrive to this part, they won't think that the inference should be different}\gabis{$\uparrow$ Given all the comments here, I think we can just remove this paragraph, let's skip to saying what we actually do}


% %In the implicit approach,\oa{maybe a name for it?} we consider three steps for this adaptation problem. Filter parallel training data from instances that the source sentence does not contain coreference phenomena (as deemed by a coreference resolver),fine-tune the model on the filtered data, and inference with the enhanced models produced by adaptation.\oa{why is this three steps? inference is not part of it; you can just say we train only on a dataset that contains coreference phenomena.}\asafy{because in inference we insert coreference markers as well, not in the implicit approach but it maybe helpful to notice that those three steps are relevant to our method. }\ariec{I agree with Omri, these 3 steps are confusing because we describe them as new method for \textbf{fine-tuning} so actually even the second point is not relevant here, you should only say that before fine-tuning, we select sentences that contain coreferencec clusters. I also suggest to explain the motivation for this method: if you fine-tune an entire dataset for MT, only less than third of the sentences have coref, and models don't manage to learn well the task. We propose to fine-tune on a subset of the data, with sentences that all contain coref. Notice that in this setting, the inference remains standartd. }

% %Regarding data filtering, we took a parallel dataset and ran a coreference resolver on the source side sentences. Then we filter all the sentences that do not contain coreference clusters.\oa{how is that defined? at least two corefering mentions?} The filtered data we got overrepresents coreference phenomena. Such that fine-tuning MT models on that data will enhance their coreference capabilities.\oa{I would remove this paragraph and instead just write formally how the filtering works.}

% \ariec{isn't it obvious? maybe we can say in the previous paragraph that we use a coref model for that and in footnote the exact criterion of 2 coreferring mentions?}
% Our data filtering schema works as follows. We take parallel dataset, we run the coreference resolver on the source sentences.% For each sentence in $\mathcal{P}$, we get all the coreference clusters $CR$ identified. 
%  In cases where a sentence does not have coreference cluster, that is, if it does not have at least two coreferring mentions, we filter it out from the dataset. the outcome dataset overrepresents coreference phenomena.%\ariec{Too much detailed, no need for mathematical symbols, should be shortened.}
% Hence is more equipped to enhance coreference capabilities.% \ariec{see my comment above, I'd start by the motivation, maybe we can find citations that also support this finding} %for  MT models.


% \ariec{I think here again we should start with some motivation, something like: The implicit method is effective, but we want to go a step further and aid the model by specifying expressly the coreferring mentions. Then we will describe how we add markup given the coreference clusters.}
% In the explicit data augmentation method, we fine-tune the MT model with the same source sentences (i.e., same filtering method) augmented with coreference markup.\ariec{this is not really clear, what is coref markup? in the next sentence, you say markers, what's the difference between them?} We integrate those coreference markers based on the coreference resolver predication's (see Figure~\ref{fig:tokens}). For each cluster, we added two unique coreference markers, which we inserted around each mention in the sentence. \ariec{Since coreference resolvers usually do not output singleton clusters (ie. cluster with only one mention), }We added such markers only for clusters containing more than two mentions.
% %\ariec{you should elaborate here, what are the markers? how exactly we obtain those markers ``based'' on the coref resolvers. I know that the figure explains it but the text should be self contained and clearly describe the process.} 
% These tokens guide the model to associate the pronoun and the coreferring antecedent, aiding the model in generating a more consistent translation that is faithful%\ariec{is it the right term?}\asafy{aligned? can be confusing too.., faithful output with respect to the source sound right} 
% to source coreference clusters.

% %\ariec{it should be written that this is only for the ``explicit'' approach}
% During inference, we can add coreference markers to the evaluation dataset in two ways. The first is by using gold annotation if such coreference annotation is available. The second is by using the predictions of a coreference resolver, as used for creating the training data. These tokens utilize the explicit coreference signal inserted into the training data to direct the model towards translation where mentions within the same cluster have the same morphological gender.~\ariec{what's the purpose of this sentence?}
% %a direct signal to associate between antecedent and pronoun within the same cluster, assisting the model in translating coreferring antecedent and pronoun with the same morphological gender.\ariec{this repeats the last sentence of the previous paragraph, consider removing. }

% %After fine-tuning, when the models already trained to use those coreference markers as indication of antecedents in the same clusters. in inference time, we can add coreference markers based on coreference resolver predication's or gold annotation if such data is available. Giving the model direct signal to associate between antecedent and pronoun within the same cluster, helping it to translate them with the same morphological gender. 

% %we consider three steps that may benefit from such fine-tuning: fine-tuning the model on parallel data where the source sentences contain coreference phenomena (as deemed by a coreference resolver), incorporating explicit coreference signal into the data, and inference with the enhanced models produced by adaptation.
% %Additionally, to add explicit coreference signal we use coreference resolver predication's to integrate the source side sentences with coreference markers as demonstrated in Figure~\ref{fig:tokens}. Those tokens guide the model to associate the pronoun and the co-referring antecedent. Aiding the model in generating a more consistent translation that is faithful to source coreference clusters.


%\oa{general note: I think we're diving too quickly to the technical details here. We should start with the general notion of integrating information about coreference into the MT model's training data. We can say that we explore two ways of do so: (1) explicitly encoding it in the input; (2) filtering the data so as to overrepresent coreference phenomena. We should also briefly refer to prev work (if it's too long, we need to add it to another section and reference it from here.} 
%Previous method used Oracle(2 articals) and gender markers to improve co-reference to minimize gender biases by adding tokens to the source sentences.\oa{I didn't understand this sentence} In a similar fashion we enrich the source side sentences with co-reference markers.
%Guiding the model to associate between the pronoun and the co-referring antecedent (entity).

% \begin{figure}[tb!]
% \centering
% \includegraphics[scale=0.31]{images/tokens.png}
% \label{fig:method}
% \caption{An example of adding coreference markers, given the prediction of a coreference model. Given an English sentence, we run a coreference resolver on it. The coreference resolver predicts the coreference clusters in the sentence. Then we add mark up to indicate mentions belonging to the same cluster.
% }
% \label{fig:tokens}
% \end{figure}

%Several previous methods aiming for improving coreference of MT models and reducing undesirable biases such as gender bias modified the training data in ways that shear some similarities with our method. \cite{vanmassenhove-etal-2018-getting} incorporate a ‘speaker gender’ tag into training data, allowing gender to be conveyed at the sentence level. Similarly, \cite{moryossef-etal-2019-filling} added a prefix to disambiguate the coreference in the sentence. \citep{stafanovics-etal-2020-mitigating}, train NMT models from scratch with all source language words annotated with target language grammatical gender. \citep{stojanovski-fraser-2018-coreference} advise oracle based approach to inject pronoun translation and its gender into the source sentence. In later research they combined this method with curriculum learning training \citep{stojanovski-fraser-2019-improving}. Our method is novel in the way it enrich the data with coreference signal using only source side and can be used with monolingual coreference model only without the need of annotated data. 

%Finally, in inference time we can add coreference markers based on model or gold clusters if available. Giving  the model direct signal to associate between antecedent and pronoun within the same cluster, helping it to translate them with the same morphological gender. 

%The method we use is reminiscent of other fine-tuning approaches to enhance model capabilities similarly to \citep{saunders-byrne-2020-reducing} that view fine-tuning as a domain adoption task.%\oa{in what sense are they similar?}
%Other lines of related work uses source-side sentences to reduce gender bias \citep{vanmassenhove-etal-2018-getting, stafanovics-etal-2020-mitigating, saunders-etal-2020-neural} or to improve coreference in MT \citep{ stojanovski-fraser-2018-coreference, stojanovski-fraser-2019-improving}, by appending them with explicit gender tokens and target pronoun tokens. However, to our knowledge, no previous work has used coreference annotation over the input to improve coreference capabilities in MT.


% In figure 2 we exemplified the way we incorporate the co-reference markers.
% Into the sentences. This method allows us to enrich the sentences with gold co-reference signal or a strong monolingual co-reference models signal.
% This way when we fine-tune the MT model it learns to associate mentions within the same cluster, helping it to translate them with the same morphological attributes.


%In our experiments we took parallel data and ran Kirshten model on the source side sentences. We then used the model prediction to incorporate co-reference markers into the source side sentences.When translating sentences in inference time we can enrich the sentences with both model or gold coreference signal, helping the model to produce consistent translation Our method incorporated source side signal allowing us to use it in both training and inference time.Differently, from other methods that incorporate target side signal prevent them to use their methods in inference time.

==> sections/04_1_experimental_setup.tex <==
% %\oa{redundant} 
% In this section, we will first describe the evaluation datasets, MT models, target languages, and alignment model we use for our consistency evaluation~(§\ref{subsec:eval}). Then, we will detail the MT models and the training datasets we use for the improving coreference consistency experiments~(§\ref{subsec:improve_exp}).

% %\ariec{We need to better structure this section. I suggest to keep the order of the paper: (1) Evaluation -- datasets (explain that we only need english sentences with coref annotation and give example of each dataset to explain why we chose those), language and morpholigizer -- and (2) Models -- models (baseline, commercial and others) and training data } 

% %\ariec{consider adding an outline of the section in a style like ``We first describe the evaluation then how we improve. (should be rephrased of course)}

% \subsection{Evaluation}
% \label{subsec:eval}

% %\ariec{This section currently looks like a bunch of boring techincal details, I suggest to add an outline of the subsection and refer to the described method for each detail (see what I wrote for the word-alignment and morphological analyzer). BTW, we might consider modifying a bit the current flow and write the paper as a story, (1) eval description + experimental setting + results and (2) improving method + experimental setting + results. Because it's a lot of technical details that are not related one to each other. }


% %In a lot of cases a lexical translation of the source sentence will seem as it preserve the necessary constraints and provide an consistent translation. This is the reason we wanted to choose a challenging data sets aiming to investigate MT models ability in challenging scenario. 
% \textbf{Evaluation Dataset.} For evaluation, we use three challenging coreference annotated test data in English. Wino-X, WinoMT and BUG aims to measure coreference capabilities in both synthetic and naturalistic settings that require world knowledge.\ariec{consider removing, we explain these datasets in more details just below.}

% %\ariec{consider removing this sentence}
% % and gender understanding.\oa{what is gender understanding? find another term or remove}

% %focus on two major obstacle for coreference models, gender and world knowledge, in both syntactic and neutral setting.
% %In our study we mainly focus on gender agreement as a way to check the coreference consistency. Accordingly, we focus on two challenge sets. 



% The first dataset is Wino-X \citep{emelin-sennrich-2021-wino}, a subset of WinoGrande \citep{Sakaguchi2020WINOGRANDEAA} built to test commonsense reasoning and coreference resolution of MT models and multilingual encoders. The dataset contains sentences similar to the one in Figure~\ref{fig:method_new}. The pronoun in all the sentences is ``it'', and it refers to one of the two entities. The dataset consists of three parts, each part constructed for a different target language (German, French, and Russian). Each part of the dataset contains sentences from WinoGrande only if the two entities in the source sentence are expected to have different morphological gender in the target language.

% %contains sentences similar to the one appearing in Figure~\ref{fig:method_new}. The pronoun in all the sentences is ``it'', and it refers to one antecedent determined by the trigger word, in our example \example{small}. The dataset was designed such that each sentence translation has two antecedents of different genders. This design forces the tested model to select, which antecedent of the two the pronoun is referring to.\ariec{need rephrasing. Start by saying that Wino-X exists in 3 languages (ru, fr, de), then for each language, they choose a subset of english sentences with that desired property.}

% %filtered to contain only sentences where the two antecedent in the target language are of different gender. Wino-X is free of gender or positional bias. Solving the CoR is heavily depend on using common-sens reasoning and deploying world knowledge.
% The second dataset is WinoMT \citep{stanovsky-etal-2019-evaluating}, a dataset built following the Winograd schema \citep{Levesque2011TheWS}, designed to test gender bias and coreference resolution of MT models. The examples in this dataset contain two human~\ariec{is this important? I mean is it critical that readers will know that WinoMT is not all entities but human entities?} entities and one gendered pronoun as in this example: \example{The \textbf{doctor} asked the \textbf{nurse} to help \textbf{her} in the procedure}. In this setting, the gender pronoun reveals the gender of the entity and adds gender attributes to the source cluster. In our example, \example{her} refers to the \example{doctor}, revealing the doctor's gender.

% The third dataset is BUG \citep{levy2021collecting}, a semi-automatic collection of natural English sentences which are challenging with respect to societal gender-role assignments.~\ariec{I don't understand this sentence} Similar to WinoMT, each sentence contains a human entity, identified by their profession and a gendered pronoun. %As these sentences are more naturalistic, they can have many more unannotated antecedents and pronouns in each sentence.%
% % Due to the naturalistic nature\ariec{what is the naturalistic nature?} of these sentences and the way the dataset was constructed, the sentences may have a greater number of mentions and pronouns.\ariec{why this is important?}
% %For example, in the sentence \example{The \textbf{doctor} said \textbf{she} did not think the boy had SARS, but would treat it as such} there is a pronoun ,\example{she}, coreferring to one entity ,\example{doctor}, and other entity and pronoun (\example{boy} \example{it}). 
% Here we use the \textsc{Gold} portion of this dataset, which was validated by human annotators, in order to reduce noise in the evaluation.
% %\ariec{be more explicit and say we use the \textsc{Gold} portion of this dataset, which was validated by human annotators, in order to reduce noise in the evaluation.}
% %While both data sets require Cor information in order to translate the sentences accurately and constantly, the later opus\ariec{what do you mean?} other difficulty\ariec{I wouldn't call it other difficulty because performance is higher in BUG than in MT.} by coming from real-world distribution. 
% % the source side

% % We note that there are a few differences between these three datasets. Wino-X is a more challenging evaluation dataset as the model choice to connect the pronoun to its true antecedent is determined by the trigger word alone.\ariec{WinoMT also depends on a trigger word} WinoMT and BUG, on the other hand, contain stereotypical and unstereotypical examples designed to test for social and gender biases. These considerations are relevant to the challenge that each dataset presents, but are orthogonal to our comparison of MT models and coreference resolvers, as all models face the same challenging datasets.\oa{what do you mean ``all models share the same challenges''? can we remove this part?}\asafy{I rephrased it, what part did you meant?}\ariec{How important is this paragraph for the paper? I mean, what the readers loose if we remove this paragraph?}
% % We also note that BUG contains more neutral sentences that tend to be longer with possibly much more mentions.

% \noindent
% \textbf{Machine translation Models.} We apply our evaluation methodology on four transformers-based machine translation models from EasyNMT\footnote{https://github.com/Helsinki-NLP/Opus-MT}: the multilingual mBART50 \citep{https://doi.org/10.48550/arxiv.2008.00401, liu-etal-2020-multilingual-denoising} the multilingual M2M\_418M, M2M\_1.2B \citep{Fan2021BeyondEM}, and the monolingual
% Opus-MT~\citep{tiedemann-thottingal-2020-opus}, representing the state-of-the-art for publicly available neural machine translations models.
% %mBART50 is a one to many, multilingual translation model built on top of a pre-trained mBART. The inclusion of mBART50 follows the assumption that extensive pre-training may endow models with commonsense knowledge, as previously indicated for large-scale monolingual LMs \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}.
% %M2M model The Many-to-many (M2M) multi-language translation model can directly translate between set of 100 languages. After large-scale pre-training, different variants can be obtained. We use 418M and 1.2B models as strong baselines.
% %Opus-MT is based on Marian-NMT2 framework, a NMT with efficient training and decoding capabilities \citep{junczys-dowmunt-etal-2018-marian}. %Those models where trained on OPUS\footnote{\url{opus.nlpl.eu}}\citep{tiedemann-2012-parallel}, a large  parallel corpora.
% In addition, we measure coreference consistency on the output of two commercial systems: Google Translate\footnote{https://cloud.google.com/translate} and Microsoft Translator\footnote{https://www.bing.com/translator}. 

% \noindent
% \textbf{Target Languages.} We conduct our evaluation study on MT models translating from English to a set of six diverse target languages with grammatical gender: Arabic, German, Spanish, Hebrew, Russian and French.
% These languages have a variety of other linguistic characteristics (e.g., alphabet, word order, number of grammatical gender, or grammar), while still allowing for highly accurate automatic morphological analysis.%\ariec{is this sentence important?}
% These languages belong to four different families: (1) Romance languages: Spanish and French, which have gendered noun-determiner agreement; Spanish is also a pro-drop language.
% %\ariec{what is it? and what about other languages?} 
% (2) Slavic languages (Cyrillic alphabet): Russian; that have three grammatical genders (3) Semitic languages: Hebrew and Arabic, each with a unique alphabet; both are partial pro-drop languages. (4) Germanic languages: German, that also have three grammatical genders. %and is non pro-drop language.
% %\ariec{Consider merging this sentence with the previous ones, the names of languages are repetitive.}
% After translating the English sentences to these six languages, we obtain word-alignment between the source and target sentences (step 2) using awesome-align \citep{dou-neubig-2021-word}, a neural word aligner based on multilingual BERT. To extract the morphological gender of the aligned entity and the pronoun (step 3), we use spaCy\footnote{\url{https://spacy.io/}} for Spanish, French, Russian, and German, and Stanza~\citep{qi-etal-2020-stanza} for Hebrew and Arabic. 

% % \noindent
% % \textbf{Alignment.} We use awesome-align \citep{dou-neubig-2021-word}. A neural word aligner that extracts word alignments from multilingual BERT (mBERT).%It obtains robust performance in zero-shot settings.

% %\textbf{Coreference Resolution Models.} For comparison with SOTA coreference models we use the AllenNLP \citep{Gardner2018AllenNLPAD} implementation of SpanBERT \citep{Joshi2020SpanBERTIP} start-to-end (\emph{s2e}) model~\citep{Kirstain2021CoreferenceRW} and \textsc{LingMess}~\citep{Otmazgin2022LingMessLI}. SpanBERT introduces contextual span representation to the the e2e-coreference model to achieve state-of-the-art results on the English portion of the popular CoNLL-2012 shared task coreference benchmark \citep{pradhan-etal-2012-conll}.(\emph{s2e}) model is a more efficient model without span representation. \textsc{LingMess} ... \asafy{arie can you elaborate}.We use those models as the best current models for coreference resolution.

% \subsection{Improving Coreference Experiment}
% \label{subsec:improve_exp}

\paragraph{MT models.} In our fine-tuning experiments, we opt for the Opus-MT model, since its size (68M parameters) and efficiency \citep{junczys-dowmunt-etal-2018-marian} enables us to run extensive experiments across many languages. 

% We apply our fine-tuning method on Opus-MT model because it's 
%For fine-tuning we used Opus-MT models. Based on Marian-NMT2 framework, 
%Opus-MT is NMT with 
%efficient training and decoding capabilities \citep{junczys-dowmunt-etal-2018-marian} and .their 
%size (68M parameters) and efficiency \citep{junczys-dowmunt-etal-2018-marian} allow us to run extensive experiments on a large set of languages.
%\ariec{This paragraph is unclear, it should be ``We apply our fine-tuning method on XXX model because...''} 
\paragraph{Training datasets.}
For fine-tuning data of Spanish, French, and German, we use Europarl \citep{Koehn2005EuroparlAP}, and for Russian, Hebrew, and Arabic, we use CCMatrix \citep{Schwenk2021CCMatrixMB}, randomly sub-sampled to 5M sentences for computational reasons. In each dataset, we find instances that require coreference resolution and add appropriate markup using the \emph{s2e} coreference resolver. We use \emph{s2e} as it performed well in the previous experiments. Table \ref{table:data_train} shows the size of \emph{Coref data} and \emph{Gender data} for all training datasets. Note that invariably \emph{Gender data} is an order of magnitude smaller than \emph{Coref data}.


\input{tables/data/train}


\paragraph{Fine-tuning and inference.}
For each language, we fine-tune the Opus-MT model using four different finetuning datasets: (1) \emph{Coref data} (2) \emph{Coref data} with explicit coreference markers, (3) \emph{Gender data} and (4) \emph{Gender data} with explicit coreference markers. The inference on our three evaluation datasets (Wino-X, WinoMT, BUG) conforms with the fine-tuning procedure of each model. Namely, we run the models (1) and (3) on raw English sentences. For the models (2) and (4), we first add explicit coreference markers according to the output of the \emph{s2e} model (a) or the gold annotation (b), then translate those augmented sentences to the different languages. 

%on Europarl/CCMatrix source side (English) sentences. We then filter the sentences without coreference clusters. We daubed this data coref data. 
%Afterward, we filter the sentences where the coreference cluster didn't contain gender pronouns, we daubed this data gender-data.~\ariec{This filtering makes sense only for some datases (WinoMT and BUG) and it's not part of our method (we didn't write this filtering in the improving section) maybe we can move it to the results? }  %For comparison we randomly sample sentences in the same sizes of coref data and gender data from the original datasets. 
%\ariec{Again, you should refer to our two methods of fine-tuning.}
%To both coref data and gender data we add coreference markers as described in section \S\ref{sec:improving}.
%In addition, for training data of Spanish, French, and German we used Europarl \citep{Koehn2005EuroparlAP}, and for Russian, Hebrew and Arabic we use CCMatrix \citep{Schwenk2021CCMatrixMB}. 




==> sections/04_2_results_and_discussion.tex <==
% %%%%%%%%% Compression of Consistency %%%%%%%%%
% \subsection{Consistency evaluation}
% % coref models:

% \ariec{arrange the start/first etc.}

% %\ariec{I rephrase, please see that it's OK}
% We \textbf{first} evaluate the performance of existing coreference resolvers on our three evaluation datasets (Wino-X, WinoMT and BUG). We select state-of-the-art models trained on CoNLL-2012~\citep{pradhan-etal-2012-conll}: SpanBERT \citep{Joshi2020SpanBERTIP}\footnote{We use the AllenNLP implementation~\citep{Gardner2018AllenNLPAD}.}, the \emph{s2e} model~\citep{Kirstain2021CoreferenceRW} and the very recent \textsc{LingMess} model~\citep{Otmazgin2022LingMessLI}.
% % For comparison~\ariec{Which comparison? it's not clear} with SOTA coreference models we use the AllenNLP \citep{Gardner2018AllenNLPAD} implementation of SpanBERT large \citep{Joshi2020SpanBERTIP}, the start-to-end (\emph{s2e}) model~\citep{Kirstain2021CoreferenceRW} and the very recent \textsc{LingMess} model~\citep{Otmazgin2022LingMessLI}. We use those models as they achieve state-of-the-art results on CoNLL-2012 coreference benchmark \citep{pradhan-etal-2012-conll}. 
% Results are shown in Table \ref{table:coref_models}.
% %We will use this table for comparison to consistncy scores of MT models throughout this section. 
% \input{tables/01_coref_models}

% % wino-x results:
% %\ariec{now that we combine the tables on Wino-X with WinoMT, it makes more sense to refer to the table once for both datasets, then you can write separetely the findings of each dataset.}

% Table~\ref{table:cons_gmf} shows the target-side coreference consistency scores for all baseline models, on the sentences from Wino-X and WinoMT. See Appendix \ref{sec:appendix:03_bug_results} for the results on BUG sentences. 

% We \textbf{start} by analyzing Wino-X results.
% \textbf{Firstly}, we notice that Wino-X is more challenging than WinoMT and BUG as all models, both coreference resolvers and MT models, perform poorly on Wino-X. The coreference resolvers average accuracy of Wino-X is $20\%$ less than the average accuracy of WinoMT.

% We \textbf{first} observe that coreference resolvers on average are more accurate on WinoMT than on Wino-X by more than $20\%$ .
% % We start by measuring the consistency results of MT models on Wino-X. We note that this dataset is exceptionally hard,\ariec{maybe use a softer expression?} such that SpanBERT achieves accuracy results that are hardly better than chance ($50\%$).\ariec{I'd write a simpler sentence, something like ``Wino-X seems more challenging that WinoMT and BUG as all models perform poorly on Wino-X.''} %, on associating the right antecedent with the pronoun. 
% %In this regard, we note that several languages, such as German and Russian have three grammatical genders, decreasing the random chance in our setting to $33\%$.\oa{so is the chance level 50\% or 33\%? or does this depend on the language? if it depends on the language, don't write in the prev sent that it's 50}
% %\oa{didn't understand the last sentence; what is the change level then in these cases? we should report chance level in all tables.}
% %Consistency results of commercial and open-source MT models on Wino-X provide an upper bound on the coreference accuracy of those models. It is noticeable that our baseline models lag behind supervised resolvers.
% %Table \ref{table:cons_gmf} shows The consistency results of commercial and open-source MT on Wino-X. 
% %The left side of Table \ref{table:cons_gmf} shows the consistency results of commercial and open-source MT on Wino-X. Results of MT models lag behind supervised resolvers even though consistency is a more forgiving measure.\ariec{consider repeating briefly why it's a more forgiving measure}
% Consistency results provide an upper bound for the source-side coreference accuracy of MT models since consistency only indicates coreference valuation and not accurate coreference assignment.
% The Consistency results of commercial and open-source MT models on Wino-X show those models lag behind supervised coreference resolvers.

% We notice that MT systems tend to produce translations where the pronoun does not carry gender. For example,  {\it cela}, {\it c'était} in French and \foreignlanguage{russian}{это,они} in Russian, meaning ``this'' or ``they'' in English.
% %\ariec{I changed to ``this'' because it can be confusing with the original ``it'' in the source sentence.} in English.
% Such translations avoid resolving the coreference as it is unclear to which entity the pronoun is referring to. Similarly, in German, the MT models tend to select the neutral pronoun ``es'' much more than the 
% male and female pronouns ``er'' and ``sie'' respectfully. \ariec{can you add some statistics of all these phenomena? Because now, it sounds like you pick a few examples and tell your observation...}
% % \input{tables/wino-x/02_Wino-x_gmf_con}
% % % wino-mt results:
% % \input{tables/wino-mt/03_consistency_gmf}
% \input{tables/2_cons_gmf_both}

% %Now, we move to discuss the evaluation of WinoMT. 
% We \textbf{start} by noting that in WinoMT we exclude translations where the candidate pronoun does not provide information on the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun. 
% See Appendix \ref{sec:appendix:04_models_exampels} for examples. 

% %Table \ref{table:cons_gmf} presents the consistency results on WinoMT. 
% Results on WinoMT suggest that consistency is affected by both MT model and target language. Regarding models, in most target languages Opus-MT performances are last, with average consistency of $59.3$. In contrast, mBART50 achieves consistently high results with average consistency of $70.5$, sometimes surpassing the second MT model by about 9 points. The cuase of this can be the extensive pre-training of mBART50, which may endow models with commonsense knowledge, as previously demonstrated for monolingual LMs \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}. similarly, Russian consistency results are systematically lower than the results in other languages. To demonstrate that we can observe that the best model in Russian provide lower results the the worst model in most other languages. In the opposite end, all model in German achieve consistency of about $70$ or more. This may be explained by German’s similarity to English \citep{Hawkins1986ACT} combined with the amounts of resources and research focus directing to improve English-German translation.

% Generally, results suggest that most tested systems across six tested languages perform quite poorly on our metric. The best consistency results( upper bound of source-side accuracy) in each language often does not match the accuracy of SOTA coreference resolvers. Two exceptions to this rule are the performances of mBART50 and consistency results in German. Specifically, mBART50 and Microsoft Translator achieve consistency results that are better than SpanBERT accuracy, although lower than \emph{s2e} and \textsc{LingMess}.

% %We first observe that coreference resolvers on average are more accurate on WinoMT than on Wino-X by more than $20\%$ .
% %\ariec{move that to afterwards, you first need to explain the results on WinoMT, then compare them to other results} 
% %We note that our consistency results are an upper bound on the coreference performance of the MT models.\ariec{But this is always the case, right?} We also note that here we exclude sentences where the pronoun does not provide information on the entity's gender. For example, in French, possessive pronouns agree with the gender of the possessed object, rather than the possessor as in English. Another example is in Spanish, which is a pro-drop language, where a valid translation can drop the pronoun and use a generic verb, leaving the only gender signal in the translation to be marked on the profession noun.

% % Our results suggest that most tested systems across six tested languages perform quite poorly on our metric.\ariec{can you write a range of performance? what do you mean by poorly? mbart obtains 75+ on some languages of WinoMT, it's not so poor...} The best performing model in each language often does not match the performance of SOTA coreference resolvers. An exception to this rule is in German, where mBART50 and Google Translate achieve better scores than SpanBERT.\ariec{Yes but SpanBERT is not so recent, these MT models are much more recent} This may be explained by German’s similarity to English \citep{Hawkins1986ACT} combined with the amounts of resources and research focus directing to improve English-German translation.\oa{so why does that mean it's more likely to work? I would just say that German is the language with the most resources and research focus, so it's likely it will score higher than others.}\asafy{I combined the two} Another interesting observation is that mBART50 achieves consistently high results compared to other models, sometimes surpassing the second MT model by 3 points. This may be attributed to the extensive pre-training of mBART50, that may endow models with commonsense knowledge, as previously indicated for large-scale monolingual LMs\ariec{is that verbatim?} \citep{Sakaguchi2020WINOGRANDEAA, Bhagavatula2020AbductiveCR, Huang2019CosmosQM}.

% \input{tables/lang_exampels}
% %We emphasize that our consistency measure can correctly identify a vast variety of different valid uses of pronoun in MT models output's.
% Previous automated metrics for pronoun translation struggled to identify valid translations that use different pronouns than the reference. Our method is agnostic to this problem as we look at consistency between entity and pronoun rather then exact match. To exemplify this finding in table \ref{table:exampels_improv}\asafy{TO DO}, we present a few translations that exhibit the use of less typical pronouns
% that differ from the gold pronoun ( giving in Wino-X).Moreover, previous methods focused on non-pro drop languages like German and French where the candidate pronoun is mostly pronoun too. In partial pro-drop languages like Hebrew and Arabic, there are cases where the information of the pronoun can encode into a verb or a noun. Our methodology can account for such cases by reeling on the gender agreement between the candidate entity and candidate pronoun even though the candidate pronoun belongs to a different part of speech. Such examples also appear in \ref{table:exampels_improv}. \asafy{TO DO}
% In addition, figure \ref{}\asafy{TO DO} we present the part of speech distribution of the candidate pronoun. We emphasize that this capability is a clear advantage of our methodology compared to previous automatic metrics for pronoun translation.

% % and examples where the candidate pronoun is a noun or a verb that expresses the pronoun gender. We note that identifying valid pronoun translations is a known problem in the field of pronoun translation that mostly focuses on non-pro drop languages like German and French. Here we show that our methodology can handle even partial pro-drop languages like Hebrew and Russian or null-subject languages like Arabic.

% % We emphasize that while the way in which pronouns are used varies between translations, our consistency measure identifies a wide range of valid translations.\oa{didn't understand the last sent}\asafy{I rephrased the sentence}\ariec{it's still not clear. You should explain the phenomenon of multiple valid translations, then say that our method is agnostic to this problem as we look at consistency between entity and pronoun} To exemplify this finding in table \ref{table:exampels_improv}\ariec{I don't see the table.}, we present a few translations that exhibit the use of less typical pronouns or use inflection to nouns or verbs to convey the pronoun gender.\ariec{not clear, you should give an example (either here or in a table) of an english sentence with expected translation and another valid translation that changes the gender of the entity or the pronoun.} We note that identifying valid pronoun translations is a known problem in the field of pronoun translation that mostly focuses on non-pro drop languages like German and French. Here we show that our methodology can handle even partial pro-drop languages like Hebrew and Russian or null-subject languages like Arabic.\ariec{some of these terms weren't define above, assume that people don't know what is a null-subject or a partial pro-drop} In figure \ref{} we present the part of speech distribution per language of the candidate pronoun.\ariec{this sentence is out-of-context, you should explicitly say that this is an advantage of our method compared to pronoun translation.}


% % When translating the English pronoun we observe that  
% % Applying our method on set of six diverse languages give rise to the morphological differences between them. Specifically, the way different 
% % A known challenge of previous works is the shortcoming regarding the ability to identify valid alternative translations.
% % consistency instead of exact matches allowing us to treat a range of valid alternative translations and observe model behavior when encountering coreference resolution phenomena.
% % We want to emphasis that our method is able to identify vast variety of valid translation. In order to exemplified our 
%%%%%%%%% Improvement of Consistency %%%%%%%%%
% wino-x improvement:
% \subsection{Improving Consistency with Fine-tuning}
% \input{tables/wino-x/04_Wino-x_ours_con}
\input{tables/3_cons_ours_both}

Table~\ref{table:cons_ours} shows the target-side coreference consistency scores of all our fine-tuned models on \winox{} and \winomt{} (see App. \S\ref{sec:appendix:03_bug_results} for the performance on BUG, which follow similar trends).
%For both datasets, our fine-tuned models surpass the Opus-MT baseline model, with a negligible degradation in BLEU score, up to 0.33 points on average, which occurs when fine-tuning with explicit coreference markers. 
For both datasets, our fine-tuned models surpass the Opus-MT baseline model, 
% with a slight improvement in overall translation quality of $0.08\%$ in BERTScore and 0.0025 on COMET when fine-tuning with explicit coreference markers.
while preserving the overall translation quality, 
% when fine-tuning with explicit coreference markers 
as indicated by automatic measures such as BERTScore~\citep{bertscore} ($+0.08\%$) and COMET-20~\citep{rei-etal-2020-comet} ($+0.0025$).


\paragraph{Effect of augmented fine-tuning data.} The models fine-tuned on \emph{Coref data} (1) and \emph{Gender data} (3) outperform the Opus-MT baseline for all languages, both in Wino-X and WinoMT. This demonstrates that MT models learn implicitly linguistic phenomena from instances involving those phenomena. Furthermore, we point out that consistency scores on \winox{} are generally higher when fine-tuning on \emph{Coref data} (1, 2a, 2b) while WinoMT results are better when fine-tuning on \emph{Gender data} (3, 4a, 4b). This performance gap likely stems  from the similarity between WinoMT and \emph{Gender data} (as both include gendered pronouns), while Wino-X's like sentences with the pronoun ``it'' appear only in \emph{Coref data}. This further confirms the important role of fine-tuning data, which is in line with the observation of \citet{saunders-byrne-2020-reducing}, that smaller, more goal-oriented data is better for fine-tuning, compared to much larger but less focused data.



\paragraph{Effect of explicit coreference markers.} In the majority of our experiments (13/18), the explicit fine-tuning models (2a and 4a) outperform the implicit data augmentation approach when using the same augmented data (1 and 3) (see examples in Table \ref{table:lang_exampels} and App. \ref{sec:appendix:04_models_exampels}). These results suggest that an explicit monolingual signal can improve results more than an implicit signal. Results also show that the improvement is more pronounced when incorporating gold coreference markers (2b and 4b) instead of predicted markers (2a and 2b). Hence, applying more accurate coreference resolution models than the \emph{s2e} model will result in higher target-side consistency results. 



% We present results for our baseline MT model, Opus-MT, and our two fine-tuning approaches applied to two sets of augmented datasets. The first dataset is Coref dataset. The second dataset is the Gender dataset, a subset of Coref, which contains only sentences with coreference phenomena that involve gender pronouns. This dataset aims to address the characteristics of WinoMT and BUG, where most sentences use gender pronouns. For each fine-tuning data, we apply both our fine-tuning approaches, and use both predicted and gold markers at inference time. See App. \S\ref{sec:appendix:03_bug_results} for the performance on BUG. \gabis{This last paragraph was very confusing to me. What do we finetune on, and do we use for evaluation? Maybe we can consider omitting the gender part? is it very important? I think it adds a layer of complexity that is not warranted.}



% Results suggest that performance on \winox{} is generally better when finetuning\oa{finetuning with or without a hyphen/space? be consistent} on Coref data and WinoMT results are better when finetuning on Gender data. These results can indicate that the model's improvement depends on the specific coreference phenomena that it is exposed to in training.
%Coref data is unequivocal more beneficial for improvement on Wino-X than Gender data.
% For example, this performance gap may be due to the paucity of sentences containing coreference with the pronoun ``it'' in Gender data. Coref is also helpful for increasing performance on WinoMT, although in most cases it provides a more moderate improvement compared with Gender.  This result is aligned with the observation of \citet{saunders-byrne-2020-reducing}, that smaller, more goal-oriented data is better for fine-tuning.

% In the vast majority of our experiments, the explicit finetuning outperforms the implicit data augmentation approach when using the same data (Coref or Gender data). These results suggest that an explicit monolingual signal can improve results more than an implicit signal.

% Results also show that improvement is more pronounced when incorporating gold coreference markers instead of predicted markers. Although these results hold for both Wino-X and WinoMT, its effect is more noticeable in Wino-X. This is likely because of the low accuracy (about $ 60\%$) of \emph{s2e} on Wino-X, effecting the quality of the added markups. In comparison, \emph{s2e} achieved more than $ 80\%$ accuracy on WinoMT. Moreover, this model was found to generate fewer translations on Wino-X where the pronoun does not carry gender ($8\%$ on average).

%Our approach\oa{dont call it that; say something like the Opus-MT when fine tuned on ..} attain comparable or better results than top commercial and much bigger open-source MT models. Specifically 
% Applying our finetuning with gold coreference markers outperforms all other baseline MT models in German and Russian on both Wino-X and WinoMT, and achieves comparable results in all other target languages.

\input{tables/exampels_improvment}

% Table \ref{table:lang_exampels} presents an example where our approach improves translation consistency and quality. We note that these fine tuning procedures only incur a minor degradation in BLEU results, which is to be expected with dedicated finetuning which leads to semantic improvements not captured by BLEU \gabis{can we summarize it here so it doesn't seem like we're evading it? What's the maximum drop we observe?} \asafy{I add the next sentence, consider removing the corresponding app.} (see results on App. \S\ref{sec:appendix:02_bleu_results}).
% Specifically, fine-tuning on Gender data decrease the results by 0.25 and fine-tuning with coref markers cause a degradation of 0.33 on average when taking into account all available test sets from Opus-MT on the relevant languages. 

%Regarding fine tuning with explicit coreference markers compared with the implicit data augmentation method, we find that on most our experiments, 15 out of 18, the explicit fine tuning was found to be more beneficial. 
% We present experiments in which we apply the methods detailed in Section \ref{sec:improving} to improve the consistency of MT models. We start by analyzing our Wino-X experiments.\ariec{again -- since we unfiy the table, say that the table shows results for both dataset (add also a reference to the appendix for the results on BUG), then you can analyze them separetely or together, here it makes more sense to analyze them together as some findings (e.g predicted vs. gold markers) are similar for both datasets} In Table \ref{table:cons_ours} we present three sets of experiments. We apply our implicit and explicit fine-tuning approaches with both coreference\ariec{you mean predicted?} and gold markers on coref data and gender data.\ariec{this sounds like 2x2x2 experiments.. See also my comment in the improving section about the gender data}

% \ariec{the flow is not good, it looks like a concatenation of independent sentences. Compare the results in that explicit order (1) coref vs. gender data (Wino-X and WinoMT behave differently), (2) implicit vs. explicit approach (same for Wino-X and WinoMT), (3) predicted vs. gold}
%, leading to substantial gains in German and French

%Noticeably, the results are better when we use coref data as the pronoun ``it'' is lacking from gender data. Fine-tuning on coref data improves the models substantially in German and French. Moreover, fine-tuning with coreference markers provides additional improvement. Improvement is more pronounced when using gold coreference markers as the accuracy of \emph{s2e} on Wino-X is quite low (about $ 60\%$). Applying our fine-tuning with gold coreference markers improves over the baseline and outperforms all other commercial and open-source MT models in German and Russian.

% wino-mt improvement:
%Table \ref{table:cons_ours} present our consistency results on WinoMT. Here, we notice that most models fine-tuned on gender data perform better on WinoMT than ones trained on coref data. This result aligned with the observation of \citealt{saunders-byrne-2020-reducing}, that smaller more goal-oriented data is better for fine-tuning. We also observe that gold markers get smaller improvements than the improvements we saw in WinoMT as coreference resolvers achieve higher accuracy on WinoMT.\ariec{This is likely because of the high performance of the \emph{s2e} model on WinoMT} Our approaches achieves comparable or better results than top commercial and much bigger open-source MT models.\ariec{e.g XX vs. XX} In Table \ref{table:lang_exampels} we show examples where our approach improve translation consistency and quality. We note that our fine tuning has only minor effect on BLEU results (see results on App. \S\ref{sec:appendix:02_bleu_results}).\ariec{This is a really important point which is not related to WinoMT, maybe you can add a paragraph for that. }
% \input{tables/wino-mt/05_consistency_ours}

%Another evaluation study we did for estimating the improvement of our method
%\ariec{Move this paragraph after all the consistency results and add a subsection}

% In the first one, we fine-tuned our MT model on data with coreference phenomena, enriching the model with an implicit signal. In the second, we use our explicit approach of fine-tuning our MT model on the same data enrich with \emph{s2e}'s coreference markers. Then we use \emph{s2e} to produce coreference markers for evaluation data too. For the third experiment, we use the same fine-tuned MT model as in the second, but gold coreference markers are used in inference time.\oa{you should not repeat the description of these methods. just mark them with names and say here that we report results with them.}

%Results show that our method greatly improves consistency results across all languages. Outperforms all other MT models in German and Russian.%\oa{what outperforms what?} Fine-tuning on coreference data improves the models substantially in German and French. Moreover, Fine-tuning with coreference markers provides additional improvement. Improvement is more pronounced when using gold coreference markers as the accuracy of \emph{s2e} on Wino-X is quite low (about $ 60\%$).

\subsection{Analysis}

We turn to observing the empirical effect of the suggested fine-tuning strategies, using additional metrics.
For each sentence in Wino-X, we have the gold target pronoun that should appear in its translation. We use it to compute pronoun translation accuracy by comparing the candidate pronoun with the gold target pronoun. Table \ref{table:ours_pm_winox} presents the results. We can see that our method provides a large improvement over the baseline. Comparing these results against those of prominent open-source and commercial MT (see App. \S\ref{sec:appendix:01_gmf_pm}) shows that our approach outperforms other MT models in German and Russian, and is only second in French.
%\oa{I would make this a paragraph in the prev section}\asafy{not sure i understand what you meant by that, the opening or discard the new subsection title? or other alternative?}

%This section evaluates the impact of the fine-tuning methods on improving coreference performance according to previously proposed evaluation metrics.%\oa{is this true?}\asafy{it somewhat similar, see the two first sentences of the abstract here: https://aclanthology.org/W17-4802.pdf, still it sufficiently different that we can present it as sanity check or other measurement we add} In Wino-X we have a gold target pronoun annotated in the dataset. We use it to compute pronoun translation accuracy by comparing the candidate pronoun with the gold target pronoun. Table \ref{table:ours_pm_winox} presents the results. We can see that our method provides a large improvement over the baseline. Comparing these results against those of prominent open-source and commercial MT (see Table in App. \S\ref{sec:appendix:01_gmf_pm}) will show that our approach outperforms other MT models in German and Russian, and it is only second to mBART50 in French. % which surpasses all other models by a large margin. 
In WinoMT, \citet{stanovsky-etal-2019-evaluating} computed {\it gender accuracy} as the percentage of instances in which the translation preserved the gender of the entity from the original English sentence~(§\ref{sec:background}). Table \ref{table:ours_acc_wino-mt} shows that our approach improved gender accuracy results across all languages except Arabic.%\ariec{e.g +XX, +XX}

%\ariec{It's not other measures, but more a drill down to the gender accuracy}
Other metrics that \citet{stanovsky-etal-2019-evaluating} used, are $\Delta S$ and $\Delta G$. $\Delta S$  measures the difference in gender accuracy between stereotypical and non-stereotypical gender role assignments (as defined by \citealp{zhao-etal-2017-men}), and $\Delta G$ measures the difference in performance (F1 score) between source sentences with male and female entities. Our method decreases biases in both $\Delta S$ and $\Delta G$ by 5-6 points on average, indicating that the explicit signal helps the model in associating the pronoun with the coreferring entity, even in the presence of social and gender biases.

% \subsection{Human Validation}

% We estimate the accuracy of our consistency evaluation method by randomly sampling 50 translations of the Opus-MT model from all evaluation datasets and in all target languages, annotating each sample by a target language native speaker. The human annotators were asked to identify if the candidate pronoun is indeed the target pronoun and to verify is the gender prediction is correct. This way, we can account for both types of possible errors, i.e., alignment and gender extraction. 
% We compare the sentence-level human annotations to the output of our automatic method and find that the average agreement over all languages and datasets is above $90\%$ ( see full human validation results in Appendix \ref{sec:appendix:05_human_validation_results}). In the research of \citealp{stanovsky-etal-2019-evaluating} they used human validation to show that the alignment and gender prediction of the entity are reliable for $85\%$ of translations across all languages.%\ariec{what's the purpose of this sentence?}
% %\oa{this sentence is unclear; in what setting did they show it?}
% %Based on the combination of \citep{stanovsky-etal-2019-evaluating} with our evaluation we can safely say that our alignment and gender prediction are reliable. 
% From the combination of these two results we can conclude that our consistency scores are reliable.

% As \citealp{stanovsky-etal-2019-evaluating} noted, some errors occur when language-specific idiosyncrasies%\ariec{I don't know this word, what does it mean?} 
% introduce ambiguity to the morphological analysis. For example, gender for certain words in Hebrew cannot be distinguished without diacritics, and some pronouns in German are used in both masculine and neutral (e.g., sein) or feminine and third-person plural (e.g., ihr) forms. In addition, we notice that BUG sentences, specifically in partial pro-drop languages, were found to be more challenging for the alignment model~\ariec{can you explain why?}, and found to account for most mistakes in Hebrew and Arabic. This can be explained by the combination of noise in BUG sentences and the way that the pronoun is translated in partial pro-drop languages.
% %\ariec{I don't understand the purpose of this paragraph, if it's an analysis of the errors for each dataset, you should support these statements with numbers. }
% %\oa{I don't understand this sentence. you mean that the agreement on BUG was considerably higher than on the Winos? if so, say that}

%\input{tables/wino-x/Wino-x_gmf_pm}
\input{tables/wino-x/06_Wino-x_ours_pm}


\input{tables/wino-mt/07_acc_ours}

% \input{tables/Wino}
% \input{tables/BugGold}

==> sections/05_Related_Work.tex <==
The study of coreference has a long tradition in machine translation.
A long line of works uses pronoun translation as a way of measuring coreference since BLEU-based evaluation was shown to be insufficient for measuring improvement in coreference \citep{hardmeier-federico-2010-modelling}.

An alternative evaluation methodology uses automatic reference-based methods.  \citep{hardmeier-federico-2010-modelling} and \citep{miculicich-werlen-popescu-belis-2017-validation} proposed approaches that produce a score based on word alignment between pronouns in the source, reference translation, and translation output.
Later works show that those approaches don't correlate with human annotation, and it doesn't detect valid translations that use different pronouns than the reference \cite{guillou-hardmeier-2018-automatic}.
Consciously, other methods used a scoring-based evaluation approach that compares model scores of a predefined set of correct and incorrect translations and evaluates how often the model selects the correct option \citep{guillou-hardmeier-2016-protest, bawden-etal-2018-evaluating, muller-etal-2018-large, stojanovski-etal-2020-contracat, emelin-sennrich-2021-wino}. 

Our method is a reference-free approach that allows for three main advantages over past methods:  1) Evaluation of many target languages on several datasets, unlike most previous works which used limited data and a single language pair. 2) Detection of consistent translation even in cases where the part of speech of the pronoun translation is not a pronoun in the target language. Accordingly, we are the first to evaluate the coreference capabilities on partial pro-drop target languages. Moreover, this advantage indicates how our method overcomes the inability of previous methods to detect valid translations without the need for predefined candidate translations that are both costly to annotate and hard to cover most relevant candidates.
3) A black-box evaluation based on output translation alone that allows us to evaluate commercial models. Differently from past methods that used the perplexity or confidence of the model. 

Several previous methods aimed to improve the coreference abilities of MT models and reduce undesirable biases, by modifying the training data in ways that share some similarities with our method. \citet{vanmassenhove-etal-2018-getting} incorporate a ``speaker gender'' tag into training data, allowing gender to be conveyed at the sentence level. Similarly, \citet{moryossef-etal-2019-filling} added a prefix to disambiguate the coreference in the sentence. \citet{stojanovski-fraser-2018-coreference} advise an oracle-based approach to inject new tokens indicating the pronoun translation and its gender into the source sentence.
Our data enrichment method is novel in the way it incorporates coreference signal from coreference resolvers instead of additional meta-data. Thus we can use the model predictions in the inference stage as well.

==> sections/06_conclusion.tex <==
Our work is the first to present an automatic methodology for assessing the coreference capabilities of MT models, that can be applied in any target language and does not require any target side annotations. Furthermore, to the best of our knowledge, we are the first to conduct a large-scale multilingual coreference evaluation study on prominent open-source and commercial MT models, and compare them against state-of-the-art coreference resolvers on three challenging benchmarks. Finally, based on the superior results of coreference resolvers, we propose a novel approach to improve the coreference capabilities of MT models, that outperforms or achieves comparable results to strong and larger MT models. Despite this substantial gain, there is still a performance gap between our model and SOTA coreference resolvers, leaving much room for improvement. We hope that our work, and specifically our automatic evaluation methodology, will encourage future research to improve the coreference cabalities of MT models. 



%\oa{in what cases is it comparable?}
% We introduced a new evaluation methodology for coreference consistency in translation. Our methodology leverages the grammatical constraint that each mentions in the generated translation need to agree upon their morphological attributes, specifically gender. This measure allows us to provide an upper bound on the ability of MT models to perform coreference and enable a fair comparison of MT models and SOTA coreference resolvers. We evaluate several prominent open-source and commercial MT systems, translating from English to six target languages, and compare them to SOTA coreference resolvers on three challenging benchmarks. Our results showed that SOTA coreference resolvers are considerably better. Based on that result, we advise two novel fine-tuning approaches, for injecting coreference signals into MT models either implicitly or explicitly, using coreference resolvers. Our experiments showed that applying these approaches can provide compelling gains in consistency, as well as in other measures.\ariec{this looks like the abstract, it should be far much shorter}

Future work can expand our approach to account for number and person agreement phenomena, investigate how to extend our approach to more coreference clusters and more mentions per cluster in intra-sentential as well as inter-sentential settings. Moreover, we intend to investigate how different morphological attributes affect MT models' coreference abilities.
%\ariec{I don't understand this sentence.} 


%further research
% broader understating of the unique morphological effect on different languages
% extend to other attributes and more mentions
% extend our method to new domains

==> sections/08_limitation.tex <==
% We note that intrinsic limitation of our evaluation methodology is regarding the ability to treat pro-drop languages.
% In pro-drop languages like Spanish, the pronoun can be drooped without any other morphological indication to it's gender. In such cases, for sentences in WinoMT and BUG the only indication regarding the way the MT models understand the coreference relations in the source side is by the gender inflection of the profession.\ariec{in the paper, we didn't say that, we manage to evaluate consistency on these languages, while accuracy is a different measure.}
% - human validation of consistency as a whole.\ariec{??}

Even though our study presents the first large-scale multilingual coreference evaluation study in MT, it still has some limitations that could be addressed in future work. First, our methodology provides an upper bound to the coreference capabilities based on detecting gender valuations. While this could allow for a  controlled evaluation experiment, this upper bound can become non-indicative in cases where gender assignment is not a discriminative factor. This can be addressed by accounting for more semantic and syntactic constraints that the translation needs to follow (e.g., singular/plural agreement). 

Second, our setting addresses one entity and a single co-referring pronoun in the naturalistic sentences experiment. Our methodology could in principle be augmented to deal with more coreference clusters and mentions per cluster. Another possible extension is to include event coreference in addition to entity coreference. For example, in this work, we focus only on the anaphoric function of the pronoun ``it'' but further research can also examine the event function of ``it'' \citep{loaiciga-etal-2017-disambiguating}.




Third, MT models should generally produce translations with accurate gender inflection for all words. However, in this work, we focus on the \textit{coreference} capabilities of MT models by evaluating gender agreement between coreferring \textit{entity} mentions. Future research can extend our evaluation methodology to assess the gender inflection of verbs and adjectives translation (e.g., the gender of ``big'' and ``small'' in Figure~\ref{fig:method_new}), using additional tools and resources such as a semantic role labeling model and a dependency parser.




% and do not asses the gender inflection of verbs and adjectives translation (e.g., the gender of ``big'' and ``small'' in Figure~\ref{fig:method_new}). 
% Future research can incorporate a semantic role labeling model and dependency parsing to evaluate and improve MT models in producing more accurate translations.

Finally, although in Section \ref{sec:improving} we show big gains from the fine-tuning approach, it is clear that there is much room for improving the coreference capabilities of MT models, especially with regard to the performance of state-of-the-art coreference resolvers. We hope this work will help others develop MT models with better coreference capabilities.


==> tables/01_coref_models.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[tb!]
\centering
\resizebox{0.4\textwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
     & Wino-X & WinoMT & BUG \\
\midrule
SpanBERT            & 51.2     & 76.6 &  72.0 &  \\
\emph{s2e}          & \textbf{60.8}     & 81.7 &  72.2 &  \\
\textsc{LingMess}  & 58.7     & \textbf{83.7} &  \textbf{74.6} &  \\
\bottomrule
\end{tabular}}
\caption{Accuracy of SpanBERT, \emph{s2e} and \textsc{LingMess} model on our evaluation datasets. For simplicity, we report the accuracy on Wino-X sentences from the three languages as a single corpus, because there is a small difference between the languages (up to 0.3). }
\label{table:coref_models}
\end{table}





==> tables/2_cons_gmf_both.tex <==
\begin{table*}[!htb]
    % \caption{Global caption}
    \centering
    \scalebox{0.9}{
           \begin{tabular}{llll|rrrrrr}
            \toprule
            & \multicolumn{3}{c}{Wino-X} & \multicolumn{6}{c}{WinoMT} \\
            \midrule
             & en$\rightarrow$de        & en$\rightarrow$fr        & en$\rightarrow$ru &
              \multicolumn{1}{c}{en$\rightarrow$de} &
              \multicolumn{1}{c}{en$\rightarrow$es} &
              \multicolumn{1}{l}{en$\rightarrow$fr} &
              \multicolumn{1}{l}{en$\rightarrow$ru} &
              \multicolumn{1}{c}{en$\rightarrow$he} &
              \multicolumn{1}{c}{en$\rightarrow$ar} \\
            \midrule
            mBART50   & 37.4         & \textbf{56.6} & 44.6   & 77.7 & \textbf{75.2} & \textbf{73.3} & \textbf{57.7} & \textbf{69.3} & \textbf{69.5}\\
            M2M\_418M & 31.4         & 48.5          & \textbf{44.9} & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
            M2M\_1.2B & 36.8          & 45.2          & \textbf{44.9}    & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
            Google         & \textbf{41.3}& 36.3          & 40.7  & 69.9 & 59.4 & 65.5 & 57.9 & 60.1 & 69.2 \\
           % Microsoft      & 40.5         & 36.7          & 43.5  & 79.9 & 73.4 & 70.2 & \textbf{60.0}   & 66.6 & 64.2 \\
            Microsoft      & 40.5         & 36.7          & 43.5  & \textbf{78.0}   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 \\
            Opus-MT       & 37.4         & 35.3          & 43.6 & 68.2 & 56.0   & 63.2 & 49.8 & 59.0   & 59.8 \\
            \bottomrule
        \end{tabular}}
    \caption{Target-side consistency results of commercial and open-source MT systems on Wino-X and WinoMT when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy.}
    \label{table:cons_gmf}
\end{table*}

% \begin{table*}[!htb]
%     % \caption{Global caption}
%     \centering
%     \begin{minipage}{.4\linewidth}
%     %   \centering
%         \small
%         \begin{tabular}{llll}
%             \toprule
%                 & en$\rightarrow$de        & en$\rightarrow$fr        & en$\rightarrow$ru        \\
%                 %               & Con.            & Con.             & Con.             \\
%                 \midrule
%                 mBART50   & 37.4         & \textbf{56.6} & 44.6          \\
%                 M2M\_418M & 31.4         & 48.5          & \textbf{44.9}          \\
%                 M2M\_1.2B & 36.8          & 45.2          & \textbf{44.9}          \\
%                 Google         & \textbf{41.3}& 36.3          & 40.7          \\
%                 Microsoft      & 40.5         & 36.7          & 43.5          \\
%                 Opus-MT       & 37.4         & 35.3          & 43.6          \\
%             \bottomrule
%         \end{tabular}
%         \caption{Wino-X}
%     \end{minipage}%
%     % \centering
%     \begin{minipage}{.6\linewidth}
%     %   \centering
%       \small
%         \begin{tabular}{lrrrrrr}
%             \toprule
%              &
%               \multicolumn{1}{c}{en$\rightarrow$de} &
%               \multicolumn{1}{c}{en$\rightarrow$es} &
%               \multicolumn{1}{l}{en$\rightarrow$fr} &
%               \multicolumn{1}{l}{en$\rightarrow$ru} &
%               \multicolumn{1}{c}{en$\rightarrow$he} &
%               \multicolumn{1}{c}{en$\rightarrow$ar} \\
%             \midrule
%             mBART50   & \textbf{77.7} & \textbf{75.2} & \textbf{73.3} & 57.7 & \textbf{69.3} & \textbf{69.5} \\
%             M2M\_418M & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
%             M2M\_1.2B & 69.9 & 59.4 & 65.5 & 57.9 & 60.1 & 69.2 \\
%             Google         & 79.9 & 73.4 & 70.2 & \textbf{60.0}   & 66.6 & 64.2 \\
%             Microsoft      & 78.0   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 \\
%             Opus-MT       & 68.2 & 56.0   & 63.2 & 49.8 & 59.0   & 59.8 \\
%             \bottomrule
%         \end{tabular}
%         \caption{WinoMT}
%     \end{minipage} 
%     \caption{Target-side consistency results of commercial and open-source MT on Wino-X and WinoMT when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy.}
% \end{table*}

==> tables/3_cons_ours_both.tex <==
\begin{table*}[!htb]
    % \caption{Global caption}
    \centering
    \scalebox{0.9}{
           \begin{tabular}{llccc|cccccc}
            \toprule
            && \multicolumn{3}{c}{Wino-X} & \multicolumn{6}{c}{WinoMT} \\
            \midrule
             && en$\rightarrow$de        & en$\rightarrow$fr        & en$\rightarrow$ru &
              \multicolumn{1}{c}{en$\rightarrow$de} &
              \multicolumn{1}{c}{en$\rightarrow$es} &
              \multicolumn{1}{l}{en$\rightarrow$fr} &
              \multicolumn{1}{l}{en$\rightarrow$ru} &
              \multicolumn{1}{c}{en$\rightarrow$he} &
              \multicolumn{1}{c}{en$\rightarrow$ar} \\
            \midrule
                Opus-MT      && 37.4& 35.3& 43.6 & 67.6 & 56.0   & 63.2 & 49.8 & 59.0   & 59.8 \\
                Coref data (1)    && 42.7& 41.0& 44.0 & 74.4 & 58.0 & 67.1 & \textbf{62.1} & 68.1 & 67.1 \\
                $+$coref markers (2a)   && 44.1& 42.6& 45.5 & 76.0 & 58.2 & 67.2 & 57.7 & 68.7   & 67.9 \\
                $+$gold markers (2b)  && \textbf{44.7} & \textbf{45.8}& \textbf{50.5}   & 77.6 & 58.2 & 67.3 & 58.6 & 69.8   & \textbf{68.9} \\
                Gender data (3)   && 41.2&37.0&45.0 & 75.0 &60.6& 68.3 & 61.6 & 68.1 & 66.2 \\
                $+$coref markers (4a)      && 43.6 & 36.6 & 43.8 &  78.7 & 60.1 & \textbf{68.6} & 58.4 & 69.0   & 60.9 \\
                $+$gold markers (4b)       && 42.9 & 36.7 & 46.3 & \textbf{80.6} & \textbf{60.8} & 68.4 & 59.6 & \textbf{69.9}   & 62.2 \\
            \bottomrule
        \end{tabular}}
    \caption{Target-side consistency results of the Opus-MT baseline and our fine-tuning experiments on Wino-X and WinoMT when translating into different languages. For both datasets, our fine-tuned models surpass the baseline.\vspace{-.3cm}}
    \label{table:cons_ours}
\end{table*}



















% % \begin{tabular}{llll}
% % \toprule
% %               & German         & French         & Russian        \\
% % %               & PM             & PM             & PM             \\
% % \midrule
% % mBART50   & 38.1          & \textbf{47.2} & 34.7          \\
% % M2M00\_418M & 33.8          & 39.5          & 32.4          \\
% % M2M100\_1.2B & 38.5          & 39.0          & 33.7          \\
% % Google         & \textbf{44.2}          & 34.8          & 35.8          \\
% % Microsoft      & 43.1          & 35.7          & \textbf{37.8}           \\
% % EasyNMT       & 39.9          & 31.8          & 37.0             \\
% % % random data    & 40.78          & 35.14          & 34.63          \\
% % % coref data     & 42.26          & 38.86          & 34.99          \\
% % % "+signal       & 43.59          & 39.32          & 37.22          \\
% % % "+gold         & \textbf{45.71} & 42.7           & \textbf{42.63} \\
% % \bottomrule
% % \end{tabular}
% % \quad
% % \begin{tabular}{llll}
% % \toprule
% %               & German         & French         & Russian        \\
% % %               & PM             & PM             & PM             \\
% % \midrule
% % mBART50   & 38.1          & \textbf{47.2} & 34.7          \\
% % M2M00\_418M & 33.8          & 39.5          & 32.4          \\
% % M2M100\_1.2B & 38.5          & 39.0          & 33.7          \\
% % Google         & \textbf{44.2}          & 34.8          & 35.8          \\
% % Microsoft      & 43.1          & 35.7          & \textbf{37.8}           \\
% % EasyNMT       & 39.9          & 31.8          & 37.0             \\
% % % random data    & 40.78          & 35.14          & 34.63          \\
% % % coref data     & 42.26          & 38.86          & 34.99          \\
% % % "+signal       & 43.59          & 39.32          & 37.22          \\
% % % "+gold         & \textbf{45.71} & 42.7           & \textbf{42.63} \\
% % \bottomrule
% % \end{tabular}

% \begin{table*}[!htb]
%     % \caption{Global caption}
%     \centering
%     \begin{minipage}{.4\linewidth}
%     %   \centering
%         \small
%         \begin{tabular}{llll}
%         \toprule
%                       & en$\rightarrow$de        & en$\rightarrow$fr         & en$\rightarrow$ru        \\
%         \midrule
%         Opus-MT      & 37.4         & 35.3          & 43.6          \\
%         %random data    & 39.9         & 38.4          & 42.1          \\
%         coref data     & 42.7         & 41.0          & 44.0          \\
%         $+$coref markers       & 44.1         & 42.6          & 45.5          \\
%         $+$gold markers        & \textbf{44.7} & \textbf{45.8}          & \textbf{50.5} \\
%         \bottomrule
%         \end{tabular}
%         \caption{Wino-X}
%     \end{minipage}%
%     % \centering
%     \begin{minipage}{.6\linewidth}
%     %   \centering
%         \small
%         \begin{tabular}{lrrrrrr}
%         \toprule
%         %  &
%         %   \multicolumn{1}{c}{German} &
%         %   \multicolumn{1}{c}{Spanish} &
%         %   \multicolumn{1}{l}{French} &
%         %   \multicolumn{1}{l}{Russian} &
%         %   \multicolumn{1}{c}{Hebrew} &
%         %   \multicolumn{1}{c}{Arabic} \\
%         &
%           \multicolumn{1}{c}{en$\rightarrow$de} &
%           \multicolumn{1}{c}{en$\rightarrow$es} &
%           \multicolumn{1}{l}{en$\rightarrow$fr} &
%           \multicolumn{1}{l}{en$\rightarrow$ru} &
%           \multicolumn{1}{c}{en$\rightarrow$he} &
%           \multicolumn{1}{c}{en$\rightarrow$ar} \\
%         \midrule
%         % mbart50\_m2m   & 77.7 & 75.2 & 73.3 & 57.7 & 69.3 & 69.5 \\
%         % m2m\_100\_418M & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
%         % m2m\_100\_1.2B & 69.9 & 59.4 & 65.5 & 57.9 & 60.1 & 69.2 \\
%         % Google         & 79.9 & 73.4 & 70.2 & 60   & 66.6 & 64.2 \\
%         % Microsoft      & 78   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 \\
%         Opus-MT       & 68.2 & 56.0   & 63.2 & 49.8 & 59   & 59.8 \\
%         % random data    & 68.2 & 59.2 & 66   & 65.4 & 67.8 & 64.5 \\
%         Gender data     & 75.1 & \textbf{60.6} & 68.3 & \textbf{61.6} & 68.1 & \textbf{66.2} \\
%         $+$coref markers       & \textbf{78.5} & 60.1 & \textbf{68.6} & 58.4 & \textbf{69.0}   & 60.9 \\
%         %\quad$+$gender         & \textbf{79.3} & 60   & \textbf{69.1} & 60.9 & 68.5 & 62.7 \\
%         \bottomrule
%         \end{tabular}
%         \caption{WinoMT}
%     \end{minipage} 
%     \caption{Target-side consistency results of our fine-tuning approaches on Wino-X and WinoMT when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy.}
% \end{table*}

==> tables/BLEU/bleu_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrrrrrr}
\toprule
%  &
%   \multicolumn{1}{c}{German} &
%   \multicolumn{1}{c}{Spanish} &
%   \multicolumn{1}{l}{French} &
%   \multicolumn{1}{l}{Russian} &
%   \multicolumn{1}{c}{Hebrew} &
%   \multicolumn{1}{c}{Arabic} \\
&
  \multicolumn{1}{c}{de} &
  \multicolumn{1}{c}{es} &
  \multicolumn{1}{l}{fr} &
  \multicolumn{1}{l}{ru} &
  \multicolumn{1}{c}{he} &
  \multicolumn{1}{c}{ar} \\
\midrule
Opus-MT        & 32.6 & 29.0 & 34.2 & 26.8 & 40.0 & 21.2 \\
% random\_text\_g & 32.656 & 28.5723 & 34.1957 & 26.435  & 35.78 & 24.69 \\
gender data  & 32.6 & 28.6 & 34.2 & 26.2 & 36.0 & 23.2 \\
$+$coref markers        & 32.4 & 28.6   & 34.1 & 26.2 & 35.9 & 23.0 \\
\bottomrule
\end{tabular}}
\caption{BLEU results of our fine tuning approaches on OPUS test data.}
\label{table:bleu}
\end{table}

==> tables/BUG/08_gmp_cons.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[tb!]
\centering
\begin{tabular}{lrrrrrr}
\toprule
%  &
%   \multicolumn{1}{c}{German} &
%   \multicolumn{1}{c}{Spanish} &
%   \multicolumn{1}{l}{French} &
%   \multicolumn{1}{l}{Russian} &
%   \multicolumn{1}{c}{Hebrew} &
%   \multicolumn{1}{c}{Arabic} \\
 &
  \multicolumn{1}{c}{en$\rightarrow$de} &
  \multicolumn{1}{c}{en$\rightarrow$es} &
  \multicolumn{1}{l}{en$\rightarrow$fr} &
  \multicolumn{1}{l}{en$\rightarrow$ru} &
  \multicolumn{1}{c}{en$\rightarrow$he} &
  \multicolumn{1}{c}{en$\rightarrow$ar} \\
\midrule
mBART50         & 74.6 & 69.4 & 76.0 & 69.1 & 80.2 & 83.0 \\
M2M\_418M       & 81.3 & 84.9 & 86.0 & \textbf{71.6} & 83.6 & 85.1 \\
M2M\_1.2B       & \textbf{83.5} & 85.1 & \textbf{90.3} & 70.4 & \textbf{89.6} & \textbf{93.4} \\
Google          & 56.0 & 84.4 & 89.2 & 71.0 & 85.2 & 91.9 \\
Microsoft       & 77.2 & \textbf{86.7} & 86.0 & 67.2 & 84.0 & 89.8 \\
Opus-MT         & 79.8 & 85.1 & 86.2 & 67.3 & 88.8 & 88.0 \\

% mBART50   & \textbf{77.7} & \textbf{75.2} & \textbf{73.3} & 57.7 & \textbf{69.3} & \textbf{69.5} \\
% M2M\_418M & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
% M2M\_1.2B & 69.9 & 59.4 & 65.5 & 57.9 & 60.1 & 69.2 \\
% Google         & 79.9 & 73.4 & 70.2 & \textbf{60.0}   & 66.6 & 64.2 \\
% Microsoft      & 78.0   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 \\
% Opus-MT       & 68.2 & 56.0   & 63.2 & 49.8 & 59.0   & 59.8 \\
% random data    & 68.2 & 59.2 & 66   & 65.4 & 67.8 & 64.5 \\
% coref data     & 75.1 & 60.6 & 68.3 & 61.6 & 68.1 & 66.2 \\
% +signal       & 78.5 & 60.1 & 68.6 & 58.4 & 69   & 60.9 \\
% +gold         & 79.3 & 60   & 69.1 & 60.9 & 68.5 & 62.7 \\
\bottomrule
\end{tabular}
\caption{Target-side consistency results of commercial and open-source MT on BUG when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy.}
%\gabis{consider merging with Table~\ref{table:gmf_cons_winox}}}
\label{table:gmf_cons_BUG}
\end{table*}







% % Please add the following required packages to your document preamble:
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[]
% \begin{tabular}{lrrrrrr}
%  &
%   \multicolumn{1}{c}{de} &
%   \multicolumn{1}{c}{es} &
%   \multicolumn{1}{c}{fr} &
%   \multicolumn{1}{c}{ru} &
%   \multicolumn{1}{c}{he} &
%   \multicolumn{1}{c}{ar} \\
%  &
%   \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &
%   \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} \\
% mBART50         & 74.6 & 69.4 & 76   & 69.1 & 80.2 & 83   \\
% M2M100\_\_418M  & 81.3 & 84.9 & 86   & 71.6 & 83.6 & 85.1 \\
% M2M100\_1.2B    & 83.5 & 85.1 & 90.3 & 70.4 & 89.6 & 93.4 \\
% Google          & 56   & 84.4 & 89.2 & 71   & 85.2 & 91.9 \\
% Microsoft       & 77.2 & 86.7 & 86   & 67.2 & 84   & 89.8 \\
% EasyNMT         & 79.8 & 85.1 & 86.2 & 67.3 & 88.8 & 88   \\
% random\_data    & 81.8 & 88.1 & 86.8 & 69.2 & 89.3 & 90.5 \\
% gender data     & 84.1 & 87.4 & 88.7 & 69.9 & 90.2 & 91.3 \\
% "+coref signal  & 84.2 & 87.4 & 88.8 & 70.1 & 89.8 & 91.8 \\
% "+gender signal & 82.2 & 0    & 86.5 & 66.6 & 0    & 0   
% \end{tabular}
% \end{table}

==> tables/big_tables/BugGold.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{@{}lccccccccccccccccccc@{}}
% \begin{tabular}{lcccccccccccccccc}
\toprule
&& \multicolumn{3}{c}{German}& \multicolumn{1}{c}{Spanish}& \multicolumn{3}{c}{French}& \multicolumn{3}{c}{Russian}& \multicolumn{3}{c}{Hebrew}& \multicolumn{3}{c}{Arabic} \\
&& {EC} & {Acc.} & {A\&C} & {Acc.} & {EC} & {Acc.} & {A\&C} & {EC} & {Acc.} & {A\&C} & {EC} & {Acc.} & {A\&C} & {EC} & {Acc.} & {A\&C} \\
\midrule
mbart50\_m2m    && 66.5& 79& 66.2& 67.5& 26.3& 75.3& 25.6& \textbf{45.4}& 83.9& 48.6& \textbf{62.2}& 80.4& 61.9& 60.6& 84.3& 59.4\\
m2m\_100\_418M  && 62.6& 68.7& 59.7& 59.6& 22.9& 64.8& 21.9& 42.1& 76.8& 43.9& 58.1& 77.5& 56.6& 55.2& 76.7& 52.7\\
m2m\_100\_1.2B  && 67.4& 78.9& 66.6& 66.2& 25.5& 73& 25& 44.7& 84.7& 49& 55.6& 79.2& 54.3& 49.2& 71.1& 44.1\\
google          && 66& \textbf{81.5}& 65.3& 68.2& 26.4& 76.5& 25.5& 40& 83.8& 43.2& 56.4& \textbf{86.6}& 56.5& \textbf{65.1}& 88.4& \textbf{65}\\
microsoft       && 3.6& 77.5& 3.1& 68.3& \textbf{26.8}& \textbf{77.8}& \textbf{26}& 44.4& \textbf{86.4}& \textbf{49}& 57.1& 83.6& \textbf{57.2}& \textbf{65.1}& \textbf{87.3}& 64.8\\
\midrule
EasyNMT (baseline)        && 64.7& 76.2& 64.7& 66.5& 26.2& 74.4& 25.8& 40.8& 78.6& 44.2& 55.5& 82& 55.5& 58.5& 80.6& 58\\
Random data    && 66& 77.3& 65.6& 66.4& 25.2& 73.2& 24.8& 40.4& 78.3& 43& 57.3& 82.1& 57& 59.1& 80.7& 58.6\\
Gender data     && 67.1& 79.4& 66.7& 67.8& 24.9& 73.8& 24.4& 41.6& 80& 44.9& 56.7& 84.6& 56.6& 62.3& 84.1& 61.8\\
\quad$+$coref signal  && \textbf{68.6}& 81.1& \textbf{68.1}& 68& 26.5& 75.2& 25.8& 42& 81& 45.2& 57.4& 85.2& 57.1& 62.7& 84.1& 62\\
\quad$+$gender signal && 68.3& 81& 67.7& \textbf{68.4}& 26.3& 74.8& 25.6& 42.5& 81.3& 46.2& 57.1& 84.4& 56.8& 63.5& 84.6& 62.9 \\
\bottomrule
\end{tabular}}
  \caption{Results on BugGold.}
\end{table*}


==> tables/big_tables/Wino-X.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
\centering
\resizebox{0.92\textwidth}{!}{
  \begin{tabular}{@{}lccccccccccccc@{}}
    \toprule
    && \multicolumn{3}{c}{German}  && \multicolumn{3}{c}{French} && \multicolumn{3}{c}{Russian} \\
    && IC & EC & PM && IC & EC & PM && IC & EC & PM \\ 
    \midrule
    && \multicolumn{9}{c}{Commercial and large open source models} \\
    \midrule
    mbart50\_m2m    && 39.03  & 37.44 & 38.05 && 62.48 & \textbf{56.69} & \textbf{47.19} && 52.14  & 44.68 & 34.72          \\
    m2m\_100\_418M  && 33.15 & 31.43  & 33.73 && 64.42 & 48.56 & 39.52 && 51.83 & 44.95 & 32.44 \\
    m2m\_100\_1.2B  && 38.29 & 36.8 & 38.53 && 63.32 & 45.25 & 39.02 && 50.18 & 44.95 & 33.65 \\
    Google          && 44.78 & 41.34 & 44.17 && 65.70 & 36.38 & 34.84 && 53.75 & 40.71 & 35.84 \\
    Microsoft       && 42.85 & 40.57 & 43.14 && 63.29 & 36.78 & 35.68 && 49.11 & 43.57 & 37.8 \\ 
    \midrule
        && \multicolumn{9}{c}{Our method} \\
    \midrule
    EasyNMT (baseline) && 39.11 & 37.44 & 39.85 && \textbf{66.03} & 35.34 & 31.79 && 48.70 & 43.61 & 37.00 \\
    Random data     && 42.34 & 39.96 & 40.78 && 64.12 & 38.42 & 35.14 && 48.08 & 42.14 & 34.63 \\
    Coref data      && 45.87 & 42.77 & 42.26 && 62.28 & 41.03 & 38.86 && 47.77 & 44.06 & 34.99 \\
    \quad$+$signal         && 47.62 & 44.14 & 43.59 && 62.08 & 42.67 & 39.32 && 48.79 & 45.53 & 37.22 \\
    \quad$+$gold           && \textbf{47.99} & \textbf{44.7} & \textbf{45.71} && 65.56 & 45.82 & 42.70 && \textbf{53.53} & \textbf{50.58} & \textbf{42.63} \\
    \bottomrule
  \end{tabular}}
  \caption{Results on Wino-X for German, French and Russian. IC- Implicate Consistency is EC but forgiving for unk pronoun, EC- Explicit Consistency is the antecedent and pronoun having the same gender,  and PM - is Pronoun Match with gold pronoun. \ariec{Explain what is IC, EC and PM. Write the main outcomes from these results. Explain also the difference between the top and the bottom models. Also, it's not cleat that Random and Coref are fine-tuned models of easynmt. General comment: do we really need two decimals?}}
\end{table*}

==> tables/big_tables/Wino.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{@{}lccccccccccccccccccc@{}}
% \begin{tabular}{lcccccccccccccccc}
\toprule
&& \multicolumn{3}{c}{German}& \multicolumn{1}{c}{Spanish}& \multicolumn{3}{c}{French}& \multicolumn{3}{c}{Russian}& \multicolumn{3}{c}{Hebrew}& \multicolumn{3}{c}{Arabic} \\
&& {EC} & {Acc.} & {A\&C} & {Acc.} & {EC} & {Acc.} & {A\&C} & {EC} & {Acc.} & {A\&C} & {EC} & {Acc.} & {A\&C} & {EC} & {Acc.} & {A\&C} \\
\midrule
mbart50\_m2m && 68.6 & 75.4 & 68.3 & \textbf{74.5} & \textbf{44.4} & \textbf{69} & \textbf{43.8} & 49.5 & 55.7 & \textbf{48.6} & \textbf{60.1} & \textbf{66} & \textbf{59.9} & \textbf{47} & 63.7 & 43.6 \\
m2m\_100\_418M && 60.9 & 63.5 & 58.5 & 57.1 & 39.5 & 53.3 & 35.4 & 46.4 & 50.5 & 44 & 49.7 & 54.6 & 48.9 & 43.7 & 55.3 & 38 \\
m2m\_100\_1.2B && 62.5 & 64.2 & 59.7 & 62 & 39.3 & 56.1 & 36.7 & 48.6 & 54.9 & 46.2 & 51.2 & 55.4 & 48.9 & 48.1 & 50 & 33 \\
Google && 70.6 & \textbf{78.7} & 70.4 & 71.9 & 42.5 & 66 & 42.1 & 48.7 & \textbf{59.8} & 48.5 & 54.6 & 64.9 & 54.7 & 45.8 & \textbf{64.3} & \textbf{45.5} \\
Microsoft && 69.7 & 76.7 & 69.5 & 67.9 & 40.4 & 64.6 & 40.1 & 49.1 & 56.6 & 48.7 & 54 & 61.8 & 54.1 & 42.8 & 61.3 & 42.4 \\
\midrule
EasyNMT  (baseline) && 60.4 & 66 & 60.3 & 60.4 & 38.6 & 56.5 & 38 & 42 & 50.2 & 41.6 & 50.4 & 56.6 & 50.4 & 42.4 & 59.8 & 42.2 \\
Random data && 60.6 & 65.8 & 60.1 & 63.1 & 40.3 & 58 & 39.6 & \textbf{52.2} & 49.3 & 40.1 & 55.8 & 57.8 & 49.7 & 44.5 & 58.5 & 41.7 \\
Gender data && 66.8 & 73.3 & 66.5 & 66.7 & 42 & 60.3 & 41.4 & 49.2 & 52.4 & 42.2 & 56.4 & 60.9 & 52.2 & 45.9 & 59.7 & 42.7 \\
\quad$+$coref signal && 69.7 & 76.8 & 69.2 & 67.9 & 41.9 & 60.1 & 41 & 48 & 53.2 & 43.9 & 57.2 & 63.5 & 54.3 & 41.6 & 55.6 & 38.5 \\
\quad$+$gender && \textbf{70.6} & 77.6 & \textbf{70.1} & 68.4 & 42.2 & 61.1 & 41.4 & 49.3 & 53.3 & 43.3 & 57 & 63.3 & 54.5 & 43.4 & 57.5 & 40.4 \\
\bottomrule
\end{tabular}}
  \caption{Results on WinoMT.}
\end{table*}




==> tables/big_tables/wino-x_gmf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
\centering
\resizebox{0.92\textwidth}{!}{
  \begin{tabular}{@{}lccccccccccccc@{}}
    \toprule
    && \multicolumn{3}{c}{German}  && \multicolumn{3}{c}{French} && \multicolumn{3}{c}{Russian} \\
    && IC & EC & PM && IC & EC & PM && IC & EC & PM \\ 
    \midrule
    && \multicolumn{9}{c}{Commercial and large open source models} \\
    \midrule
    mbart50\_m2m    && 39.03  & 37.44 & 38.05 && 62.48 & \textbf{56.69} & \textbf{47.19} && 52.14  & 44.68 & 34.72          \\
    m2m\_100\_418M  && 33.15 & 31.43  & 33.73 && 64.42 & 48.56 & 39.52 && 51.83 & 44.95 & 32.44 \\
    m2m\_100\_1.2B  && 38.29 & 36.8 & 38.53 && 63.32 & 45.25 & 39.02 && 50.18 & 44.95 & 33.65 \\
    Google          && 44.78 & 41.34 & 44.17 && 65.70 & 36.38 & 34.84 && 53.75 & 40.71 & 35.84 \\
    Microsoft       && 42.85 & 40.57 & 43.14 && 63.29 & 36.78 & 35.68 && 49.11 & 43.57 & 37.8 \\ 
    \bottomrule
  \end{tabular}}
\end{table*}

==> tables/big_tables/wino-x_ours.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}
\centering
\resizebox{0.92\textwidth}{!}{
  \begin{tabular}{@{}lccccccccccccc@{}}
    \toprule
    && \multicolumn{3}{c}{German}  && \multicolumn{3}{c}{French} && \multicolumn{3}{c}{Russian} \\
    && IC & EC & PM && IC & EC & PM && IC & EC & PM \\ 
    \midrule
            && \multicolumn{9}{c}{Our method} \\
    \midrule
    EasyNMT (baseline) && 39.11 & 37.44 & 39.85 && \textbf{66.03} & 35.34 & 31.79 && 48.70 & 43.61 & 37.00 \\
    % Random data     && 42.34 & 39.96 & 40.78 && 64.12 & 38.42 & 35.14 && 48.08 & 42.14 & 34.63 \\
    Coref data      && 45.87 & 42.77 & 42.26 && 62.28 & 41.03 & 38.86 && 47.77 & 44.06 & 34.99 \\
    \quad$+$signal         && 47.62 & 44.14 & 43.59 && 62.08 & 42.67 & 39.32 && 48.79 & 45.53 & 37.22 \\
    \quad$+$gold           && \textbf{47.99} & \textbf{44.7} & \textbf{45.71} && 65.56 & 45.82 & 42.70 && \textbf{53.53} & \textbf{50.58} & \textbf{42.63} \\
    \bottomrule
  \end{tabular}}
\end{table*}

==> tables/data/train.tex <==
\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lllllll}
\toprule
            & de   & es   & fr   & ru   & he   & ar   \\
\midrule
Coref data  & 500K & 744K & 761K & 149K & 1.1M & 1.4M \\
Gender data & 38K  & 50K  & 51K  & 19K  & 265K & 268K \\
\bottomrule
\end{tabular}}
\caption{Number of fine-tuning instances in \emph{Coref Data} (requiring some sort of coreference resolution) and \emph{Gender data} (requiring coreference resolution with some gendered pronoun) for each target language.}
\label{table:data_train}
\end{table}

==> tables/data/val.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\centering
\begin{tabular}{lr}
\toprule
Dataset  & \#sentences \\
\midrule
Wino-X (en $\rightarrow$ de) & 3,774 \\
Wino-X (en $\rightarrow$ fr) & 2,988 \\
Wino-X (en $\rightarrow$ ru) & 2,238 \\
WinoMT      & 3,888 \\
BUG         & 1,717 \\
\bottomrule
\end{tabular}
\caption{Statistics of our evaluation datasets. Note that in all datasets we use the corresponding English source-side sentences as our input.}
\label{table:data_val}
\end{table}

==> tables/try.tex <==
% % \begin{tabular}{llll}
% % \toprule
% %               & German         & French         & Russian        \\
% % %               & PM             & PM             & PM             \\
% % \midrule
% % mBART50   & 38.1          & \textbf{47.2} & 34.7          \\
% % M2M00\_418M & 33.8          & 39.5          & 32.4          \\
% % M2M100\_1.2B & 38.5          & 39.0          & 33.7          \\
% % Google         & \textbf{44.2}          & 34.8          & 35.8          \\
% % Microsoft      & 43.1          & 35.7          & \textbf{37.8}           \\
% % EasyNMT       & 39.9          & 31.8          & 37.0             \\
% % % random data    & 40.78          & 35.14          & 34.63          \\
% % % coref data     & 42.26          & 38.86          & 34.99          \\
% % % "+signal       & 43.59          & 39.32          & 37.22          \\
% % % "+gold         & \textbf{45.71} & 42.7           & \textbf{42.63} \\
% % \bottomrule
% % \end{tabular}
% % \quad
% % \begin{tabular}{llll}
% % \toprule
% %               & German         & French         & Russian        \\
% % %               & PM             & PM             & PM             \\
% % \midrule
% % mBART50   & 38.1          & \textbf{47.2} & 34.7          \\
% % M2M00\_418M & 33.8          & 39.5          & 32.4          \\
% % M2M100\_1.2B & 38.5          & 39.0          & 33.7          \\
% % Google         & \textbf{44.2}          & 34.8          & 35.8          \\
% % Microsoft      & 43.1          & 35.7          & \textbf{37.8}           \\
% % EasyNMT       & 39.9          & 31.8          & 37.0             \\
% % % random data    & 40.78          & 35.14          & 34.63          \\
% % % coref data     & 42.26          & 38.86          & 34.99          \\
% % % "+signal       & 43.59          & 39.32          & 37.22          \\
% % % "+gold         & \textbf{45.71} & 42.7           & \textbf{42.63} \\
% % \bottomrule
% % \end{tabular}

\begin{table*}[!htb]
    % \caption{Global caption}
    \centering
    \begin{minipage}{.5\linewidth}
    %   \centering
        \small
        \begin{tabular}{llll}
            \toprule
                & en$\rightarrow$de        & en$\rightarrow$fr        & en$\rightarrow$ru        \\
                %               & Con.            & Con.             & Con.             \\
                \midrule
                mBART50   & 37.4         & \textbf{56.6} & 44.6          \\
                M2M\_418M & 31.4         & 48.5          & \textbf{44.9}          \\
                M2M\_1.2B & 36.8          & 45.2          & \textbf{44.9}          \\
                Google         & \textbf{41.3}& 36.3          & 40.7          \\
                Microsoft      & 40.5         & 36.7          & 43.5          \\
                Opus-MT       & 37.4         & 35.3          & 43.6          \\
            \bottomrule
        \end{tabular}
        \caption{Wino-X}
    \end{minipage}%
    % \centering
    \begin{minipage}{.5\linewidth}
    %   \centering
      \small
        \begin{tabular}{rrrrrr}
            \toprule
             
              \multicolumn{1}{c}{en$\rightarrow$de} &
              \multicolumn{1}{c}{en$\rightarrow$es} &
              \multicolumn{1}{l}{en$\rightarrow$fr} &
              \multicolumn{1}{l}{en$\rightarrow$ru} &
              \multicolumn{1}{c}{en$\rightarrow$he} &
              \multicolumn{1}{c}{en$\rightarrow$ar} \\
            \midrule
            \textbf{77.7} & \textbf{75.2} & \textbf{73.3} & 57.7 & \textbf{69.3} & \textbf{69.5} \\
            69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
            69.9 & 59.4 & 65.5 & 57.9 & 60.1 & 69.2 \\
            79.9 & 73.4 & 70.2 & \textbf{60.0}   & 66.6 & 64.2 \\
            78.0   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 \\
            68.2 & 56.0   & 63.2 & 49.8 & 59.0   & 59.8 \\
            \bottomrule
        \end{tabular}
        \caption{WinoMT}
    \end{minipage} 
    \caption{Target-side consistency results of commercial and open-source MT on Wino-X and WinoMT when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy.}
\end{table*}

==> tables/try2.tex <==
% % \begin{tabular}{llll}
% % \toprule
% %               & German         & French         & Russian        \\
% % %               & PM             & PM             & PM             \\
% % \midrule
% % mBART50   & 38.1          & \textbf{47.2} & 34.7          \\
% % M2M00\_418M & 33.8          & 39.5          & 32.4          \\
% % M2M100\_1.2B & 38.5          & 39.0          & 33.7          \\
% % Google         & \textbf{44.2}          & 34.8          & 35.8          \\
% % Microsoft      & 43.1          & 35.7          & \textbf{37.8}           \\
% % EasyNMT       & 39.9          & 31.8          & 37.0             \\
% % % random data    & 40.78          & 35.14          & 34.63          \\
% % % coref data     & 42.26          & 38.86          & 34.99          \\
% % % "+signal       & 43.59          & 39.32          & 37.22          \\
% % % "+gold         & \textbf{45.71} & 42.7           & \textbf{42.63} \\
% % \bottomrule
% % \end{tabular}
% % \quad
% % \begin{tabular}{llll}
% % \toprule
% %               & German         & French         & Russian        \\
% % %               & PM             & PM             & PM             \\
% % \midrule
% % mBART50   & 38.1          & \textbf{47.2} & 34.7          \\
% % M2M00\_418M & 33.8          & 39.5          & 32.4          \\
% % M2M100\_1.2B & 38.5          & 39.0          & 33.7          \\
% % Google         & \textbf{44.2}          & 34.8          & 35.8          \\
% % Microsoft      & 43.1          & 35.7          & \textbf{37.8}           \\
% % EasyNMT       & 39.9          & 31.8          & 37.0             \\
% % % random data    & 40.78          & 35.14          & 34.63          \\
% % % coref data     & 42.26          & 38.86          & 34.99          \\
% % % "+signal       & 43.59          & 39.32          & 37.22          \\
% % % "+gold         & \textbf{45.71} & 42.7           & \textbf{42.63} \\
% % \bottomrule
% % \end{tabular}

\begin{table*}[!htb]
    % \caption{Global caption}
    \centering
    \scalebox{0.9}{
           \begin{tabular}{llll|rrrrrr}
            \toprule
            & \multicolumn{3}{c}{Wino-X} & \multicolumn{6}{c}{WinoMT} \\
            \midrule
             & en$\rightarrow$de        & en$\rightarrow$fr        & en$\rightarrow$ru &
              \multicolumn{1}{c}{en$\rightarrow$de} &
              \multicolumn{1}{c}{en$\rightarrow$es} &
              \multicolumn{1}{l}{en$\rightarrow$fr} &
              \multicolumn{1}{l}{en$\rightarrow$ru} &
              \multicolumn{1}{c}{en$\rightarrow$he} &
              \multicolumn{1}{c}{en$\rightarrow$ar} \\
            \midrule
            mBART50   & 37.4         & \textbf{56.6} & 44.6   & \textbf{77.7} & \textbf{75.2} & \textbf{73.3} & 57.7 & \textbf{69.3} & \textbf{69.5}\\
            M2M\_418M & 31.4         & 48.5          & \textbf{44.9} & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
            M2M\_1.2B & 36.8          & 45.2          & \textbf{44.9}    & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
            Google         & \textbf{41.3}& 36.3          & 40.7  & 69.9 & 59.4 & 65.5 & 57.9 & 60.1 & 69.2 \\
            Microsoft      & 40.5         & 36.7          & 43.5  & 79.9 & 73.4 & 70.2 & \textbf{60.0}   & 66.6 & 64.2 \\
            Microsoft      & 40.5         & 36.7          & 43.5  & 78.0   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 \\
            Opus-MT       & 37.4         & 35.3          & 43.6 & 68.2 & 56.0   & 63.2 & 49.8 & 59.0   & 59.8 \\
            \bottomrule
        \end{tabular}}
    \caption{Target-side consistency results of commercial and open-source MT on Wino-X and WinoMT when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy.}
\end{table*}

==> tables/wino-mt/03_consistency_gmf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[tb!]
\centering
\begin{tabular}{lrrrrrr}
\toprule
%  &
%   \multicolumn{1}{c}{German} &
%   \multicolumn{1}{c}{Spanish} &
%   \multicolumn{1}{l}{French} &
%   \multicolumn{1}{l}{Russian} &
%   \multicolumn{1}{c}{Hebrew} &
%   \multicolumn{1}{c}{Arabic} \\
 &
  \multicolumn{1}{c}{en$\rightarrow$de} &
  \multicolumn{1}{c}{en$\rightarrow$es} &
  \multicolumn{1}{l}{en$\rightarrow$fr} &
  \multicolumn{1}{l}{en$\rightarrow$ru} &
  \multicolumn{1}{c}{en$\rightarrow$he} &
  \multicolumn{1}{c}{en$\rightarrow$ar} \\
\midrule
mBART50   & \textbf{77.7} & \textbf{75.2} & \textbf{73.3} & 57.7 & \textbf{69.3} & \textbf{69.5} \\
M2M\_418M & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
M2M\_1.2B & 69.9 & 59.4 & 65.5 & 57.9 & 60.1 & 69.2 \\
Google         & 79.9 & 73.4 & 70.2 & \textbf{60.0}   & 66.6 & 64.2 \\
Microsoft      & 78.0   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 \\
Opus-MT       & 68.2 & 56.0   & 63.2 & 49.8 & 59.0   & 59.8 \\
% random data    & 68.2 & 59.2 & 66   & 65.4 & 67.8 & 64.5 \\
% coref data     & 75.1 & 60.6 & 68.3 & 61.6 & 68.1 & 66.2 \\
% +signal       & 78.5 & 60.1 & 68.6 & 58.4 & 69   & 60.9 \\
% +gold         & 79.3 & 60   & 69.1 & 60.9 & 68.5 & 62.7 \\
\bottomrule
\end{tabular}
\caption{Target-side consistency results of commercial and open-source MT on WinoMT when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy.}
%\gabis{consider merging with Table~\ref{table:gmf_cons_winox}}}
\label{table:gmf_cons_wino-mt}
\end{table*}


==> tables/wino-mt/05_consistency_ours.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht!]
\centering
\begin{tabular}{lrrrrrr}
\toprule
%  &
%   \multicolumn{1}{c}{German} &
%   \multicolumn{1}{c}{Spanish} &
%   \multicolumn{1}{l}{French} &
%   \multicolumn{1}{l}{Russian} &
%   \multicolumn{1}{c}{Hebrew} &
%   \multicolumn{1}{c}{Arabic} \\
&
  \multicolumn{1}{c}{en$\rightarrow$de} &
  \multicolumn{1}{c}{en$\rightarrow$es} &
  \multicolumn{1}{l}{en$\rightarrow$fr} &
  \multicolumn{1}{l}{en$\rightarrow$ru} &
  \multicolumn{1}{c}{en$\rightarrow$he} &
  \multicolumn{1}{c}{en$\rightarrow$ar} \\
\midrule
% mbart50\_m2m   & 77.7 & 75.2 & 73.3 & 57.7 & 69.3 & 69.5 \\
% m2m\_100\_418M & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
% m2m\_100\_1.2B & 69.9 & 59.4 & 65.5 & 57.9 & 60.1 & 69.2 \\
% Google         & 79.9 & 73.4 & 70.2 & 60   & 66.6 & 64.2 \\
% Microsoft      & 78   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 \\
Opus-MT       & 68.2 & 56.0   & 63.2 & 49.8 & 59   & 59.8 \\
% random data    & 68.2 & 59.2 & 66   & 65.4 & 67.8 & 64.5 \\
Gender data     & 75.1 & \textbf{60.6} & 68.3 & \textbf{61.6} & 68.1 & \textbf{66.2} \\
$+$coref markers       & \textbf{78.5} & 60.1 & \textbf{68.6} & 58.4 & \textbf{69.0}   & 60.9 \\
%\quad$+$gender         & \textbf{79.3} & 60   & \textbf{69.1} & 60.9 & 68.5 & 62.7 \\
\bottomrule
\end{tabular}
\caption{Target-side consistency results of our implicit and explicit fine tuning approaches on WinoMT.\ariec{Add coref-data and gold. Explain why we also train on Gender data (subset of coref data) on WinoMT.}}
\label{table:ours_cons_wino-mt}
\end{table*}

==> tables/wino-x/02_Wino-x_gmf_con.tex <==
\begin{table}[tb!]
\begin{tabular}{llll}
\toprule
               & en$\rightarrow$de        & en$\rightarrow$fr        & en$\rightarrow$ru        \\
%               & Con.            & Con.             & Con.             \\
\midrule
mBART50   & 37.4         & \textbf{56.6} & 44.6          \\
M2M\_418M & 31.4         & 48.5          & \textbf{44.9}          \\
M2M\_1.2B & 36.8          & 45.2          & \textbf{44.9}          \\
Google         & \textbf{41.3}& 36.3          & 40.7          \\
Microsoft      & 40.5         & 36.7          & 43.5          \\
Opus-MT       & 37.4         & 35.3          & 43.6          \\
\bottomrule
\end{tabular}
\caption{Target-side consistency results of commercial and open-source MT on Wino-X when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy.}
\label{table:gmf_cons_winox}
\end{table}

==> tables/wino-x/04_Wino-x_ours_con.tex <==
\begin{table}[tb!]
\centering
\begin{tabular}{llll}
\toprule
               & en$\rightarrow$de        & en$\rightarrow$fr         & en$\rightarrow$ru        \\
\midrule
Opus-MT      & 37.4         & 35.3          & 43.6          \\
%random data    & 39.9         & 38.4          & 42.1          \\
coref data     & 42.7         & 41.0          & 44.0          \\
$+$coref markers       & 44.1         & 42.6          & 45.5          \\
$+$gold markers        & \textbf{44.7} & \textbf{45.8}          & \textbf{50.5} \\
\bottomrule
\end{tabular}
\caption{Target-side consistency results of our implicate and explicate fine tuning approaches and on Wino-X}
\label{table:ours_cons_winox}
\end{table}

==> tables/winomt_bug.tex <==
\begin{table*}[!htb]
    % \caption{Global caption}
    \centering
    \scalebox{0.95}{
           \begin{tabular}{llcccccclcccccc}
            \toprule
            && \multicolumn{6}{c}{WinoMT} && \multicolumn{6}{c}{BUG} \\
            \midrule
             
             &&
             de & 
             es & 
             fr & 
             ru & 
             he & 
             ar &&
             de & 
             es & 
             fr & 
             ru & 
             he & 
             ar &
             
    
            \midrule
            mBART50   && 77.7 & \textbf{75.2} & \textbf{73.3} & 57.7 & \textbf{69.3} & \textbf{69.5} && 74.6 & 69.4 & 76.0 & 69.1 & 80.2 & 83.0 \\
            M2M\_418M && 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 && 81.3 & 84.9 & 86.0 & \textbf{71.6} & 83.6 & 85.1  \\
            M2M\_1.2B && 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 && \textbf{83.5} & 85.1 & \textbf{90.3} & 70.4 & \textbf{89.6} & \textbf{93.4} \\
            Google   && 69.9 & 59.4 & 65.5 & \textbf{57.9} & 60.1 & 69.2 && 56.0 & 84.4 & 89.2 & 71.0 & 85.2 & 91.9 \\
           % Microsoft      & 40.5         & 36.7          & 43.5  & 79.9 & 73.4 & 70.2 & \textbf{60.0}   & 66.6 & 64.2 \\
            Microsoft     & & \textbf{78.0}   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 && 77.2 & \textbf{86.7} & 86.0 & 67.2 & 84.0 & 89.8  \\
            Opus-MT       && 68.2 & 56.0   & 63.2 & 49.8 & 59.0   & 59.8 && 79.8 & 85.1 & 86.2 & 67.3 & 88.8 & 88.0\\
            \bottomrule
        \end{tabular}}
    \caption{Target-side consistency results of commercial and open-source MT systems on WinoMT and BUG when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy. .\vspace{-.3cm}}
    \label{table:winomt_bug}
\end{table*}















% % \begin{tabular}{llll}
% % \toprule
% %               & German         & French         & Russian        \\
% % %               & PM             & PM             & PM             \\
% % \midrule
% % mBART50   & 38.1          & \textbf{47.2} & 34.7          \\
% % M2M00\_418M & 33.8          & 39.5          & 32.4          \\
% % M2M100\_1.2B & 38.5          & 39.0          & 33.7          \\
% % Google         & \textbf{44.2}          & 34.8          & 35.8          \\
% % Microsoft      & 43.1          & 35.7          & \textbf{37.8}           \\
% % EasyNMT       & 39.9          & 31.8          & 37.0             \\
% % % random data    & 40.78          & 35.14          & 34.63          \\
% % % coref data     & 42.26          & 38.86          & 34.99          \\
% % % "+signal       & 43.59          & 39.32          & 37.22          \\
% % % "+gold         & \textbf{45.71} & 42.7           & \textbf{42.63} \\
% % \bottomrule
% % \end{tabular}
% % \quad
% % \begin{tabular}{llll}
% % \toprule
% %               & German         & French         & Russian        \\
% % %               & PM             & PM             & PM             \\
% % \midrule
% % mBART50   & 38.1          & \textbf{47.2} & 34.7          \\
% % M2M00\_418M & 33.8          & 39.5          & 32.4          \\
% % M2M100\_1.2B & 38.5          & 39.0          & 33.7          \\
% % Google         & \textbf{44.2}          & 34.8          & 35.8          \\
% % Microsoft      & 43.1          & 35.7          & \textbf{37.8}           \\
% % EasyNMT       & 39.9          & 31.8          & 37.0             \\
% % % random data    & 40.78          & 35.14          & 34.63          \\
% % % coref data     & 42.26          & 38.86          & 34.99          \\
% % % "+signal       & 43.59          & 39.32          & 37.22          \\
% % % "+gold         & \textbf{45.71} & 42.7           & \textbf{42.63} \\
% % \bottomrule
% % \end{tabular}

% \begin{table*}[!htb]
%     % \caption{Global caption}
%     \centering
%     \begin{minipage}{.4\linewidth}
%     %   \centering
%         \small
%         \begin{tabular}{llll}
%         \toprule
%                       & en$\rightarrow$de        & en$\rightarrow$fr         & en$\rightarrow$ru        \\
%         \midrule
%         Opus-MT      & 37.4         & 35.3          & 43.6          \\
%         %random data    & 39.9         & 38.4          & 42.1          \\
%         coref data     & 42.7         & 41.0          & 44.0          \\
%         $+$coref markers       & 44.1         & 42.6          & 45.5          \\
%         $+$gold markers        & \textbf{44.7} & \textbf{45.8}          & \textbf{50.5} \\
%         \bottomrule
%         \end{tabular}
%         \caption{Wino-X}
%     \end{minipage}%
%     % \centering
%     \begin{minipage}{.6\linewidth}
%     %   \centering
%         \small
%         \begin{tabular}{lrrrrrr}
%         \toprule
%         %  &
%         %   \multicolumn{1}{c}{German} &
%         %   \multicolumn{1}{c}{Spanish} &
%         %   \multicolumn{1}{l}{French} &
%         %   \multicolumn{1}{l}{Russian} &
%         %   \multicolumn{1}{c}{Hebrew} &
%         %   \multicolumn{1}{c}{Arabic} \\
%         &
%           \multicolumn{1}{c}{en$\rightarrow$de} &
%           \multicolumn{1}{c}{en$\rightarrow$es} &
%           \multicolumn{1}{l}{en$\rightarrow$fr} &
%           \multicolumn{1}{l}{en$\rightarrow$ru} &
%           \multicolumn{1}{c}{en$\rightarrow$he} &
%           \multicolumn{1}{c}{en$\rightarrow$ar} \\
%         \midrule
%         % mbart50\_m2m   & 77.7 & 75.2 & 73.3 & 57.7 & 69.3 & 69.5 \\
%         % m2m\_100\_418M & 69.7 & 55.1 & 65.4 & 54.7 & 56.5 & 64.3 \\
%         % m2m\_100\_1.2B & 69.9 & 59.4 & 65.5 & 57.9 & 60.1 & 69.2 \\
%         % Google         & 79.9 & 73.4 & 70.2 & 60   & 66.6 & 64.2 \\
%         % Microsoft      & 78   & 66.5 & 69.3 & 57.3 & 63.9 & 60.7 \\
%         Opus-MT       & 68.2 & 56.0   & 63.2 & 49.8 & 59   & 59.8 \\
%         % random data    & 68.2 & 59.2 & 66   & 65.4 & 67.8 & 64.5 \\
%         Gender data     & 75.1 & \textbf{60.6} & 68.3 & \textbf{61.6} & 68.1 & \textbf{66.2} \\
%         $+$coref markers       & \textbf{78.5} & 60.1 & \textbf{68.6} & 58.4 & \textbf{69.0}   & 60.9 \\
%         %\quad$+$gender         & \textbf{79.3} & 60   & \textbf{69.1} & 60.9 & 68.5 & 62.7 \\
%         \bottomrule
%         \end{tabular}
%         \caption{WinoMT}
%     \end{minipage} 
%     \caption{Target-side consistency results of our fine-tuning approaches on Wino-X and WinoMT when translating into different languages. These numbers are an upper bound for the source-side coreference accuracy.}
% \end{table*}

==> tables/winox_cons.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lccc}
    \toprule
    & en $\rightarrow$ de & en $\rightarrow$ fr & en $\rightarrow$ ru \\
    \midrule
    mBART50   & 37.4         & \textbf{56.6} & 44.6    \\
    M2M\_418M & 31.4         & 48.5          & \textbf{44.9} \\
    Google         & \textbf{41.3}& 36.3          & 40.7 \\
    Microsoft      & 40.5         & 36.7          & 43.5 \\
    Opus-MT       & 37.4         & 35.3          & 43.6 \\
    \bottomrule
    \end{tabular}
    \caption{Target-side consistency results of commercial and open-source MT systems on Wino-X when translating into German, French and Russian.}
    \label{tab:winox_cons}
\end{table}


==> tables_new/exampels_improvment.tex <==
\begin{table*}[ht]
% \begin{tabular}{lll}
\centering
\small
\resizebox{1\textwidth}{!}{
\begin{tabular}{p{8cm}p{8cm}p{0.1cm}}
\toprule
Source & {[}Target lang.{]} Predicted translation &  \\
  \midrule
% \parbox{5cm}{  The \textcolor{orange}{sheriff} gave the  \textcolor{orange}{secretary} no more chances and arrested  \textcolor{blue}{him}.} &
%   \parbox{5.5cm}{{[}FR.{]}  \textcolor{blue}{Le shérif} n'a donné aucune chance au \textcolor{blue}{secrétaire} et l'a \textcolor{blue}{arrêté}.} &
%   \parbox{5cm}{ In French, the candidate pronoun is the verb ``arrêté''.} \\
%   \midrule

% RU example:
  % The factory worker had a hard time loading the \textcolor{orange}{furniture} on the \textcolor{orange}{truck} because \textcolor{orange}{it} was too big.
  % &
  % {{[}RU.{]} \foreignlanguage{russian}{Работнику завода было трудно загрузить \textcolor{red}{мебель} в \textcolor{blue}{грузовик}, потому что \textcolor{blue}{он}  был слишком больим}} &
  % \textbf{\textcolor{red}{\xmark}} \\
  % \midrule
  % {The factory worker had a hard time loading the <ENT1> \textcolor{orange}{furniture} </ENT1> on the \textcolor{orange}{truck} because <ENT1> \textcolor{orange}{it} </ENT1> was too big.} &
  % {{[}RU.{]} \foreignlanguage{russian}{Работнику завода было трудно загрузить \textcolor{red}{мебель} в \textcolor{blue}{грузовик}, потому что \textcolor{red}{она}  был слишком большим}} &
  % \textbf{\textcolor{greenrgb}{\cmark}} \\

% FR example:
  % The chickens escaped from the \textcolor{orange}{yard} and fled to the \textcolor{orange}{field}, as they found \textcolor{orange}{it} so confining..
  % &
  % {{[}FR.{]} Les poulets se sont échappés de \textcolor{red}{la cour} et ont fui vers \textcolor{blue}{le champ}, comme ils l'ont \textcolor{blue}{trouvé} si restreint.} \\
  % \midrule
  % {The factory worker had a hard time loading the <ENT1> \textcolor{orange}{furniture} </ENT1> on the \textcolor{orange}{truck} because <ENT1> \textcolor{orange}{it} </ENT1> was too big.} &
  % {{[}RU.{]} \foreignlanguage{russian}{Работнику завода было трудно загрузить \textcolor{red}{мебель} в \textcolor{blue}{грузовик}, потому что \textcolor{red}{она}  был слишком большим}} &
  % \textbf{\textcolor{greenrgb}{\cmark}} \\

The chickens escaped from the \textcolor{orange}{yard} and fled to the \textcolor{orange}{field}, as they found \textcolor{orange}{it} so confining. &
  {{[}FR.{]} Les poulets se sont échappés de \textcolor{red}{la cour} et ont fui vers \textcolor{blue}{le champ}, comme ils \textcolor{blue}{l'}ont trouv\textcolor{blue}{é} si restreint.} &
%  \parbox{5cm}{ In the baseline translation to French the pronoun has different gender than the coreferring entity} 
  \textbf{\textcolor{red}{\xmark}} \\

  \midrule
{The chickens escaped from the <ENT1> \textcolor{orange}{yard} </ENT1> and fled to the \textcolor{orange}{field}, as they found <ENT1> \textcolor{orange}{it} </ENT1> so confining.} &
  {{[}FR.{]} Les poulets se sont échappés de \textcolor{red}{la cour} et ont fui vers \textcolor{blue}{le champ}, car ils \textcolor{red}{l'}ont trouv\textcolor{red}{ée} si encombrée.} &
%  \parbox{5cm}{ Our model translation to French has the same gender to the pronoun and the coreferring entity} \\
  \textbf{\textcolor{greenrgb}{\cmark}} \\

\bottomrule
% The developer argued with the designer\\ because she did not like the design. &
%   {[}ES.{]} La desarrolladora discutió con la\\ diseñadora porque no le gustaba el diseño. &
%   The pronoun is dropped in Spanish \\
%   \midrule
% The developer argued with the designer\\ because his idea cannot be implemented. &
%   {[}ES.{]} El desarrollador discutió\\ con el diseñador porque su idea no puede ser implementada. &
%   The pronoun is dropped in Spanish \\
% The physician examined the teacher\\ and she was unable to find the source of the illness. & \\
% \midrule

%   {[}HE.{]} הרופאה בדקה את המורה ולא הצליחה למצוא את מקור המחלה. &
%   \\
% The construction worker asked the attendant to not lose her car. &
%   {[}HE.{]} עובד הבניין ביקש מהדיילת לא לאבד את מכוניתה. &
%   \\
% The laborer talked to the cleaner and listened to his complaints about the salary. &
%   {[}HE.{]} הפועל דיבר עם המנקה והאזין לתלונותיו על המשכורת. &
  
\end{tabular}
}
\caption{Translation example of a Wino-X sentence to French by the baseline (first row) and our model (second row). Words in blue, red, and orange indicate male, female and neutral entities, respectively.}
\label{table:lang_exampels}
\end{table*}

==> tables_new/lang_improv_app.tex <==
\begin{table*}[ht]
% \begin{tabular}{lll}
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{p{7cm}p{7.5cm}p{0.5cm}}
\toprule
Source & {[}Target lang.{]} Predicted translation &  \\
  \midrule
\parbox{7cm}{Bob would rather fill his emergency fund using his \textcolor{orange}{mobile} instead of the \textcolor{orange}{bank} because \textcolor{orange}{it} was closed.} &
  \parbox{7.5cm}{{[}FR.{]} Bob préférerait remplir son fonds d'urgence en utilisant son \textcolor{blue}{mobile} au lieu de la \textcolor{red}{banque} parce \textcolor{blue}{qu'il} était fermé.} &
  % \parbox{5cm}{ In the baseline translation to French the pronoun have different gender than the coreferring entity} \\
    \textbf{\textcolor{red}{\xmark}} \\
  \midrule
\parbox{7cm}{Bob would rather fill his emergency fund using his \textcolor{orange}{mobile} instead of the <ENT1> \textcolor{orange}{bank} </ENT1> because <ENT1> \textcolor{orange}{it} </ENT1> was closed.} &
  \parbox{7.5cm}{{[}FR.{]} Bob préférerait remplir son fonds d'urgence en utilisant son \textcolor{blue}{téléphone} portable au lieu de la \textcolor{red}{banque} parce \textcolor{red}{qu'elle} était fermée.} &
  % \parbox{5cm}{ Our model translation to French have the same gender to the pronoun and the coreferring entity} \\
    \textbf{\textcolor{greenrgb}{\cmark}} \\
  % \bottomrule

  \midrule
  \parbox{7cm}{The headphones blocked the \textcolor{orange}{noise} but not the \textcolor{orange}{vibration}, as \textcolor{orange}{it} was relatively strong.}
  &
  \parbox{7.5cm}{{{[}RU.{]} \foreignlanguage{russian}{Наушники блокировали \textcolor{blue}{шум}, но не \textcolor{red}{вибрацию}, поскольку \textcolor{blue}{он} был относительно сильным.}}} &
  \textbf{\textcolor{red}{\xmark}} \\
  \midrule
  \parbox{7cm}{The headphones blocked the \textcolor{orange}{noise} but not the <ENT1> \textcolor{orange}{vibration} </ENT1>, as <ENT1> \textcolor{orange}{it} </ENT1> was relatively strong.} &
  \parbox{7.5cm}{{{[}RU.{]} \foreignlanguage{russian}{Наушники блокировали \textcolor{blue}{шум}, но не \textcolor{red}{вибрацию}, так как \textcolor{red}{она} была относительно сильной.}}} &
  \textbf{\textcolor{greenrgb}{\cmark}} \\
  \bottomrule
\end{tabular}
}
\caption{Examples of sentences from our datasets and their translations. Those translation examples show a case where the baseline model fails to generate the correct translation, but our model succeeds. Words in blue,
red, and orange indicate male, female and neutral entities, respectively.}
\label{table:lang_improve_app}
\end{table*}

==> zh_yshan/01_introduction.tex <==
% In recent years NMT models are showing great success (ref), and even achieving near human level results (ref). in order to successfully perform MT, thoes models need to successfully perform a number of NLP tasks implicitly.

Machine translation is a complex task that requires solving several NLP tasks implicitly and poses diverse linguistic knowledge in order to perform successfully. NMT models need to solve tasks such as NER, POS tagging, and coreference resolution (CR) implicitly in order to generate correct translation. A lot of times the way those models are evaluated is only by comparing their output to a gold translation without examining how well the model performs those required tasks.

In this work, we propose a new metric aiming to assess the coreference resolution consistency of an NMT model. Our method is based on the requirement that different mentions in the same cluster will have the same gender (i.e. Gender agreement). This constraint is necessary but not sufficient by itself to indicate that two mentions are in the same cluster. Therefore, our metric provides an upper bound of the model coreference resolution ability and only measures its consistency.

Using that metric we are comparing monolingual CR models with NMT. In our comparison, we show that monolingual models are marginally more accurate than NMT models. Based on that observation we advise a new way of fine-tuning on parallel data with injected monolingual coreference signal. We enrich the data with monolingual coreference signal by adding both coreference and gender markers. additionally, we compare ourselves with fine-tuning on the data without any markers and fine-tuning on random data. We conduct experiments on six languages and two data sets. 

our main contributions are:
    \begin{itemize}

    \item The observation that monolingual CR models are more accurate than NMT models.
    \item A new metric for measuring coreference resolution consistency of NMT model.
    \item A new method for improving coreference resolution consistency that enhance performances on several languages multiple data sets.

    \end{itemize}
